An Adaptive Mixed Precision and Dynamically Scaled Preconditioned Conjugate Gradient Algorithm

We propose an adaptive mixed precision and dynamically scaled preconditioned conjugate gradient algorithm (AMP-PCG). It dynamically adjusts the precision for storing vectors and computing, exploiting low precision when appropriate, while maintaining a convergence rate and accuracy comparable to that of double precision PCG. Our mixed precision strategy consists of three main components: (1) The residual and matrix-vector product are initially computed in double precision, and the algorithm switches these to single precision based on the chosen convergence tolerance and an estimate of the residual gap. (2) Depending on the eigenvalue distribution, the preconditioned residual and search direction are either in half precision throughout the iterations or initially in double precision and then stepwise reduced to single and half precision. (3) A dynamically scaled residual is used at every iteration to mitigate underflow in half precision. We provide theoretical support for our estimates and we demonstrate the effectiveness of AMP-PCG through numerical experiments, highlighting both its robustness and the significant performance gains (1.63x speedup) achieved compared to double precision PCG on a GPU.

==> 5.Numerical/5.libpResultBackup.tex <==
In this subsection, we compare and analyze the performance of the double precision PCG and \APCG{}  algorithm on a GPU.
\begin{example}
    Consider the screened Poisson equation
\begin{equation}
- \Delta u(x,y,z) + \lambda \, u(x,y,z) = f(x,y,z) \quad \text{in } \Omega=[-0.5,0.5]^3,
\label{eq:screened poisson}
\end{equation}
with Dirichlet boundary conditions and $\lambda=10^3$. The forcing function $f(x,y,z)$ is defined in \cref{eq:f}. 
The equation is discretized using a high-order finite element method with a polynomial degree of $N=7$ on a mesh with $40\times 40\times 40$  tensor-product hexahedral elements, yielding approximately $21.7 \times 10^6$ DoFs. For simplicity in performance analysis, we consider solving the linear system using both double precision PCG and \APCG{} with a Jacobi preconditioner.
\label{ex: jac libp}
\end{example}

All computations are performed on an NVIDIA H100 SXM 80GB GPU. We assume that the physical elements are mapped from the reference element via trilinear mappings. As a result, the geometry factors involved in the matrix-free operations can be calculated from the coordinates of the element vertices ($3\times 8\times N_{\text{element}}$, where $N_{\text{element}}$ is the number of elements)  which requires a negligible memory footprint compared to the total number of DoFs.
The experiments were performed using libParanumal \cite{ChalmersKarakusAustinSwirydowiczWarburton2020}. 

In \cref{fig: performance convg}, we present the convergence curves for  the fully double-precision implementation and \APCG(FP64), where the precisions of $u_{z,k}$ and $u_{r,k}$ are adaptively selected based on \cref{eq: criterion}. The convergence behavior of \APCG(FP64) closely follows that of the fully double-precision PCG.
The \APCG(FP64) process consists of three phases: 
(1) all vectors in double precision, 
(2) $\Bz_k$ and $\Bp_k$ in single precision, 
(3) $\Bz_k$ and $\Bp_k$  in half precision, with $\Br_k$ and $\Bq_k$  in single precision. 
Using a stopping criterion of $\| \mathbf{r}_k \| \leq 10^{-12} \| \mathbf{r}_0 \|$, \APCG(FP64) achieves a speedup of over $1.12\times$ compared to the fully double-precision PCG.
In \cref{fig:performance_runtime}, we analyze the runtime of each phase for five main kernels involved in \APCG: \texttt{zamx}, \texttt{innerProd}, \texttt{axpy}, \texttt{Ax}, and \texttt{updatePCG}, collected from \textit{Nsight Compute}. Among these, all except \texttt{Ax} are memory-bound. Therefore, their maximum achievable speedup can be estimated based on the amount of data movement, as summarized in \cref{tab:pcg_cost}. 
% Speedup of \texttt{zamx} and \texttt{innerProd} kernels of phase 2 and phase 3 over phase 1 aligns well with the maximu speedup in 
% \cref{tab:pcg_cost}

% \begin{figure}[h!]
% \centering
% \begin{tikzpicture}
% \begin{groupplot}[
%     group style={
%         group name=myplot,
%         group size=2 by 1,
%         horizontal sep=20pt,
%         vertical sep=2cm
%     },
%     height=5cm,
%     width=5.5cm
% ]
%   % First plot with y-axis labels
%   \nextgroupplot[
%   title={(a) Updated residual},
%     xlabel={Iteration},
%     ylabel={Relative residual norm},
%     ymode=log,
%     ymin=1e-15,
%     ymax=100,
%   ]
%   \input{5.Numerical/data/libp_Res}
  
%   % Second plot without y-axis tick labels
%   \nextgroupplot[
%     title={(b) True residual},
%     xlabel={Iteration},
%     ymode=log,
%     ymin=1e-15,
%     ymax=100,
%     yticklabels={}
%   ]
%   \input{5.Numerical/data/libp_trueRes}
 
% \end{groupplot}

% \path (myplot c1r1.south west|-current bounding box.south)--
%       coordinate(legendpos)
%       (myplot c2r1.south east|-current bounding box.south);

% \matrix[
%     matrix of nodes,
%     anchor=west, % align the left edge of the legend with the anchor point
%     draw,
%     inner sep=0.2em,
%     nodes={font=\small}
% ] at ([xshift=2em]myplot c2r1.east) % shift a bit to the right
% {
% \ref{plot:fp64} &  PCG(FP64)\\
%     \ref{plot:fp64mixed} & \APCG(FP64)\\
%     \ref{plot:fp64tofp32} & $ u_{z,k}=\mathrm{FP32}$ \\
%     \ref{plot:fp32tofp16} & $ u_{z,k}=\mathrm{FP16}$ \\
%     \ref{plot:residualfp64tofp32} & $ u_{r,k}=\mathrm{FP32}$ \\
%     \\
% };
% \end{tikzpicture}
% \caption{
% Convergence curves of the relative residual norm for two PCG variant: fully double-precision CG and \APCG(FP64), applied to the Poisson equation with high-order finite element discretization and Jacobi preconditioner, as discussed in \cref{ex: jac libp}. The red crosses indicate the iterations at which $u_{z,k}$ (i.e., the precision of $\Bz_k$ and $\Bp_k$) is set to single precision in \APCG(FP64), while the black crosses mark those where $u_{z,k}$ is set to half precision. Similarly, the blue circle symbols denote the iterations where $u_{r,k}$ is switched to single precision.
% }
% \label{fig: performance convg}
% \end{figure}


\begin{figure}[h!]
\centering
\begin{tikzpicture}
\begin{axis}[
    name=myplot,
    height=5cm,
    width=7cm,
    xlabel={Iteration},
    ylabel={Relative residual norm},
    ymode=log,
    ymin=1e-11,
    ymax=100,
    grid=both,
]
  \input{5.Numerical/data/libp_Res}
\end{axis}

\path (myplot.south west |- current bounding box.south) --
      coordinate(legendpos)
      (myplot.south east |- current bounding box.south);

\matrix[
    matrix of nodes,
    anchor=west,
    draw,
    inner sep=0.2em,
    nodes={font=\small}
] at ([xshift=2em]myplot.east) {
    \ref{plot:fp64} &  PCG(FP64)\\
    \ref{plot:fp64mixed} & \APCG(FP16)\\
    % \ref{plot:fp64tofp32} & $ u_{z,k}=\mathrm{FP32}$ \\
    % \ref{plot:fp32tofp16} & $ u_{z,k}=\mathrm{FP16}$ \\
    \ref{plot:residualfp64tofp32} & $ u_{r,k}=\mathrm{FP32}$ \\
    \\
};
\end{tikzpicture}
\caption{%
Convergence curves of the relative residual norm for two PCG variants: fully double-precision PCG and \APCG(FP16), applied to the Poisson equation with high-order finite element discretization and Jacobi preconditioner, as discussed in \cref{ex: jac libp}. The red crosses indicate iterations where $u_{z,k}$ (i.e., the precision of $\Bz_k$ and $\Bp_k$) is set to single precision, the black crosses to half precision, and the blue circles mark when $u_{r,k}$ switches to single precision.
}
\label{fig: performance convg}
\end{figure}



\begin{figure}[htbp]
    \centering
  \begin{tikzpicture}
  \begin{axis}[
    ybar=0.25cm,
    x=2.5cm,
    bar width=12pt,
    width=14cm,
    height=6cm,
    ymin=0,
    enlarge x limits=0.15,
    symbolic x coords={zamx, innerProd, axpy, Ax, updatePCG},
    xtick=data,
    ylabel={Duration (\(\mu\)s)},
    ylabel style={font=\small},
    % xticklabel style={font=\small, rotate=0, anchor=east},
    major x tick style=transparent,
    legend style={at={(0.25, 0.62)}, anchor=south, legend columns=1, font=\small},
    nodes near coords,
    every node near coord/.append style={
        font=\footnotesize,
        text=black
    },
    nodes near coords style={
        /pgf/number format/fixed,
        /pgf/number format/precision=0
    },
    legend style={font=\small}
  ]
   \addplot[draw=mylightblue, fill=mylightblue,
     point meta=explicit symbolic,
    nodes near coords style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2,
        text=black
    }
    ] 
 coordinates { 
(zamx, 325.90) [1.0]
 (innerProd, 216.00)  [1.0]
 (axpy, 281.54)  [1.0]
 (Ax, 1850)  [1.0]
 (updatePCG, 752.83)  [1.0]
 }; 
   \addplot[draw=vtorange, fill=vtorange, 
       point meta=explicit symbolic,
    nodes near coords style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2,
        text=black
    }
    ] 
 coordinates { 
(zamx, 227.14) [1.43]
 (innerProd, 163.68)  [1.32]
 (axpy, 162.27)  [1.73]
 (Ax, 1830)  [1.01]
 (updatePCG, 703.89)  [1.07]
 }; 
   \addplot[draw=mygreen, fill=mygreen,
       point meta=explicit symbolic,
    nodes near coords style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2,
        text=black
    }] 
 coordinates { 
(zamx, 114.88) [2.83]
 (innerProd, 89.07)  [2.42]
 (axpy, 104.43)  [2.7]
 (Ax, 1130)  [1.63]
 (updatePCG, 452.59)  [1.66]
 }; 
    \legend{
        {Phase 1 (all double)},
        {Phase 2 (single $\mathbf{z}_k, \mathbf{p}_k$)},
        {Phase 3 (half, $\mathbf{z}_k$, $\mathbf{p}_k$, single $\mathbf{r}_k$, $\mathbf{q}_k$)}
    }
    \end{axis}
\end{tikzpicture}
\caption{
Runtime of the main kernels in \APCG{}, measured on an NVIDIA H100 SXM 80GB GPU using \textit{Nsight Compute}.
Numbers on the top of bars are the speedup relative to phase 1.
The test case uses a mesh with $50 \times 50 \times 50$ elements and polynomial degree $N=7$, yielding approximately $42.5 \times 10^6$ degrees of freedom.
Phase~1 includes iterations where all variables are stored in double precision.
Phase~2 begins when $u_{z,k}$ is stored in FP32, and Phase~3 starts when $u_{z,k}$ is further reduced to FP16 while $u_{r,k}$ is stored in FP32.
The corresponding data movement per degree of freedom is detailed in \cref{tab:pcg_cost}.
% With a stopping criterion of $\|\Br_k\| \leq 10^{-12} \|\Bb\|$, \APCG{} achieves an 11.2\% speedup compared to double-precision PCG.
The convergence history is shown in \cref{fig: performance convg}.
}
    \label{fig:performance_runtime}
\end{figure}




\begin{table}[htbp]
  \centering
  \caption{Data movement (read and write) per degree of freedom in \APCG{}, measured in bytes. Here, $\BM$ denotes the Jacobi preconditioner. $N_{\ell}$ is the number of local DoFs and $N_s$ is the number of global DoFs.}
  \label{tab:pcg_cost}
  \begin{tabular}{|l|l|c|c|c|}
    \hline
    \multirow{ 3}{*}{Kernel} & {Phase} & {Phase 1} & {Phase 2} & {Phase 3} \\
    \cline{2-5}
    & \multirow{ 2}{*}{Precision} & \multirow{ 2}{*}{All FP64} & \multirow{ 2}{*}{$u_{z,k}=$ FP32} & $u_{z,k}=$ FP16 \\
    & & & &  $u_{r,k}=$ FP32 \\
    \hline
    \texttt{zamx} & $\Bz = \BM \Br$ & 24 & 16 & 8 \\       
    \texttt{innerProd} &$\gamma = \Bz^T\Br$ &  16 & 12 & 6 \\
     \texttt{axpy} &$\Bp = \Bz + \beta\Bp$ & 24 & 12 & 6 \\
     \texttt{Ax} &$\Bq = \BA\Bp$, $\mu = \Bp^T\Bq$ & $\approx 28\,{N_{\ell}}/{N_s}$ & $\approx 24\,{N_{\ell}}/{N_s}$ & $\approx 14\,{N_{\ell}}/{N_s}$ \\
    \texttt{updatePCG} & $\Br = \Br - \alpha\Bq$, $\Bx = \Bx + \alpha\Bp$, $\|\Br\|$ &  48 & 44 & 22 \\
    % \hline
    % \multicolumn{2}{|l|}{{Total}} & $28\,{N_{\ell}}/{N_s} + 112$ & $24\,{N_{\ell}}/{N_s} + 84$ & $14\,{N_{\ell}}/{N_s} + 42$ \\
    % \multicolumn{2}{|l|}{{Max speedup ($N=7$)}} & 1.00 & 1.28 & 2.44 \\
    \hline
  \end{tabular}
\end{table}


==> 5.Numerical/data/libp_trueRes.tex <==
\addplot[color=myyellow, line width=1.0pt] coordinates { 
(0, 1)
(1, 2.794701306665e+00)
(2, 3.142935711860e+00)
(3, 4.045519460022e+00)
(4, 6.095535090402e+00)
(5, 7.297648228026e+00)
(6, 7.094455597057e+00)
(7, 1.460626653313e+01)
(8, 9.812116039966e+00)
(9, 1.233425697931e+01)
(10, 1.113445096309e+01)
(11, 8.603083673871e+00)
(12, 8.265040172626e+00)
(13, 5.684128295503e+00)
(14, 3.095399201635e+00)
(15, 1.472347186430e+00)
(16, 6.793823783067e-01)
(17, 7.350674515587e-01)
(18, 5.666210215713e-01)
(19, 4.166077738502e-01)
(20, 3.291461835551e-01)
(21, 2.196829714011e-01)
(22, 1.555960942377e-01)
(23, 1.135021099076e-01)
(24, 6.715967683272e-02)
(25, 4.685307860738e-02)
(26, 3.259284611437e-02)
(27, 1.918678050378e-02)
(28, 7.764381834406e-03)
(29, 5.458440212424e-03)
(30, 2.970190808984e-03)
(31, 1.352037352084e-03)
(32, 7.457248802205e-04)
(33, 2.842099101740e-04)
(34, 2.053621704021e-04)
(35, 8.762189987841e-05)
(36, 4.412304709382e-05)
(37, 3.265150298006e-05)
(38, 1.843586146283e-05)
(39, 8.505353982836e-06)
(40, 3.695845077116e-06)
(41, 2.096206354989e-06)
(42, 1.108978961507e-06)
(43, 7.479695987049e-07)
(44, 3.593030470902e-07)
(45, 2.690667188631e-07)
(46, 1.037136367990e-07)
(47, 4.811951410600e-08)
(48, 3.214650118570e-08)
(49, 1.765258959174e-08)
(50, 4.511974828014e-09)
(51, 1.374414663767e-09)
(52, 6.258630869938e-10)
(53, 3.260058182051e-10)
(54, 1.028811337143e-10)
(55, 4.429714542598e-11)
(56, 2.509204306328e-11)
(57, 1.349071912706e-11)
(58, 5.440602815789e-12)
(59, 2.934239623549e-12)
(60, 2.072637427904e-12)
(61, 1.353843125457e-12)
(62, 1.279491448904e-12)
(63, 1.264158112945e-12)
(64, 1.260745454107e-12)
(65, 1.260484353617e-12)
(66, 1.272710305506e-12)
(67, 1.301164984324e-12)
(68, 1.314353651835e-12)
(69, 1.308932376895e-12)
(70, 1.311024772512e-12)
(71, 1.320424031121e-12)
(72, 1.326405936952e-12)
(73, 1.337569238252e-12)
(74, 1.373168241698e-12)
(75, 1.377191655358e-12)
(76, 1.369552100094e-12)
(77, 1.376588546485e-12)
(78, 1.382638823671e-12)
(79, 1.412550537626e-12)
(80, 1.445800896863e-12)
(81, 1.424490253323e-12)
(82, 1.422057073499e-12)
(83, 1.438610807157e-12)
(84, 1.460610759795e-12)
(85, 1.459510125132e-12)
(86, 1.461759196412e-12)
(87, 1.468574305277e-12)
(88, 1.481567433470e-12)
(89, 1.517436902257e-12)
(90, 1.502747878352e-12)
}; \label{plot:fp64} 
\addplot[color=mydeepblue, dashed, line width=1.0pt] coordinates { (1, 2.794701327454e+00) 
(2, 3.142935669830e+00) 
(3, 4.045519395242e+00) 
(4, 6.095533635739e+00) 
(5, 7.297649141490e+00) 
(6, 7.094455169275e+00) 
(7, 1.460626650792e+01) 
(8, 9.812113871664e+00) 
(9, 1.233424245743e+01) 
(10, 1.113444211481e+01) 
(11, 8.603048326191e+00) 
(12, 8.265023693238e+00) 
(13, 5.684119148290e+00) 
(14, 3.095389002943e+00) 
(15, 1.472345119849e+00) 
(16, 6.793804695828e-01) 
(17, 7.350585650220e-01) 
(18, 5.666202031530e-01) 
(19, 4.166067255483e-01) 
(20, 3.291458137172e-01) 
(21, 2.196804288715e-01) 
(22, 1.555929402774e-01) 
(23, 1.135022335216e-01) 
(24, 6.715948996353e-02) 
(25, 4.685263502135e-02) 
(26, 3.259283264164e-02) 
(27, 1.918651078883e-02) 
(28, 7.764410110951e-03) 
(29, 5.458438704844e-03) 
(30, 2.970190587065e-03) 
(31, 1.352036328918e-03) 
(32, 7.457246022691e-04) 
(33, 2.842098298669e-04) 
(34, 2.053620122608e-04) 
(35, 8.762182147424e-05) 
(36, 4.412292249793e-05) 
(37, 3.264827372282e-05) 
(38, 1.842963020752e-05) 
(39, 8.484293682572e-06) 
(40, 3.549328039965e-06) 
(41, 2.069718515599e-06) 
(42, 1.122815149652e-06) 
(43, 7.461411584927e-07) 
(44, 3.493187499108e-07) 
(45, 2.558684018434e-07) 
(46, 1.043307672291e-07) 
(47, 4.784041510037e-08) 
(48, 3.121154298914e-08) 
(49, 1.742210981798e-08) 
(50, 4.488143236352e-09) 
(51, 1.366125461489e-09) 
(52, 5.933251794920e-10) 
(53, 3.247942920372e-10) 
(54, 1.023839001538e-10) 
(55, 4.367336786445e-11) 
(56, 2.443726634512e-11) 
(57, 1.419021107077e-11) 
(58, 6.583728992623e-12) 
(59, 4.597664008450e-12) 
(60, 4.427298334326e-12) 
(61, 3.739884296030e-12) 
(62, 3.959071813233e-12) 
(63, 3.536244396190e-12) 
(64, 3.311380765203e-12) 
(65, 3.234231591193e-12) 
(66, 3.152657257986e-12) 
(67, 3.173042011257e-12) 
(68, 3.204389978861e-12) 
(69, 3.130811752401e-12) 
(70, 3.125786775948e-12) 
(71, 3.133348949527e-12) 
(72, 3.149764047703e-12) 
(73, 3.143243993539e-12) 
(74, 3.128057365327e-12) 
(75, 3.142225492500e-12) 
(76, 3.147990495246e-12) 
(77, 3.143650983224e-12) 
(78, 3.150814570401e-12) 
(79, 3.158245747828e-12) 
(80, 3.157476825352e-12) 
(81, 3.168081937555e-12) 
(82, 3.169758925494e-12) 
(83, 3.174335470340e-12) 
(84, 3.178570626108e-12) 
(85, 3.184206686524e-12) 
(86, 3.195149176600e-12) 
(87, 3.196256699636e-12) 
(88, 3.192940024956e-12) 
(89, 3.225702746148e-12) 
(90, 3.213058326873e-12) 
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=x, color=red,  mark size=3pt,  line width=1.5pt] coordinates { 
(36, 4.412292297016e-05) 
}; \label{plot:fp32tofp16} 
 \addplot[only marks, mark=x, color=black,  mark size=3pt,  line width=1.5pt] coordinates { 
(44, 3.490957684049e-07) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=o, color=blue,  mark size=3pt, line width=1.0pt] coordinates { 
(44, 3.490957684049e-07) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/limitation3.tex <==
% \addplot[color=myyellow, line width=1.0pt] coordinates { 
% (0, 1)
% (1, 1.35449)
% (2, 1.72138)
% (3, 1.37459)
% (4, 1.56375)
% (5, 1.47229)
% (6, 1.03221)
% (7, 0.796625)
% (8, 0.762054)
% (9, 0.803988)
% (10, 0.855695)
% (11, 1.05268)
% (12, 0.985007)
% (13, 0.791337)
% (14, 0.566758)
% (15, 0.497666)
% (16, 0.583826)
% (17, 0.459874)
% (18, 0.450717)
% (19, 0.360695)
% (20, 0.25205)
% (21, 0.230945)
% (22, 0.19436)
% (23, 0.203808)
% (24, 0.140429)
% (25, 0.256621)
% (26, 0.126733)
% (27, 0.117124)
% (28, 0.20549)
% (29, 0.0693786)
% (30, 0.0582846)
% (31, 0.0516264)
% (32, 0.0539919)
% (33, 0.052353)
% (34, 0.0330245)
% (35, 0.0228144)
% (36, 0.0379775)
% (37, 0.0140154)
% (38, 0.0393552)
% (39, 0.0101133)
% (40, 0.0298352)
% (41, 0.00647101)
% (42, 0.00405157)
% (43, 0.00643594)
% (44, 0.00900943)
% (45, 0.00442824)
% (46, 0.00350172)
% (47, 0.00287944)
% (48, 0.00820359)
% (49, 0.00384942)
% (50, 0.00150352)
% (51, 0.00459382)
% (52, 0.00135997)
% (53, 0.00128485)
% (54, 0.00201151)
% (55, 0.000835952)
% (56, 0.00197633)
% (57, 0.000486383)
% (58, 0.000648875)
% (59, 0.00158859)
% (60, 0.000283079)
% (61, 0.000317173)
% (62, 0.000150973)
% (63, 0.000201462)
% (64, 7.72737e-05)
% (65, 7.41552e-05)
% (66, 0.000158624)
% (67, 0.000127618)
% (68, 5.03128e-05)
% (69, 4.37537e-05)
% (70, 5.56792e-05)
% (71, 3.48398e-05)
% (72, 1.71817e-05)
% (73, 2.0153e-05)
% (74, 6.22788e-05)
% (75, 1.02538e-05)
% (76, 4.64091e-06)
% (77, 8.452e-06)
% (78, 1.67563e-05)
% (79, 2.32751e-05)
% (80, 3.06758e-06)
% (81, 1.90748e-06)
% (82, 7.79952e-06)
% (83, 6.51348e-06)
% (84, 4.0658e-06)
% (85, 2.84012e-07)
% (86, 2.62839e-07)
% (87, 3.84711e-07)
% (88, 2.15075e-07)
% (89, 6.03226e-07)
% (90, 9.64007e-07)
% (91, 1.93346e-07)
% (92, 9.83754e-09)
% (93, 6.50136e-09)
% (94, 2.28695e-09)
% (95, 1.78612e-09)
% (96, 4.02205e-09)
% (97, 4.31895e-09)
% (98, 1.80563e-09)
% (99, 3.09896e-10)
% (100, 7.14432e-11)
% (101, 3.28481e-11)
% (102, 1.6335e-11)
% (103, 4.98303e-12)
% (104, 1.73653e-12)
% (105, 3.02917e-12)
% (106, 1.77871e-12)
% (107, 1.98635e-13)
% (108, 9.5159e-14)
% (109, 3.67039e-14)
% (110, 1.68224e-14)
% (111, 2.39605e-14)
% (112, 3.05084e-15)
% (113, 1.43079e-15)
% (114, 1.03459e-15)
% (115, 6.56964e-16)
% }; \label{plot:limfp64} 
% \addplot[color=mydeepblue, line width=1.0pt] coordinates { 
% (0, 1)
% (1, 1.35449)
% (2, 1.72138)
% (3, 1.37459)
% (4, 1.56375)
% (5, 1.47229)
% (6, 1.03221)
% (7, 0.796625)
% (8, 0.762054)
% (9, 0.803988)
% (10, 0.855695)
% (11, 1.05268)
% (12, 0.985007)
% (13, 0.791337)
% (14, 0.566758)
% (15, 0.497666)
% (16, 0.583826)
% (17, 0.459874)
% (18, 0.450717)
% (19, 0.360695)
% (20, 0.25205)
% (21, 0.230945)
% (22, 0.19436)
% (23, 0.203796)
% (24, 0.13586)
% (25, 0.287537)
% (26, 0.127109)
% (27, 0.115801)
% (28, 0.155038)
% (29, 0.072899)
% (30, 0.0582579)
% (31, 0.0424393)
% (32, 0.0776161)
% (33, 0.0321003)
% (34, 0.056806)
% (35, 0.0209952)
% (36, 0.0477207)
% (37, 0.0140924)
% (38, 0.0218939)
% (39, 0.0109828)
% (40, 0.031139)
% (41, 0.00646066)
% (42, 0.00950899)
% (43, 0.0039345)
% (44, 0.00683592)
% (45, 0.00414528)
% (46, 0.00365827)
% (47, 0.0028239)
% (48, 0.00904182)
% (49, 0.0041073)
% (50, 0.00147132)
% (51, 0.00429213)
% (52, 0.00101824)
% (53, 0.0019889)
% (54, 0.00224657)
% (55, 0.000806807)
% (56, 0.00298757)
% (57, 0.000751194)
% (58, 0.000448623)
% (59, 0.000794366)
% (60, 0.000275731)
% (61, 0.000229023)
% (62, 0.000176023)
% (63, 0.000242796)
% (64, 6.87681e-05)
% (65, 8.32528e-05)
% (66, 0.000135616)
% (67, 0.00010832)
% (68, 3.24648e-05)
% (69, 8.43653e-05)
% (70, 9.00647e-05)
% (71, 3.00757e-05)
% (72, 1.50362e-05)
% (73, 3.28106e-05)
% (74, 6.20459e-05)
% (75, 3.77517e-05)
% (76, 4.49952e-06)
% (77, 7.73652e-06)
% (78, 2.0655e-05)
% (79, 1.04346e-05)
% (80, 8.31242e-06)
% (81, 2.00375e-06)
% (82, 3.58211e-06)
% (83, 7.26611e-06)
% (84, 5.00367e-06)
% (85, 7.27228e-06)
% (86, 7.46084e-06)
% (87, 1.67817e-06)
% (88, 9.52767e-07)
% (89, 6.00789e-07)
% (90, 2.21088e-07)
% (91, 2.7917e-07)
% (92, 2.82638e-07)
% (93, 3.63479e-07)
% (94, 5.41817e-07)
% (95, 5.13479e-07)
% (96, 3.57333e-07)
% (97, 1.70253e-07)
% (98, 8.46346e-08)
% (99, 9.40801e-08)
% (100, 6.41522e-08)
% (101, 1.7488e-08)
% (102, 1.24291e-08)
% (103, 4.51321e-09)
% (104, 2.23733e-09)
% (105, 2.68911e-09)
% (106, 2.77133e-09)
% (107, 3.05655e-09)
% (108, 3.99967e-09)
% (109, 2.37213e-09)
% (110, 3.5828e-09)
% (111, 3.68935e-09)
% (112, 3.50613e-09)
% (113, 1.12136e-09)
% (114, 8.00175e-10)
% (115, 9.80122e-10)
% (116, 3.76529e-10)
% (117, 3.70467e-10)
% (118, 2.89689e-10)
% (119, 1.71794e-10)
% (120, 2.11175e-10)
% (121, 1.72725e-10)
% (122, 8.82416e-11)
% (123, 4.759e-11)
% (124, 3.71699e-11)
% (125, 4.64163e-11)
% (126, 2.63991e-11)
% (127, 1.92699e-11)
% (128, 1.5229e-11)
% (129, 1.72683e-11)
% (130, 1.62099e-11)
% (131, 8.6646e-12)
% (132, 7.42057e-12)
% (133, 7.33623e-12)
% (134, 7.37386e-12)
% (135, 7.9615e-12)
% (136, 2.6926e-12)
% (137, 2.43451e-12)
% (138, 3.0619e-12)
% (139, 2.90125e-12)
% (140, 1.27562e-12)
% (141, 1.60201e-12)
% (142, 9.25888e-13)
% (143, 1.39656e-12)
% (144, 1.01663e-12)
% (145, 1.0473e-12)
% (146, 1.29135e-12)
% (147, 5.82413e-13)
% (148, 3.80601e-13)
% (149, 5.73252e-13)
% (150, 8.21565e-13)
% (151, 5.8919e-13)
% (152, 5.39434e-13)
% (153, 4.38976e-13)
% (154, 2.43588e-13)
% (155, 4.70821e-13)
% (156, 2.96737e-13)
% (157, 3.57564e-13)
% (158, 3.22161e-13)
% (159, 2.12568e-13)
% (160, 1.75343e-13)
% (161, 2.73254e-13)
% (162, 2.65438e-13)
% (163, 2.21546e-13)
% (164, 2.24956e-13)
% (165, 1.7846e-13)
% (166, 7.33365e-14)
% (167, 5.99124e-14)
% (168, 7.0894e-14)
% (169, 8.48821e-14)
% (170, 7.17963e-14)
% (171, 1.19149e-13)
% (172, 9.03653e-14)
% (173, 7.4583e-14)
% (174, 5.71332e-14)
% (175, 8.24286e-14)
% (176, 4.50838e-14)
% (177, 5.1195e-14)
% (178, 4.87292e-14)
% (179, 9.46202e-14)
% (180, 4.68576e-14)
% (181, 4.44655e-14)
% (182, 4.21978e-14)
% (183, 2.59111e-14)
% (184, 2.17692e-14)
% (185, 2.24272e-14)
% (186, 2.09745e-14)
% (187, 2.33031e-14)
% (188, 2.59556e-14)
% (189, 1.42257e-14)
% (190, 7.84177e-15)
% (191, 8.39489e-15)
% (192, 1.00154e-14)
% (193, 1.17224e-14)
% (194, 1.23003e-14)
% (195, 7.75723e-15)
% (196, 6.65531e-15)
% (197, 4.14033e-15)
% (198, 5.3884e-15)
% (199, 6.10848e-15)
% (200, 5.64641e-15)
% (201, 4.39101e-15)
% (202, 3.6561e-15)
% (203, 5.19736e-15)
% (204, 3.13052e-15)
% (205, 2.5566e-15)
% (206, 3.24783e-15)
% (207, 2.6717e-15)
% (208, 2.65072e-15)
% (209, 1.78354e-15)
% (210, 2.82879e-15)
% (211, 2.42135e-15)
% (212, 2.10747e-15)
% (213, 2.16354e-15)
% (214, 1.65687e-15)
% (215, 1.95477e-15)
% (216, 1.31659e-15)
% (217, 1.65111e-15)
% (218, 1.91972e-15)
% (219, 1.46285e-15)
% (220, 1.38231e-15)
% (221, 1.38001e-15)
% (222, 1.54607e-15)
% (223, 1.04e-15)
% (224, 9.3801e-16)
% }; \label{plot:limfp64mixed} 
% \addplot[ color=mygreen, line width=1.0pt] coordinates { 
% (0, 1)
% (1, 1.35449)
% (2, 1.72161)
% (3, 1.3746)
% (4, 1.56408)
% (5, 1.47247)
% (6, 1.03267)
% (7, 0.79666)
% (8, 0.76188)
% (9, 0.803019)
% (10, 0.856367)
% (11, 1.05548)
% (12, 0.986674)
% (13, 0.799058)
% (14, 0.686122)
% (15, 0.658931)
% (16, 0.555855)
% (17, 0.835282)
% (18, 0.525098)
% (19, 0.503206)
% (20, 0.511731)
% (21, 0.471179)
% (22, 0.359909)
% (23, 0.398003)
% (24, 0.276585)
% (25, 0.343557)
% (26, 0.252442)
% (27, 0.353291)
% (28, 0.250218)
% (29, 0.333288)
% (30, 0.171015)
% (31, 0.220342)
% (32, 0.150909)
% (33, 0.18838)
% (34, 0.171625)
% (35, 0.125478)
% (36, 0.135966)
% (37, 0.092676)
% (38, 0.0911455)
% (39, 0.124698)
% (40, 0.0856808)
% (41, 0.0879393)
% (42, 0.0676783)
% (43, 0.057637)
% (44, 0.059554)
% (45, 0.0369462)
% (46, 0.0552563)
% (47, 0.0573547)
% (48, 0.0504752)
% (49, 0.0396711)
% (50, 0.0623365)
% (51, 0.0209473)
% (52, 0.021263)
% (53, 0.027373)
% (54, 0.034562)
% (55, 0.014625)
% (56, 0.0321597)
% (57, 0.0169746)
% (58, 0.0197108)
% (59, 0.0117627)
% (60, 0.0239761)
% (61, 0.0160597)
% (62, 0.0127086)
% (63, 0.00633922)
% (64, 0.00516275)
% (65, 0.00747321)
% (66, 0.00652237)
% (67, 0.00543418)
% (68, 0.00739302)
% (69, 0.00522666)
% (70, 0.00759487)
% (71, 0.00859005)
% (72, 0.00445336)
% (73, 0.00408375)
% (74, 0.00437654)
% (75, 0.00510223)
% (76, 0.00559557)
% (77, 0.00525672)
% (78, 0.0039006)
% (79, 0.00267576)
% (80, 0.00203553)
% (81, 0.00284538)
% (82, 0.00287657)
% (83, 0.0031876)
% (84, 0.0034813)
% (85, 0.00201018)
% (86, 0.00247148)
% (87, 0.00141923)
% (88, 0.00200472)
% (89, 0.00115024)
% (90, 0.00181235)
% (91, 0.00125827)
% (92, 0.00115466)
% (93, 0.00163666)
% (94, 0.00128961)
% (95, 0.00151103)
% (96, 0.00143868)
% (97, 0.000639082)
% (98, 0.000520265)
% (99, 0.000462505)
% (100, 0.000771455)
% (101, 0.000473377)
% (102, 0.000533673)
% (103, 0.0003923)
% (104, 0.00024752)
% (105, 0.000256336)
% (106, 0.000393288)
% (107, 0.000223713)
% (108, 0.000205947)
% (109, 0.000204938)
% (110, 0.000116566)
% (111, 0.000123447)
% (112, 0.000211599)
% (113, 0.000215127)
% (114, 0.000201351)
% (115, 0.000113521)
% (116, 7.99613e-05)
% (117, 8.89445e-05)
% (118, 8.04486e-05)
% (119, 7.76465e-05)
% (120, 5.69798e-05)
% (121, 9.57134e-05)
% (122, 0.000118974)
% (123, 0.000120597)
% (124, 4.5609e-05)
% (125, 5.05896e-05)
% (126, 3.73725e-05)
% (127, 4.60444e-05)
% (128, 6.63658e-05)
% (129, 2.96693e-05)
% (130, 8.21217e-05)
% (131, 3.6182e-05)
% (132, 2.1627e-05)
% (133, 1.65675e-05)
% (134, 1.43217e-05)
% (135, 2.10879e-05)
% (136, 1.88883e-05)
% (137, 2.47689e-05)
% (138, 1.97525e-05)
% (139, 1.81461e-05)
% (140, 1.83754e-05)
% (141, 1.65738e-05)
% (142, 1.17616e-05)
% (143, 1.17058e-05)
% (144, 8.84278e-06)
% (145, 7.26865e-06)
% (146, 9.67847e-06)
% (147, 4.19395e-06)
% (148, 3.93514e-06)
% (149, 5.28759e-06)
% (150, 6.14985e-06)
% (151, 5.21056e-06)
% (152, 6.15798e-06)
% (153, 5.58854e-06)
% (154, 4.99701e-06)
% (155, 5.09522e-06)
% (156, 5.30754e-06)
% (157, 6.4326e-06)
% (158, 3.34386e-06)
% (159, 2.44671e-06)
% (160, 2.98648e-06)
% (161, 1.26502e-06)
% (162, 1.50556e-06)
% (163, 2.03363e-06)
% (164, 1.96658e-06)
% (165, 2.70508e-06)
% (166, 1.67441e-06)
% (167, 1.47575e-06)
% (168, 1.53333e-06)
% (169, 9.09025e-07)
% (170, 9.5476e-07)
% (171, 1.18216e-06)
% (172, 8.17361e-07)
% (173, 6.21266e-07)
% (174, 3.81e-07)
% (175, 4.4895e-07)
% (176, 2.45967e-07)
% (177, 1.89726e-07)
% (178, 1.82279e-07)
% (179, 1.87317e-07)
% (180, 1.94042e-07)
% (181, 1.49625e-07)
% (182, 1.99044e-07)
% (183, 2.77419e-07)
% (184, 3.05608e-07)
% (185, 1.67356e-07)
% (186, 1.38708e-07)
% (187, 2.75724e-07)
% (188, 1.94079e-07)
% (189, 1.05e-07)
% (190, 1.80575e-07)
% (191, 1.27623e-07)
% (192, 1.09529e-07)
% (193, 4.39748e-08)
% (194, 3.15073e-08)
% (195, 4.21929e-08)
% (196, 2.7284e-08)
% (197, 1.38711e-08)
% (198, 1.42183e-08)
% (199, 1.24809e-08)
% (200, 1.19202e-08)
% (201, 1.2347e-08)
% (202, 1.17079e-08)
% (203, 6.34357e-09)
% (204, 7.12973e-09)
% (205, 4.77183e-09)
% (206, 3.56286e-09)
% (207, 3.19966e-09)
% (208, 2.08974e-09)
% (209, 1.23095e-09)
% (210, 2.50736e-09)
% (211, 1.67682e-09)
% (212, 1.83072e-09)
% (213, 1.70764e-09)
% (214, 8.65584e-10)
% (215, 7.03239e-10)
% (216, 9.35205e-10)
% (217, 1.03239e-09)
% (218, 8.34687e-10)
% (219, 1.32992e-09)
% (220, 1.01916e-09)
% (221, 5.37952e-10)
% (222, 7.03646e-10)
% (223, 5.07242e-10)
% (224, 6.65146e-10)
% (225, 7.18646e-10)
% (226, 5.76114e-10)
% (227, 4.70029e-10)
% (228, 3.28612e-10)
% (229, 3.79084e-10)
% (230, 5.43018e-10)
% (231, 3.54815e-10)
% (232, 2.8187e-10)
% (233, 2.38794e-10)
% (234, 2.87181e-10)
% (235, 1.30937e-10)
% (236, 1.47846e-10)
% (237, 1.9459e-10)
% (238, 2.80858e-10)
% (239, 3.30241e-10)
% (240, 1.39744e-10)
% (241, 1.47042e-10)
% (242, 1.60052e-10)
% (243, 1.33762e-10)
% (244, 1.37379e-10)
% (245, 1.08811e-10)
% (246, 1.53531e-10)
% (247, 1.52901e-10)
% (248, 1.54692e-10)
% (249, 1.1996e-10)
% (250, 8.43736e-11)
% }; \label{plot:limfp16} 
% \addplot[ color=myrose, line width=1.0pt] coordinates { 
% (0, 1)
% (1, 1.35449)
% (2, 1.72138)
% (3, 1.37459)
% (4, 1.56375)
% (5, 1.47229)
% (6, 1.03221)
% (7, 0.796625)
% (8, 0.762054)
% (9, 0.803988)
% (10, 0.855695)
% (11, 1.05268)
% (12, 0.985007)
% (13, 0.791337)
% (14, 0.566758)
% (15, 0.497669)
% (16, 0.584098)
% (17, 0.467705)
% (18, 0.758682)
% (19, 0.464142)
% (20, 0.356665)
% (21, 0.371935)
% (22, 0.273895)
% (23, 0.23957)
% (24, 0.228406)
% (25, 0.313864)
% (26, 0.217307)
% (27, 0.279494)
% (28, 0.121241)
% (29, 0.135308)
% (30, 0.152182)
% (31, 0.1148)
% (32, 0.163875)
% (33, 0.0751979)
% (34, 0.12593)
% (35, 0.0562966)
% (36, 0.0868664)
% (37, 0.0833729)
% (38, 0.0354315)
% (39, 0.0415344)
% (40, 0.042634)
% (41, 0.0768386)
% (42, 0.025162)
% (43, 0.0197149)
% (44, 0.022468)
% (45, 0.0181166)
% (46, 0.0420535)
% (47, 0.0185712)
% (48, 0.0106952)
% (49, 0.0187317)
% (50, 0.0124416)
% (51, 0.00610744)
% (52, 0.00952927)
% (53, 0.00679976)
% (54, 0.00354644)
% (55, 0.0117204)
% (56, 0.00700677)
% (57, 0.00712419)
% (58, 0.00337938)
% (59, 0.00522598)
% (60, 0.00574043)
% (61, 0.00393432)
% (62, 0.00207312)
% (63, 0.00316331)
% (64, 0.00191007)
% (65, 0.00382683)
% (66, 0.00385044)
% (67, 0.00325236)
% (68, 0.00117879)
% (69, 0.00160352)
% (70, 0.00100501)
% (71, 0.00259058)
% (72, 0.00277274)
% (73, 0.000746201)
% (74, 0.00138197)
% (75, 0.000995612)
% (76, 0.000375139)
% (77, 0.000478717)
% (78, 0.000726969)
% (79, 0.000806299)
% (80, 0.000365915)
% (81, 0.000299821)
% (82, 0.000284672)
% (83, 0.000133811)
% (84, 0.000200434)
% (85, 0.000225185)
% (86, 0.000236819)
% (87, 0.000241558)
% (88, 0.000157842)
% (89, 4.92916e-05)
% (90, 9.24326e-05)
% (91, 8.94151e-05)
% (92, 0.00012741)
% (93, 7.26116e-05)
% (94, 3.69407e-05)
% (95, 8.08504e-05)
% (96, 4.31398e-05)
% (97, 6.69155e-05)
% (98, 8.3753e-05)
% (99, 4.29029e-05)
% (100, 1.82776e-05)
% (101, 2.32963e-05)
% (102, 1.6693e-05)
% (103, 2.00845e-05)
% (104, 2.87913e-05)
% (105, 1.64142e-05)
% (106, 6.98878e-06)
% (107, 4.83649e-06)
% (108, 5.00313e-06)
% (109, 1.21287e-05)
% (110, 8.30421e-06)
% (111, 6.44263e-06)
% (112, 1.12734e-05)
% (113, 1.58619e-06)
% (114, 3.28813e-06)
% (115, 2.76451e-06)
% (116, 3.73997e-06)
% (117, 3.90901e-06)
% (118, 4.61707e-06)
% (119, 1.69188e-06)
% (120, 5.83269e-07)
% (121, 5.71275e-07)
% (122, 7.10274e-07)
% (123, 5.53835e-07)
% (124, 2.17519e-07)
% (125, 1.53212e-07)
% (126, 2.06207e-07)
% (127, 5.06415e-07)
% (128, 4.69931e-07)
% (129, 3.04081e-07)
% (130, 2.66844e-07)
% (131, 1.7869e-07)
% (132, 2.55212e-07)
% (133, 9.68523e-08)
% (134, 6.79542e-08)
% (135, 2.9375e-08)
% (136, 2.22552e-08)
% (137, 1.26355e-08)
% (138, 7.78038e-09)
% (139, 5.64921e-09)
% (140, 3.02534e-09)
% (141, 3.10325e-09)
% (142, 2.78035e-09)
% (143, 1.43158e-09)
% (144, 2.0295e-09)
% (145, 1.07919e-09)
% (146, 2.34776e-09)
% (147, 2.04612e-09)
% (148, 1.12784e-09)
% (149, 9.49777e-10)
% (150, 3.13755e-09)
% (151, 9.83874e-10)
% (152, 9.24887e-10)
% (153, 3.66748e-10)
% (154, 1.53562e-10)
% (155, 2.51338e-10)
% (156, 2.06241e-10)
% (157, 6.98721e-11)
% (158, 5.0906e-11)
% (159, 5.50697e-11)
% (160, 2.03817e-11)
% (161, 2.37363e-11)
% (162, 1.47116e-11)
% (163, 8.48151e-12)
% (164, 8.2988e-12)
% (165, 4.98736e-12)
% (166, 9.47954e-12)
% (167, 5.28539e-12)
% (168, 2.86338e-12)
% (169, 2.85506e-12)
% (170, 4.78801e-13)
% (171, 5.95223e-13)
% (172, 7.64232e-13)
% (173, 2.69162e-13)
% (174, 1.6636e-13)
% (175, 2.05788e-13)
% (176, 1.3346e-13)
% (177, 3.00757e-13)
% (178, 2.22812e-13)
% (179, 2.87131e-13)
% (180, 1.021e-13)
% (181, 8.28719e-14)
% (182, 1.21785e-13)
% (183, 5.20633e-14)
% (184, 1.0953e-13)
% (185, 8.52485e-14)
% (186, 6.06138e-14)
% (187, 9.94026e-14)
% (188, 5.32656e-14)
% (189, 1.04229e-13)
% (190, 1.16735e-13)
% (191, 7.06134e-14)
% (192, 6.31019e-14)
% (193, 3.7897e-14)
% (194, 6.50583e-14)
% (195, 1.48538e-14)
% (196, 2.43749e-14)
% (197, 3.40179e-14)
% (198, 5.34092e-15)
% (199, 5.83198e-15)
% (200, 9.40161e-15)
% (201, 1.04374e-14)
% (202, 9.17088e-15)
% (203, 7.89554e-15)
% (204, 3.74548e-15)
% (205, 1.41086e-15)
% (206, 3.63439e-15)
% (207, 3.03786e-15)
% (208, 3.87024e-15)
% (209, 2.8472e-15)
% (210, 2.35064e-15)
% (211, 2.26502e-15)
% (212, 2.88165e-15)
% (213, 1.83418e-15)
% (214, 1.07338e-15)
% (215, 1.05915e-15)
% (216, 2.35483e-15)
% (217, 1.61826e-15)
% (218, 6.44838e-16)
% }; \label{plot:limfp32} 
% \addplot[only marks,  mark=o, color=red, mark size=3pt, line width=1.0pt] coordinates {
% (64, 6.87681e-05)

% }; \label{plot:limfp64tofp32}
% \addplot[only marks,  mark=o, color=black, mark size=3pt, line width=1.0pt] coordinates {
% (103, 4.51321e-09)
% };\label{plot:limfp32tofp16}


 

==> 5.Numerical/data/limitation_small_2.tex <==
\addplot[color=myyellow, line width=1.0pt] coordinates { 
(0, 1)
(1, 2.3012)
(2, 2.28146)
(3, 1.79871)
(4, 1.01498)
(5, 0.328493)
(6, 0.0535088)
(7, 0.00310962)
(8, 0.0151897)
(9, 3.84665e-05)
(10, 0.000151613)
(11, 6.39881e-08)
(12, 2.01771e-07)
(13, 3.86551e-11)
(14, 1.72787e-11)
(15, 5.82206e-16)
}; \label{plot:fp64} 
\addplot[color=mydeepblue, line width=1.0pt, dashed] coordinates { 
(0, 1)
(1, 2.3012)
(2, 2.28146)
(3, 1.79871)
(4, 1.01498)
(5, 0.328493)
(6, 0.0535088)
(7, 0.00310959)
(8, 0.0112055)
(9, 3.84597e-05)
(10, 3.85952e-05)
(11, 6.40507e-08)
(12, 2.09705e-07)
(13, 4.27006e-08)
(14, 6.64492e-10)
(15, 3.51187e-11)
(16, 7.84433e-11)
(17, 1.00014e-11)
(18, 5.52671e-11)
(19, 5.08799e-11)
(20, 1.32178e-11)
(21, 1.09088e-12)
(22, 7.91042e-13)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=x, color=red,  mark size=3pt,  line width=1.5pt] coordinates { 
 (9, 3.84597e-05) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=x, color=black,  mark size=3pt,  line width=1.5pt] coordinates { 
 (11, 6.40507e-08) 
}; \label{plot:fp32tofp16} 


==> 5.Numerical/data/limitation_small_res.tex <==
\addplot[color=myyellow, line width=1.0pt] coordinates { 
(0, 1)
(1, 2.42739)
(2, 2.33885)
(3, 1.70247)
(4, 0.73796)
(5, 0.150502)
(6, 0.012199)
(7, 0.000273788)
(8, 0.000399892)
(9, 1.99862e-06)
(10, 6.38657e-07)
(11, 7.57034e-09)
(12, 1.60939e-10)
(13, 1.22591e-09)
(14, 6.43777e-13)
(15, 1.64825e-15)
(16, 3.19866e-17)
(17, 3.59876e-20)
}; \label{plot:fp64} 
\addplot[color=mydeepblue, line width=1.0pt, dashed] coordinates { 
(0, 1)
(1, 2.42739)
(2, 2.33885)
(3, 1.70247)
(4, 0.73796)
(5, 0.150502)
(6, 0.012199)
(7, 0.00054297)
(8, 0.000248438)
(9, 9.40911e-06)
(10, 6.09629e-07)
(11, 5.04695e-09)
(12, 1.61098e-10)
(13, 2.4818e-09)
(14, 4.18053e-10)
(15, 7.64817e-14)
(16, 1.99646e-14)
(17, 1.24708e-15)
(18, 1.08134e-15)
(19, 2.32471e-16)
(20, 3.29979e-17)
(21, 5.06783e-17)
(22, 5.27112e-18)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=x, color=red,  mark size=3pt,  line width=1.5pt] coordinates { 
 (9, 9.40911e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=x, color=black,  mark size=3pt,  line width=1.5pt] coordinates { 
 (11, 5.04695e-09) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=o, color=blue,  mark size=3pt, line width=1.0pt] coordinates { 
 (11, 5.04695e-09) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/limitation_small_trueRes.tex <==
\addplot[color=myyellow, line width=1.0pt] coordinates { 
(0, 1)
(1, 2.42739)
(2, 2.33885)
(3, 1.70247)
(4, 0.73796)
(5, 0.150502)
(6, 0.012199)
(7, 0.000273788)
(8, 0.000399892)
(9, 1.99862e-06)
(10, 6.38657e-07)
(11, 7.57034e-09)
(12, 1.60939e-10)
(13, 1.22591e-09)
(14, 6.43817e-13)
(15, 1.6426e-15)
(16, 4.55056e-16)
(17, 4.55056e-16)
}; \label{plot:fp64} 
\addplot[color=mydeepblue, line width=1.0pt, dashed] coordinates { 
(0, 1)
(1, 2.42739)
(2, 2.33885)
(3, 1.70247)
(4, 0.73796)
(5, 0.150502)
(6, 0.012199)
(7, 0.00054297)
(8, 0.000248438)
(9, 9.40911e-06)
(10, 6.09629e-07)
(11, 5.04695e-09)
(12, 1.61098e-10)
(13, 2.4818e-09)
(14, 4.18053e-10)
(15, 7.62925e-14)
(16, 1.98711e-14)
(17, 1.12456e-15)
(18, 1.17337e-15)
(19, 3.66542e-16)
(20, 3.1205e-16)
(21, 3.34912e-16)
(22, 3.1205e-16)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=x, color=red,  mark size=3pt,  line width=1.5pt] coordinates { 
 (9, 9.40911e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=x, color=black,  mark size=3pt,  line width=1.5pt] coordinates { 
 (11, 5.04695e-09) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=o, color=blue,  mark size=3pt, line width=1.0pt] coordinates { 
 (11, 5.04695e-09) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/matrixCollection1.tex <==
\addplot[color=vtorange, line width=1.5pt] coordinates { 
(0, 1)
(1, 1.48544)
(2, 3.19641)
(3, 3.55056)
(4, 4.22653)
(5, 3.26341)
(6, 1.57429)
(7, 1.38719)
(8, 0.742365)
(9, 0.268803)
(10, 0.148026)
(11, 0.0494908)
(12, 0.0210536)
(13, 0.00908201)
(14, 0.00792442)
(15, 0.00246247)
(16, 0.00151582)
(17, 0.000553924)
(18, 0.000106187)
(19, 3.76011e-05)
(20, 6.86054e-06)
(21, 1.62399e-06)
(22, 2.77765e-07)
(23, 3.80358e-08)
(24, 5.98803e-09)
(25, 9.53028e-10)
(26, 8.11766e-11)
(27, 5.41671e-12)
(28, 5.67339e-13)
(29, 1.0045e-13)
(30, 3.93415e-14)
(31, 4.25637e-15)
(32, 8.52822e-15)
(33, 3.92619e-14)
(34, 5.32713e-15)
(35, 6.47145e-16)
}; \label{plot:fp64} 
\addplot[ color=mygreen, line width=1.5pt, dotted] coordinates { 
(0, 1)
(1, 1.48544)
(2, 3.41544)
(3, 4.79783)
(4, 5.81231)
(5, 5.97428)
(6, 2.7129)
(7, 2.6112)
(8, 1.22877)
(9, 0.472644)
(10, 0.262356)
(11, 0.103592)
(12, 0.029717)
(13, 0.039123)
(14, 0.013216)
(15, 0.009309)
(16, 0.00335305)
(17, 0.00156855)
(18, 0.000607346)
(19, 0.000650566)
(20, 0.00161987)
(21, 0.00277157)
(22, 0.00389179)
(23, 0.00159984)
(24, 0.000441143)
(25, 0.0003273)
(26, 0.000210753)
(27, 0.00011156)
(28, 5.29547e-05)
(29, 3.50424e-05)
(30, 1.59518e-05)
(31, 4.66102e-06)
(32, 2.10823e-06)
(33, 2.81717e-06)
(34, 1.27232e-06)
(35, 1.74492e-06)
(36, 4.96177e-06)
(37, 5.93087e-06)
(38, 6.09713e-06)
(39, 3.73131e-06)
(40, 8.63045e-07)
(41, 3.62199e-07)
(42, 2.31505e-07)
(43, 6.76673e-08)
(44, 4.21461e-08)
(45, 1.9635e-08)
(46, 1.6367e-08)
(47, 8.36901e-09)
(48, 4.51401e-09)
(49, 2.90422e-09)
(50, 3.33426e-09)
(51, 3.79086e-09)
(52, 6.87131e-09)
(53, 1.33391e-08)
(54, 8.37495e-09)
(55, 3.59773e-09)
(56, 3.67672e-09)
(57, 2.14513e-09)
(58, 8.14585e-10)
(59, 2.77848e-10)
(60, 1.21514e-10)
(61, 3.903e-11)
(62, 2.07515e-11)
(63, 9.69815e-12)
(64, 1.1191e-11)
(65, 1.0429e-11)
(66, 1.23237e-11)
(67, 2.09304e-11)
(68, 2.64932e-11)
(69, 2.63199e-11)
(70, 2.73746e-11)
(71, 1.35153e-11)
(72, 4.56384e-12)
(73, 2.16713e-12)
(74, 1.68362e-12)
(75, 6.65552e-13)
(76, 4.60253e-13)
(77, 3.41348e-13)
(78, 1.08528e-13)
(79, 6.93653e-14)
(80, 2.61441e-14)
(81, 3.75236e-14)
(82, 1.06798e-13)
(83, 1.41088e-13)
(84, 1.07212e-13)
(85, 6.08178e-14)
(86, 4.10055e-14)
(87, 2.50912e-14)
(88, 2.49196e-14)
(89, 6.07652e-15)
(90, 2.8643e-15)
(91, 1.49193e-15)
(92, 8.49618e-16)
}; \label{plot:fp16} 
\addplot[color=mydeepblue, line width=2.5pt, dashed] coordinates { 
(0, 1)
(1, 1.48544)
(2, 3.19641)
(3, 3.55056)
(4, 4.22653)
(5, 3.26341)
(6, 1.57429)
(7, 1.38719)
(8, 0.742365)
(9, 0.268803)
(10, 0.148026)
(11, 0.0494908)
(12, 0.0210536)
(13, 0.00908201)
(14, 0.00792442)
(15, 0.00246247)
(16, 0.00151582)
(17, 0.000553924)
(18, 0.000106187)
(19, 3.76011e-05)
(20, 6.86054e-06)
(21, 1.62399e-06)
(22, 2.77765e-07)
(23, 3.90977e-08)
(24, 6.10401e-09)
(25, 9.95606e-10)
(26, 1.12204e-10)
(27, 6.23616e-12)
(28, 1.47806e-12)
(29, 5.00466e-12)
(30, 4.03177e-12)
(31, 8.27799e-12)
(32, 1.25763e-11)
(33, 9.60429e-12)
(34, 8.21403e-12)
(35, 3.52992e-12)
(36, 8.6906e-13)
(37, 5.59268e-13)
(38, 2.44281e-13)
(39, 2.84806e-13)
(40, 1.07049e-13)
(41, 3.20835e-14)
(42, 1.6141e-14)
(43, 6.93642e-15)
(44, 4.31789e-15)
(45, 1.80072e-15)
(46, 3.17651e-15)
(47, 1.2819e-14)
(48, 9.16207e-15)
(49, 3.95881e-15)
(50, 3.15331e-15)
(51, 2.08914e-15)
(52, 1.01164e-15)
(53, 5.56637e-16)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=*, color=vtorange, mark options={ fill=vtorange}, line width=1.5pt] coordinates { 
 (19, 0.000106187) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=*, color=mygreen, mark options={ fill=mygreen}, line width=1.5pt] coordinates { 
 (22, 1.62399e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=square, color=vtmaroon, mark options={ fill=vtmaroon}, mark size=4pt, line width=1.0pt] coordinates { 
 (22, 1.62399e-06) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/matrixCollection2.tex <==
\addplot[color=vtorange, line width=1.5pt] coordinates { 
(0, 1)
(1, 0.778697)
(2, 0.579372)
(3, 0.450932)
(4, 0.0779467)
(5, 0.0102075)
(6, 0.00296766)
(7, 0.00100495)
(8, 0.000446799)
(9, 0.000145747)
(10, 7.32036e-05)
(11, 1.20748e-05)
(12, 4.62444e-06)
(13, 1.61959e-06)
(14, 2.6628e-07)
(15, 1.62551e-07)
(16, 6.77682e-08)
(17, 1.60565e-08)
(18, 2.67954e-09)
(19, 2.63787e-10)
(20, 4.50892e-11)
(21, 1.26607e-11)
(22, 2.18033e-12)
(23, 3.66116e-13)
(24, 6.15097e-14)
(25, 9.45616e-15)
(26, 1.77228e-15)
(27, 3.32928e-16)
}; \label{plot:fp64} 
\addplot[ color=mygreen, line width=1.5pt, dotted] coordinates { 
(0, 1)
(1, 0.778697)
(2, 0.580599)
(3, 0.45189)
(4, 0.0779708)
(5, 0.0102539)
(6, 0.00297672)
(7, 0.00100759)
(8, 0.000448808)
(9, 0.0001469)
(10, 7.38231e-05)
(11, 1.2151e-05)
(12, 4.6659e-06)
(13, 1.68096e-06)
(14, 3.94159e-07)
(15, 4.35559e-07)
(16, 2.10514e-07)
(17, 1.16965e-07)
(18, 6.39305e-08)
(19, 1.59286e-08)
(20, 1.86377e-09)
(21, 2.24629e-10)
(22, 5.8476e-11)
(23, 1.10942e-11)
(24, 2.42076e-12)
(25, 6.50737e-13)
(26, 7.60616e-13)
(27, 3.48973e-13)
(28, 7.62558e-14)
(29, 3.64019e-14)
(30, 1.49054e-14)
(31, 5.57454e-15)
(32, 1.74222e-15)
(33, 4.57204e-16)
}; \label{plot:fp16} 
\addplot[color=mydeepblue, line width=2.5pt, dashed] coordinates { 
(0, 1)
(1, 0.778697)
(2, 0.579372)
(3, 0.450932)
(4, 0.0779467)
(5, 0.0102075)
(6, 0.00296766)
(7, 0.00100495)
(8, 0.000446799)
(9, 0.000145747)
(10, 7.32036e-05)
(11, 1.20748e-05)
(12, 4.62444e-06)
(13, 1.61959e-06)
(14, 2.6628e-07)
(15, 1.62565e-07)
(16, 6.78385e-08)
(17, 1.60919e-08)
(18, 2.68229e-09)
(19, 2.64267e-10)
(20, 4.51339e-11)
(21, 1.26937e-11)
(22, 2.195e-12)
(23, 3.79064e-13)
(24, 1.13248e-13)
(25, 1.02301e-13)
(26, 5.032e-14)
(27, 2.84082e-14)
(28, 1.52962e-14)
(29, 2.80463e-15)
(30, 8.77621e-16)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=*, color=vtorange, mark options={ fill=vtorange}, line width=1.5pt] coordinates { 
 (10, 0.000145747) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=*, color=mygreen, mark options={ fill=mygreen}, line width=1.5pt] coordinates { 
 (14, 1.61959e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=square,  mark size=4pt, color=vtmaroon, mark options={ fill=vtmaroon}, line width=1.0pt] coordinates { 
 (14, 1.61959e-06) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/matrixCollection3.tex <==
\addplot[color=vtorange, line width=1.5pt] coordinates { 
(0, 1)
(1, 1.42637)
(2, 0.878305)
(3, 0.660423)
(4, 0.621626)
(5, 0.617083)
(6, 0.444714)
(7, 0.3016)
(8, 0.236347)
(9, 0.261193)
(10, 0.352013)
(11, 0.297942)
(12, 0.28825)
(13, 0.287969)
(14, 0.33694)
(15, 0.370409)
(16, 0.407543)
(17, 0.420782)
(18, 0.539186)
(19, 0.542635)
(20, 0.542156)
(21, 0.409052)
(22, 0.363244)
(23, 0.476827)
(24, 0.467993)
(25, 0.369677)
(26, 0.261651)
(27, 0.231202)
(28, 0.20573)
(29, 0.215601)
(30, 0.207284)
(31, 0.197114)
(32, 0.19343)
(33, 0.225947)
(34, 0.219554)
(35, 0.216848)
(36, 0.213816)
(37, 0.179577)
(38, 0.168588)
(39, 0.177722)
(40, 0.20091)
(41, 0.245376)
(42, 0.307874)
(43, 0.343784)
(44, 0.3239)
(45, 0.310015)
(46, 0.381407)
(47, 0.394666)
(48, 0.412247)
(49, 0.414696)
(50, 0.350553)
(51, 0.28652)
(52, 0.347155)
(53, 0.356346)
(54, 0.432601)
(55, 0.420322)
(56, 0.403148)
(57, 0.353494)
(58, 0.290692)
(59, 0.336153)
(60, 0.314811)
(61, 0.304414)
(62, 0.262099)
(63, 0.219692)
(64, 0.161287)
(65, 0.150513)
(66, 0.144207)
(67, 0.145611)
(68, 0.157899)
(69, 0.173957)
(70, 0.185294)
(71, 0.158717)
(72, 0.141262)
(73, 0.149172)
(74, 0.15941)
(75, 0.141312)
(76, 0.134768)
(77, 0.12582)
(78, 0.11699)
(79, 0.124224)
(80, 0.121435)
(81, 0.100634)
(82, 0.0902935)
(83, 0.0932379)
(84, 0.0905371)
(85, 0.0865168)
(86, 0.0786874)
(87, 0.0771799)
(88, 0.0790719)
(89, 0.0922611)
(90, 0.123265)
(91, 0.149412)
(92, 0.162163)
(93, 0.192384)
(94, 0.159813)
(95, 0.127276)
(96, 0.105846)
(97, 0.102336)
(98, 0.0851896)
(99, 0.0702177)
(100, 0.06678)
(101, 0.0729973)
(102, 0.0579428)
(103, 0.0652762)
(104, 0.0623484)
(105, 0.0610203)
(106, 0.0746428)
(107, 0.0919592)
(108, 0.0959937)
(109, 0.132104)
(110, 0.142923)
(111, 0.153966)
(112, 0.161779)
(113, 0.150666)
(114, 0.143432)
(115, 0.116784)
(116, 0.108386)
(117, 0.10972)
(118, 0.113533)
(119, 0.113555)
(120, 0.0966089)
(121, 0.0930293)
(122, 0.0828717)
(123, 0.0742513)
(124, 0.0675264)
(125, 0.0580481)
(126, 0.0584521)
(127, 0.0463781)
(128, 0.0389031)
(129, 0.0305147)
(130, 0.0274424)
(131, 0.0233545)
(132, 0.0193726)
(133, 0.0202562)
(134, 0.0188696)
(135, 0.0195995)
(136, 0.020403)
(137, 0.0243228)
(138, 0.0235843)
(139, 0.0244297)
(140, 0.0267226)
(141, 0.0304593)
(142, 0.0388173)
(143, 0.0434623)
(144, 0.0493787)
(145, 0.0451681)
(146, 0.0367089)
(147, 0.02356)
(148, 0.0163057)
(149, 0.0118964)
(150, 0.00876251)
(151, 0.00818986)
(152, 0.00970798)
(153, 0.0111386)
(154, 0.01373)
(155, 0.0160522)
(156, 0.0177938)
(157, 0.0190229)
(158, 0.0242091)
(159, 0.0293)
(160, 0.0375718)
(161, 0.0332539)
(162, 0.0288242)
(163, 0.0237145)
(164, 0.0188621)
(165, 0.015623)
(166, 0.0123549)
(167, 0.0100467)
(168, 0.00788753)
(169, 0.0057471)
(170, 0.00544758)
(171, 0.00622627)
(172, 0.00736818)
(173, 0.00857822)
(174, 0.00884979)
(175, 0.00861999)
(176, 0.00907043)
(177, 0.0115219)
(178, 0.0140396)
(179, 0.01733)
(180, 0.0211218)
(181, 0.0202344)
(182, 0.0174074)
(183, 0.0142901)
(184, 0.0100696)
(185, 0.00742962)
(186, 0.00487273)
(187, 0.00344434)
(188, 0.00206944)
(189, 0.00148136)
(190, 0.00108805)
(191, 0.000778848)
(192, 0.00053916)
(193, 0.000403605)
(194, 0.000373124)
(195, 0.000380614)
(196, 0.000342803)
(197, 0.000334842)
(198, 0.000378981)
(199, 0.000437651)
(200, 0.000610479)
(201, 0.000784919)
(202, 0.00110406)
(203, 0.00157208)
(204, 0.00202965)
(205, 0.00267034)
(206, 0.00301075)
(207, 0.00305877)
(208, 0.00252005)
(209, 0.0019307)
(210, 0.00121207)
(211, 0.000826942)
(212, 0.000476651)
(213, 0.000272348)
(214, 0.000150423)
(215, 7.85885e-05)
(216, 4.16448e-05)
(217, 2.52592e-05)
(218, 1.42849e-05)
(219, 9.28334e-06)
(220, 5.73277e-06)
(221, 3.37778e-06)
(222, 2.01789e-06)
(223, 1.23495e-06)
(224, 7.0438e-07)
(225, 4.75967e-07)
(226, 3.40695e-07)
(227, 2.23559e-07)
(228, 1.35799e-07)
(229, 8.82757e-08)
(230, 6.25414e-08)
(231, 4.00625e-08)
(232, 2.31393e-08)
(233, 1.38716e-08)
(234, 8.68004e-09)
(235, 5.13065e-09)
(236, 2.727e-09)
(237, 1.5594e-09)
(238, 1.007e-09)
(239, 6.20397e-10)
(240, 3.98772e-10)
(241, 2.5144e-10)
(242, 1.83547e-10)
(243, 1.22309e-10)
(244, 9.87599e-11)
(245, 7.54893e-11)
(246, 6.26785e-11)
(247, 6.65325e-11)
(248, 7.93887e-11)
(249, 8.85705e-11)
(250, 9.50496e-11)
(251, 8.14002e-11)
(252, 5.4589e-11)
(253, 3.63676e-11)
(254, 2.2133e-11)
(255, 1.18433e-11)
(256, 7.82188e-12)
(257, 5.10906e-12)
(258, 4.2293e-12)
(259, 3.78278e-12)
(260, 4.77716e-12)
(261, 6.21967e-12)
(262, 8.0469e-12)
(263, 7.21452e-12)
(264, 4.34059e-12)
(265, 2.69378e-12)
(266, 2.01244e-12)
(267, 1.7777e-12)
(268, 1.93186e-12)
(269, 2.32327e-12)
(270, 3.04402e-12)
(271, 3.05196e-12)
(272, 2.16781e-12)
(273, 1.48904e-12)
(274, 9.68105e-13)
(275, 6.50085e-13)
(276, 4.79628e-13)
(277, 3.82155e-13)
(278, 3.93799e-13)
(279, 4.32508e-13)
(280, 4.40164e-13)
(281, 3.61967e-13)
(282, 2.62953e-13)
(283, 1.71465e-13)
(284, 1.07516e-13)
(285, 6.31207e-14)
(286, 3.80317e-14)
(287, 3.07385e-14)
(288, 4.0996e-14)
(289, 4.23888e-14)
(290, 4.93218e-14)
(291, 4.28644e-14)
(292, 2.54029e-14)
(293, 1.6902e-14)
(294, 1.19613e-14)
(295, 9.21322e-15)
(296, 9.48137e-15)
(297, 1.42753e-14)
(298, 1.92204e-14)
(299, 2.15847e-14)
(300, 1.66954e-14)
(301, 1.33153e-14)
(302, 1.2645e-14)
(303, 1.57773e-14)
(304, 2.25591e-14)
(305, 2.6455e-14)
(306, 2.30269e-14)
(307, 1.55234e-14)
(308, 9.32963e-15)
(309, 7.24848e-15)
(310, 4.82443e-15)
(311, 4.49608e-15)
(312, 4.80282e-15)
(313, 4.70019e-15)
(314, 3.59977e-15)
(315, 2.7856e-15)
(316, 1.96989e-15)
(317, 2.00102e-15)
(318, 2.36377e-15)
(319, 4.32818e-15)
(320, 7.28592e-15)
(321, 1.04897e-14)
(322, 1.12115e-14)
(323, 8.90897e-15)
(324, 6.44847e-15)
(325, 4.48751e-15)
(326, 2.98667e-15)
(327, 2.46442e-15)
(328, 3.06384e-15)
(329, 2.87023e-15)
(330, 2.20228e-15)
(331, 1.71824e-15)
(332, 2.1662e-15)
(333, 3.30381e-15)
(334, 4.63403e-15)
(335, 5.95717e-15)
(336, 5.37669e-15)
(337, 5.34957e-15)
(338, 4.2811e-15)
(339, 4.78924e-15)
(340, 5.55215e-15)
(341, 5.67908e-15)
(342, 5.20443e-15)
(343, 3.64818e-15)
(344, 2.56908e-15)
(345, 2.07954e-15)
(346, 1.96437e-15)
(347, 1.6823e-15)
(348, 1.36815e-15)
(349, 1.03975e-15)
(350, 7.86172e-16)
}; \label{plot:fp64} 
\addplot[ color=mygreen, line width=1.5pt, dotted] coordinates { 
(0, 1)
(1, 1.42637)
(2, 0.878307)
(3, 0.660887)
(4, 0.623283)
(5, 0.618855)
(6, 0.445565)
(7, 0.30116)
(8, 0.236006)
(9, 0.261402)
(10, 0.352634)
(11, 0.298786)
(12, 0.289633)
(13, 0.288953)
(14, 0.337607)
(15, 0.368303)
(16, 0.404125)
(17, 0.417083)
(18, 0.533332)
(19, 0.538878)
(20, 0.540553)
(21, 0.408687)
(22, 0.360587)
(23, 0.470801)
(24, 0.462375)
(25, 0.36646)
(26, 0.260727)
(27, 0.230126)
(28, 0.203112)
(29, 0.212649)
(30, 0.203857)
(31, 0.194616)
(32, 0.190238)
(33, 0.224395)
(34, 0.220496)
(35, 0.216509)
(36, 0.209771)
(37, 0.178901)
(38, 0.168335)
(39, 0.176294)
(40, 0.200458)
(41, 0.241412)
(42, 0.301184)
(43, 0.338061)
(44, 0.32249)
(45, 0.325061)
(46, 0.398813)
(47, 0.403455)
(48, 0.41255)
(49, 0.421946)
(50, 0.353297)
(51, 0.294528)
(52, 0.343042)
(53, 0.357927)
(54, 0.426865)
(55, 0.402068)
(56, 0.404711)
(57, 0.355707)
(58, 0.296065)
(59, 0.351443)
(60, 0.34828)
(61, 0.311596)
(62, 0.283169)
(63, 0.221355)
(64, 0.174176)
(65, 0.158367)
(66, 0.139721)
(67, 0.146986)
(68, 0.159777)
(69, 0.172325)
(70, 0.181094)
(71, 0.162666)
(72, 0.145112)
(73, 0.152674)
(74, 0.167388)
(75, 0.142805)
(76, 0.144019)
(77, 0.130304)
(78, 0.120645)
(79, 0.116413)
(80, 0.123547)
(81, 0.107886)
(82, 0.093208)
(83, 0.0905465)
(84, 0.0983509)
(85, 0.0858526)
(86, 0.0837765)
(87, 0.076961)
(88, 0.0811588)
(89, 0.0837728)
(90, 0.118591)
(91, 0.140036)
(92, 0.14867)
(93, 0.171326)
(94, 0.177759)
(95, 0.136495)
(96, 0.125348)
(97, 0.106921)
(98, 0.100353)
(99, 0.082458)
(100, 0.0697646)
(101, 0.0710792)
(102, 0.0694833)
(103, 0.0562643)
(104, 0.0657892)
(105, 0.0615676)
(106, 0.0639323)
(107, 0.0811637)
(108, 0.0961141)
(109, 0.105999)
(110, 0.144119)
(111, 0.145987)
(112, 0.160597)
(113, 0.161972)
(114, 0.14886)
(115, 0.137871)
(116, 0.113084)
(117, 0.114525)
(118, 0.117612)
(119, 0.124305)
(120, 0.11737)
(121, 0.0971443)
(122, 0.0978534)
(123, 0.0873749)
(124, 0.0777181)
(125, 0.068251)
(126, 0.0618016)
(127, 0.0610746)
(128, 0.0520452)
(129, 0.0421089)
(130, 0.0323474)
(131, 0.0296059)
(132, 0.0254351)
(133, 0.0225026)
(134, 0.0198388)
(135, 0.0212186)
(136, 0.0190033)
(137, 0.0200296)
(138, 0.0225404)
(139, 0.0264495)
(140, 0.0257329)
(141, 0.0259003)
(142, 0.0282943)
(143, 0.036159)
(144, 0.0434346)
(145, 0.0477672)
(146, 0.0537776)
(147, 0.0447276)
(148, 0.0336107)
(149, 0.0231863)
(150, 0.0153256)
(151, 0.0112328)
(152, 0.00938301)
(153, 0.00857272)
(154, 0.010607)
(155, 0.0123345)
(156, 0.0144695)
(157, 0.0172131)
(158, 0.0178444)
(159, 0.0203521)
(160, 0.0242631)
(161, 0.0287844)
(162, 0.0363654)
(163, 0.0368834)
(164, 0.0297856)
(165, 0.0247557)
(166, 0.0204965)
(167, 0.0175079)
(168, 0.01508)
(169, 0.0128131)
(170, 0.011223)
(171, 0.00947307)
(172, 0.00891168)
(173, 0.0105245)
(174, 0.0123284)
(175, 0.012366)
(176, 0.0111097)
(177, 0.00940878)
(178, 0.00794735)
(179, 0.0079161)
(180, 0.00912962)
(181, 0.00978485)
(182, 0.0105894)
(183, 0.010532)
(184, 0.00913995)
(185, 0.00839014)
(186, 0.00871035)
(187, 0.00910605)
(188, 0.0104233)
(189, 0.012407)
(190, 0.0125574)
(191, 0.0142031)
(192, 0.0146389)
(193, 0.0145421)
(194, 0.0110798)
(195, 0.00979813)
(196, 0.00899575)
(197, 0.00867178)
(198, 0.00824992)
(199, 0.00835608)
(200, 0.00866848)
(201, 0.00896887)
(202, 0.00755835)
(203, 0.00548216)
(204, 0.00431436)
(205, 0.00325346)
(206, 0.00274349)
(207, 0.00251936)
(208, 0.00240135)
(209, 0.00239041)
(210, 0.00230297)
(211, 0.00204119)
(212, 0.00194104)
(213, 0.00176818)
(214, 0.00167027)
(215, 0.00140477)
(216, 0.00123115)
(217, 0.00119992)
(218, 0.00113575)
(219, 0.00102291)
(220, 0.00105256)
(221, 0.00110065)
(222, 0.0010492)
(223, 0.00106737)
(224, 0.000915774)
(225, 0.00100547)
(226, 0.00101933)
(227, 0.000941211)
(228, 0.000772909)
(229, 0.000497339)
(230, 0.000352375)
(231, 0.000296391)
(232, 0.000327262)
(233, 0.000425225)
(234, 0.000598172)
(235, 0.000741828)
(236, 0.000827292)
(237, 0.000886195)
(238, 0.000925108)
(239, 0.000934018)
(240, 0.00100253)
(241, 0.0011767)
(242, 0.00142072)
(243, 0.00147191)
(244, 0.00136447)
(245, 0.0014375)
(246, 0.00164299)
(247, 0.00167948)
(248, 0.00188161)
(249, 0.00196727)
(250, 0.00158704)
(251, 0.0012561)
(252, 0.00117172)
(253, 0.00112743)
(254, 0.00109763)
(255, 0.00123599)
(256, 0.00107507)
(257, 0.000998674)
(258, 0.000802647)
(259, 0.000540418)
(260, 0.000370174)
(261, 0.000281446)
(262, 0.000227757)
(263, 0.000189322)
(264, 0.000174545)
(265, 0.000140637)
(266, 0.000103818)
(267, 8.42344e-05)
(268, 5.84647e-05)
(269, 5.1752e-05)
(270, 4.90923e-05)
(271, 5.97698e-05)
(272, 6.34291e-05)
(273, 6.78775e-05)
(274, 7.50931e-05)
(275, 7.86991e-05)
(276, 9.3312e-05)
(277, 0.000102461)
(278, 0.000106695)
(279, 0.000113979)
(280, 0.000112734)
(281, 8.80885e-05)
(282, 6.55745e-05)
(283, 5.45173e-05)
(284, 4.80152e-05)
(285, 3.42336e-05)
(286, 2.06361e-05)
(287, 1.44687e-05)
(288, 1.2856e-05)
(289, 1.30128e-05)
(290, 1.48284e-05)
(291, 1.68487e-05)
(292, 2.08193e-05)
(293, 2.18814e-05)
(294, 1.90255e-05)
(295, 1.55109e-05)
(296, 1.21603e-05)
(297, 1.18046e-05)
(298, 1.23168e-05)
(299, 1.47437e-05)
(300, 1.71382e-05)
(301, 1.88832e-05)
(302, 1.87031e-05)
(303, 1.58788e-05)
(304, 1.42463e-05)
(305, 1.81866e-05)
(306, 2.01108e-05)
(307, 2.28959e-05)
(308, 2.52592e-05)
(309, 2.43201e-05)
(310, 2.16978e-05)
(311, 2.11459e-05)
(312, 2.19453e-05)
(313, 1.83287e-05)
(314, 1.76873e-05)
(315, 1.55244e-05)
(316, 1.35104e-05)
(317, 1.38365e-05)
(318, 1.49381e-05)
(319, 1.44879e-05)
(320, 1.22932e-05)
(321, 1.02937e-05)
(322, 1.00179e-05)
(323, 1.11471e-05)
(324, 1.33383e-05)
(325, 1.48698e-05)
(326, 1.56999e-05)
(327, 1.7438e-05)
(328, 1.54648e-05)
(329, 1.8147e-05)
(330, 1.82187e-05)
(331, 1.9197e-05)
(332, 2.08936e-05)
(333, 2.15713e-05)
(334, 2.04734e-05)
(335, 2.0996e-05)
(336, 1.82513e-05)
(337, 2.0149e-05)
(338, 1.7123e-05)
(339, 1.51081e-05)
(340, 1.49571e-05)
(341, 1.59596e-05)
(342, 1.54184e-05)
(343, 1.4158e-05)
(344, 1.26788e-05)
(345, 1.08594e-05)
(346, 9.83671e-06)
(347, 7.93662e-06)
(348, 5.93834e-06)
(349, 4.85914e-06)
(350, 3.7385e-06)
(351, 3.59985e-06)
(352, 4.52355e-06)
(353, 5.32614e-06)
(354, 4.27346e-06)
(355, 3.28371e-06)
(356, 3.29867e-06)
(357, 3.52539e-06)
(358, 4.13437e-06)
(359, 4.21449e-06)
(360, 5.91037e-06)
(361, 7.8565e-06)
(362, 9.0793e-06)
(363, 8.22353e-06)
(364, 7.57779e-06)
(365, 6.16397e-06)
(366, 4.83229e-06)
(367, 4.13657e-06)
(368, 4.21314e-06)
(369, 4.98851e-06)
(370, 6.36829e-06)
(371, 7.01762e-06)
(372, 6.44678e-06)
(373, 6.51106e-06)
(374, 8.27091e-06)
(375, 1.1152e-05)
(376, 1.31792e-05)
(377, 1.40733e-05)
(378, 1.33447e-05)
(379, 1.20787e-05)
(380, 1.06686e-05)
(381, 8.55552e-06)
(382, 6.86539e-06)
(383, 6.22106e-06)
(384, 5.37399e-06)
(385, 3.73546e-06)
(386, 2.64807e-06)
(387, 2.37184e-06)
(388, 2.47947e-06)
(389, 2.44992e-06)
(390, 1.94264e-06)
(391, 1.47297e-06)
(392, 1.48866e-06)
(393, 1.60005e-06)
(394, 1.47349e-06)
(395, 2.03807e-06)
(396, 2.98431e-06)
(397, 3.89868e-06)
(398, 3.86704e-06)
(399, 3.51374e-06)
(400, 4.18958e-06)
(401, 4.79769e-06)
(402, 3.98423e-06)
(403, 2.75376e-06)
(404, 2.29154e-06)
(405, 2.10954e-06)
(406, 2.34872e-06)
(407, 2.89349e-06)
(408, 3.16474e-06)
(409, 2.88608e-06)
(410, 2.04011e-06)
(411, 1.50348e-06)
(412, 1.30336e-06)
(413, 1.25457e-06)
(414, 1.24656e-06)
(415, 1.11526e-06)
(416, 9.84654e-07)
(417, 9.8154e-07)
(418, 8.83463e-07)
(419, 1.03935e-06)
(420, 1.05292e-06)
(421, 1.01618e-06)
(422, 9.94472e-07)
(423, 9.28879e-07)
(424, 9.89384e-07)
(425, 1.19782e-06)
(426, 1.45517e-06)
(427, 1.54025e-06)
(428, 2.11901e-06)
(429, 2.41914e-06)
(430, 2.3806e-06)
(431, 2.23184e-06)
(432, 2.08887e-06)
(433, 2.31171e-06)
(434, 1.93589e-06)
(435, 1.45848e-06)
(436, 1.28518e-06)
(437, 1.15959e-06)
(438, 1.10025e-06)
(439, 9.63197e-07)
(440, 1.02538e-06)
(441, 1.34724e-06)
(442, 1.31627e-06)
(443, 9.68645e-07)
(444, 8.60283e-07)
(445, 8.8598e-07)
(446, 8.02698e-07)
(447, 7.68557e-07)
(448, 7.92004e-07)
(449, 7.71474e-07)
(450, 6.99197e-07)
(451, 7.58646e-07)
(452, 9.31563e-07)
(453, 9.91237e-07)
(454, 1.10131e-06)
(455, 1.3748e-06)
(456, 1.49178e-06)
(457, 1.26788e-06)
(458, 1.08756e-06)
(459, 9.41444e-07)
(460, 8.2176e-07)
(461, 7.08501e-07)
(462, 7.57516e-07)
(463, 7.34264e-07)
(464, 6.61892e-07)
(465, 6.27117e-07)
(466, 6.19641e-07)
(467, 6.14585e-07)
(468, 5.87825e-07)
(469, 4.42015e-07)
(470, 3.0831e-07)
(471, 2.80765e-07)
(472, 2.89912e-07)
(473, 2.76438e-07)
(474, 2.60482e-07)
(475, 2.16321e-07)
(476, 2.02164e-07)
(477, 1.90005e-07)
(478, 1.70758e-07)
(479, 1.19111e-07)
(480, 1.154e-07)
(481, 1.14897e-07)
(482, 9.79064e-08)
(483, 8.01558e-08)
(484, 6.34247e-08)
(485, 4.64065e-08)
(486, 2.75418e-08)
(487, 2.24537e-08)
(488, 1.9977e-08)
(489, 1.95282e-08)
(490, 1.66583e-08)
(491, 1.44143e-08)
(492, 1.44726e-08)
(493, 1.36082e-08)
(494, 1.33437e-08)
(495, 1.54354e-08)
(496, 1.56856e-08)
(497, 1.75822e-08)
(498, 2.31536e-08)
(499, 2.88418e-08)
(500, 2.98759e-08)
}; \label{plot:fp16} 
\addplot[color=mydeepblue, line width=2.5pt, dashed] coordinates { 
(0, 1)
(1, 1.42637)
(2, 0.878305)
(3, 0.660423)
(4, 0.621626)
(5, 0.617083)
(6, 0.444714)
(7, 0.3016)
(8, 0.236347)
(9, 0.261193)
(10, 0.352013)
(11, 0.297942)
(12, 0.28825)
(13, 0.287969)
(14, 0.33694)
(15, 0.370409)
(16, 0.407543)
(17, 0.420782)
(18, 0.539186)
(19, 0.542635)
(20, 0.542156)
(21, 0.409052)
(22, 0.363244)
(23, 0.476827)
(24, 0.467993)
(25, 0.369677)
(26, 0.261651)
(27, 0.231202)
(28, 0.20573)
(29, 0.215601)
(30, 0.207284)
(31, 0.197114)
(32, 0.19343)
(33, 0.225947)
(34, 0.219554)
(35, 0.216848)
(36, 0.213816)
(37, 0.179577)
(38, 0.168588)
(39, 0.177722)
(40, 0.20091)
(41, 0.245376)
(42, 0.307874)
(43, 0.343784)
(44, 0.3239)
(45, 0.310015)
(46, 0.381407)
(47, 0.394666)
(48, 0.412247)
(49, 0.414696)
(50, 0.350553)
(51, 0.28652)
(52, 0.347155)
(53, 0.356346)
(54, 0.432601)
(55, 0.420322)
(56, 0.403148)
(57, 0.353494)
(58, 0.290692)
(59, 0.336153)
(60, 0.314811)
(61, 0.304414)
(62, 0.262099)
(63, 0.219692)
(64, 0.161287)
(65, 0.150513)
(66, 0.144207)
(67, 0.145611)
(68, 0.157899)
(69, 0.173957)
(70, 0.185294)
(71, 0.158717)
(72, 0.141262)
(73, 0.149172)
(74, 0.15941)
(75, 0.141312)
(76, 0.134768)
(77, 0.12582)
(78, 0.11699)
(79, 0.124224)
(80, 0.121435)
(81, 0.100634)
(82, 0.0902935)
(83, 0.0932379)
(84, 0.0905371)
(85, 0.0865168)
(86, 0.0786874)
(87, 0.0771799)
(88, 0.0790719)
(89, 0.0922611)
(90, 0.123265)
(91, 0.149412)
(92, 0.162163)
(93, 0.192384)
(94, 0.159813)
(95, 0.127276)
(96, 0.105846)
(97, 0.102336)
(98, 0.0851896)
(99, 0.0702177)
(100, 0.06678)
(101, 0.0729973)
(102, 0.0579428)
(103, 0.0652762)
(104, 0.0623484)
(105, 0.0610203)
(106, 0.0746428)
(107, 0.0919592)
(108, 0.0959937)
(109, 0.132104)
(110, 0.142923)
(111, 0.153966)
(112, 0.161779)
(113, 0.150666)
(114, 0.143432)
(115, 0.116784)
(116, 0.108386)
(117, 0.10972)
(118, 0.113533)
(119, 0.113555)
(120, 0.0966089)
(121, 0.0930293)
(122, 0.0828717)
(123, 0.0742513)
(124, 0.0675264)
(125, 0.0580481)
(126, 0.0584521)
(127, 0.0463781)
(128, 0.0389031)
(129, 0.0305147)
(130, 0.0274424)
(131, 0.0233545)
(132, 0.0193726)
(133, 0.0202562)
(134, 0.0188696)
(135, 0.0195995)
(136, 0.020403)
(137, 0.0243228)
(138, 0.0235843)
(139, 0.0244297)
(140, 0.0267226)
(141, 0.0304593)
(142, 0.0388173)
(143, 0.0434623)
(144, 0.0493787)
(145, 0.0451681)
(146, 0.0367089)
(147, 0.02356)
(148, 0.0163057)
(149, 0.0118964)
(150, 0.0087625)
(151, 0.00818985)
(152, 0.00970797)
(153, 0.0111386)
(154, 0.01373)
(155, 0.0160522)
(156, 0.0177937)
(157, 0.0190229)
(158, 0.0242091)
(159, 0.0292999)
(160, 0.0375718)
(161, 0.0332539)
(162, 0.0288241)
(163, 0.0237145)
(164, 0.0188621)
(165, 0.015623)
(166, 0.0123549)
(167, 0.0100467)
(168, 0.0078875)
(169, 0.00574708)
(170, 0.00544755)
(171, 0.00622625)
(172, 0.00736812)
(173, 0.00857812)
(174, 0.00884982)
(175, 0.00861998)
(176, 0.00907049)
(177, 0.011522)
(178, 0.0140397)
(179, 0.0173298)
(180, 0.0211215)
(181, 0.0202338)
(182, 0.0174071)
(183, 0.0142898)
(184, 0.0100694)
(185, 0.007429)
(186, 0.00487183)
(187, 0.00344402)
(188, 0.00206888)
(189, 0.00148059)
(190, 0.00108746)
(191, 0.000778097)
(192, 0.000538539)
(193, 0.000403058)
(194, 0.000372466)
(195, 0.000379839)
(196, 0.000341661)
(197, 0.000333302)
(198, 0.000376415)
(199, 0.000433661)
(200, 0.000604479)
(201, 0.00077484)
(202, 0.00108251)
(203, 0.00152912)
(204, 0.00194784)
(205, 0.00254187)
(206, 0.00283717)
(207, 0.00283378)
(208, 0.00227381)
(209, 0.00174958)
(210, 0.0011198)
(211, 0.000771758)
(212, 0.000447654)
(213, 0.000261124)
(214, 0.000152079)
(215, 8.06836e-05)
(216, 4.4154e-05)
(217, 2.70242e-05)
(218, 1.52633e-05)
(219, 9.93583e-06)
(220, 6.04245e-06)
(221, 3.53729e-06)
(222, 2.08749e-06)
(223, 1.26774e-06)
(224, 7.16593e-07)
(225, 4.8089e-07)
(226, 3.43188e-07)
(227, 2.24542e-07)
(228, 1.36145e-07)
(229, 8.82902e-08)
(230, 6.25255e-08)
(231, 4.00477e-08)
(232, 2.31158e-08)
(233, 1.38602e-08)
(234, 8.6742e-09)
(235, 5.12377e-09)
(236, 2.72206e-09)
(237, 1.55519e-09)
(238, 1.00358e-09)
(239, 6.17547e-10)
(240, 3.95662e-10)
(241, 2.47559e-10)
(242, 1.77622e-10)
(243, 1.14262e-10)
(244, 8.64843e-11)
(245, 5.9413e-11)
(246, 4.03865e-11)
(247, 3.37398e-11)
(248, 3.42358e-11)
(249, 3.82578e-11)
(250, 4.83507e-11)
(251, 5.63838e-11)
(252, 4.85742e-11)
(253, 3.72056e-11)
(254, 2.42578e-11)
(255, 1.29321e-11)
(256, 8.45705e-12)
(257, 5.0672e-12)
(258, 3.74382e-12)
(259, 2.64844e-12)
(260, 2.56185e-12)
(261, 2.86055e-12)
(262, 3.34052e-12)
(263, 3.25542e-12)
(264, 2.23648e-12)
(265, 1.66575e-12)
(266, 1.63568e-12)
(267, 1.85453e-12)
(268, 2.17835e-12)
(269, 2.19696e-12)
(270, 2.10345e-12)
(271, 1.60226e-12)
(272, 1.1295e-12)
(273, 9.90932e-13)
(274, 1.03084e-12)
(275, 1.1588e-12)
(276, 1.2227e-12)
(277, 1.05331e-12)
(278, 8.74717e-13)
(279, 6.49624e-13)
(280, 4.88862e-13)
(281, 4.22856e-13)
(282, 4.21034e-13)
(283, 4.59843e-13)
(284, 4.93417e-13)
(285, 4.84978e-13)
(286, 4.68318e-13)
(287, 4.553e-13)
(288, 4.36977e-13)
(289, 3.84574e-13)
(290, 5.36198e-13)
(291, 5.51983e-13)
(292, 5.11002e-13)
(293, 5.28213e-13)
(294, 4.99144e-13)
(295, 5.87059e-13)
(296, 8.43779e-13)
(297, 1.07757e-12)
(298, 1.05559e-12)
(299, 1.07724e-12)
(300, 9.30671e-13)
(301, 8.90998e-13)
(302, 8.63649e-13)
(303, 8.56783e-13)
(304, 7.48568e-13)
(305, 5.7558e-13)
(306, 4.73619e-13)
(307, 4.66636e-13)
(308, 5.30927e-13)
(309, 5.88826e-13)
(310, 4.94461e-13)
(311, 4.31238e-13)
(312, 3.27782e-13)
(313, 3.9287e-13)
(314, 5.81461e-13)
(315, 8.15061e-13)
(316, 8.58179e-13)
(317, 8.32708e-13)
(318, 6.63758e-13)
(319, 6.76489e-13)
(320, 6.84424e-13)
(321, 9.04427e-13)
(322, 9.32378e-13)
(323, 8.77266e-13)
(324, 8.21006e-13)
(325, 7.67002e-13)
(326, 7.64038e-13)
(327, 7.57844e-13)
(328, 6.93911e-13)
(329, 6.11617e-13)
(330, 5.14477e-13)
(331, 3.65578e-13)
(332, 3.66788e-13)
(333, 3.64873e-13)
(334, 3.04621e-13)
(335, 2.06363e-13)
(336, 1.73597e-13)
(337, 1.99469e-13)
(338, 2.09239e-13)
(339, 2.53115e-13)
(340, 2.49314e-13)
(341, 2.79014e-13)
(342, 2.48723e-13)
(343, 2.42108e-13)
(344, 3.18124e-13)
(345, 4.43026e-13)
(346, 5.57686e-13)
(347, 5.26127e-13)
(348, 4.09405e-13)
(349, 3.01114e-13)
(350, 2.64237e-13)
(351, 2.16435e-13)
(352, 1.58852e-13)
(353, 1.06211e-13)
(354, 7.7037e-14)
(355, 5.78951e-14)
(356, 5.08157e-14)
(357, 4.7909e-14)
(358, 5.02233e-14)
(359, 5.32065e-14)
(360, 5.98898e-14)
(361, 6.53253e-14)
(362, 8.54583e-14)
(363, 1.18278e-13)
(364, 1.35456e-13)
(365, 1.2107e-13)
(366, 1.06283e-13)
(367, 1.16538e-13)
(368, 1.1906e-13)
(369, 9.10153e-14)
(370, 6.70519e-14)
(371, 5.53265e-14)
(372, 5.88525e-14)
(373, 4.98243e-14)
(374, 4.54506e-14)
(375, 4.51249e-14)
(376, 4.26985e-14)
(377, 4.82052e-14)
(378, 5.24718e-14)
(379, 6.16856e-14)
(380, 6.38895e-14)
(381, 5.1328e-14)
(382, 4.60143e-14)
(383, 4.65144e-14)
(384, 4.26046e-14)
(385, 4.51827e-14)
(386, 4.7353e-14)
(387, 5.16772e-14)
(388, 5.59197e-14)
(389, 5.70702e-14)
(390, 6.39705e-14)
(391, 6.95333e-14)
(392, 6.78772e-14)
(393, 7.03258e-14)
(394, 7.18445e-14)
(395, 8.26989e-14)
(396, 9.39101e-14)
(397, 1.15086e-13)
(398, 1.22941e-13)
(399, 9.81694e-14)
(400, 7.84976e-14)
(401, 5.84778e-14)
(402, 4.95216e-14)
(403, 4.23911e-14)
(404, 3.46133e-14)
(405, 3.18396e-14)
(406, 3.68915e-14)
(407, 3.16616e-14)
(408, 2.9125e-14)
(409, 3.11824e-14)
(410, 3.02963e-14)
(411, 2.86583e-14)
(412, 2.39401e-14)
(413, 2.98041e-14)
(414, 3.86464e-14)
(415, 3.36133e-14)
(416, 2.67102e-14)
(417, 2.6034e-14)
(418, 2.83067e-14)
(419, 2.64018e-14)
(420, 2.24384e-14)
(421, 2.27945e-14)
(422, 2.08569e-14)
(423, 2.08037e-14)
(424, 2.5993e-14)
(425, 3.07433e-14)
(426, 2.39377e-14)
(427, 1.88164e-14)
(428, 1.93033e-14)
(429, 1.94864e-14)
(430, 2.07507e-14)
(431, 2.46657e-14)
(432, 2.2945e-14)
(433, 2.00204e-14)
(434, 2.09874e-14)
(435, 2.4205e-14)
(436, 2.51802e-14)
(437, 2.60982e-14)
(438, 3.4332e-14)
(439, 3.7944e-14)
(440, 3.7655e-14)
(441, 2.81505e-14)
(442, 2.06204e-14)
(443, 1.75962e-14)
(444, 2.09449e-14)
(445, 2.12872e-14)
(446, 1.97506e-14)
(447, 2.16902e-14)
(448, 2.01475e-14)
(449, 1.96704e-14)
(450, 1.91216e-14)
(451, 1.79306e-14)
(452, 1.50844e-14)
(453, 1.42215e-14)
(454, 1.48825e-14)
(455, 1.99846e-14)
(456, 2.92252e-14)
(457, 3.32891e-14)
(458, 3.49898e-14)
(459, 4.03022e-14)
(460, 3.94433e-14)
(461, 3.15797e-14)
(462, 2.9594e-14)
(463, 2.58595e-14)
(464, 2.31866e-14)
(465, 2.41549e-14)
(466, 2.44115e-14)
(467, 2.31359e-14)
(468, 1.89146e-14)
(469, 1.94083e-14)
(470, 1.87128e-14)
(471, 1.55669e-14)
(472, 1.61917e-14)
(473, 1.18099e-14)
(474, 8.30484e-15)
(475, 6.60556e-15)
(476, 6.31108e-15)
(477, 5.48369e-15)
(478, 4.48995e-15)
(479, 2.59784e-15)
(480, 1.89907e-15)
(481, 1.77386e-15)
(482, 1.34142e-15)
(483, 1.64973e-15)
(484, 2.18603e-15)
(485, 2.85844e-15)
(486, 3.51575e-15)
(487, 4.80669e-15)
(488, 5.37795e-15)
(489, 6.26192e-15)
(490, 6.57149e-15)
(491, 7.43445e-15)
(492, 7.93908e-15)
(493, 1.02262e-14)
(494, 1.16218e-14)
(495, 8.47746e-15)
(496, 5.97115e-15)
(497, 4.23128e-15)
(498, 3.81041e-15)
(499, 3.48676e-15)
(500, 2.59727e-15)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=*, color=vtorange, mark options={ fill=vtorange}, line width=1.5pt] coordinates { 
 (215, 0.000152079) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=*, color=mygreen, mark options={ fill=mygreen}, line width=1.5pt] coordinates { 
 (224, 1.26774e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=square,  mark size=4pt, color=vtmaroon, mark options={ fill=vtmaroon}, line width=1.0pt] coordinates { 
 (224, 1.26774e-06) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/matrixCollectionTrueRes1.tex <==
\addplot[color=vtorange, line width=1.5pt] coordinates { 
(0, 1)
(1, 1.48544)
(2, 3.19641)
(3, 3.55056)
(4, 4.22653)
(5, 3.26341)
(6, 1.57429)
(7, 1.38719)
(8, 0.742365)
(9, 0.268803)
(10, 0.148026)
(11, 0.0494908)
(12, 0.0210536)
(13, 0.00908201)
(14, 0.00792442)
(15, 0.00246247)
(16, 0.00151582)
(17, 0.000553924)
(18, 0.000106187)
(19, 3.76011e-05)
(20, 6.86054e-06)
(21, 1.62399e-06)
(22, 2.77765e-07)
(23, 3.80357e-08)
(24, 5.98794e-09)
(25, 9.53438e-10)
(26, 8.19384e-11)
(27, 1.15532e-11)
(28, 1.04816e-11)
(29, 1.0805e-11)
(30, 1.07362e-11)
(31, 1.0702e-11)
(32, 1.06892e-11)
(33, 1.06354e-11)
(34, 1.10172e-11)
(35, 1.10173e-11)
}; \label{plot:fp64} 
\addplot[ color=mygreen, line width=1.5pt, dotted] coordinates { 
(0, 1)
(1, 1.48544)
(2, 3.41544)
(3, 4.79783)
(4, 5.81231)
(5, 5.97428)
(6, 2.7129)
(7, 2.6112)
(8, 1.22877)
(9, 0.472644)
(10, 0.262356)
(11, 0.103592)
(12, 0.029717)
(13, 0.039123)
(14, 0.013216)
(15, 0.009309)
(16, 0.00335305)
(17, 0.00156855)
(18, 0.000607346)
(19, 0.000650566)
(20, 0.00161987)
(21, 0.00277157)
(22, 0.00389179)
(23, 0.00159984)
(24, 0.000441143)
(25, 0.0003273)
(26, 0.000210753)
(27, 0.00011156)
(28, 5.29547e-05)
(29, 3.50424e-05)
(30, 1.59518e-05)
(31, 4.66102e-06)
(32, 2.10823e-06)
(33, 2.81717e-06)
(34, 1.27232e-06)
(35, 1.74492e-06)
(36, 4.96178e-06)
(37, 5.93088e-06)
(38, 6.09713e-06)
(39, 3.73131e-06)
(40, 8.63044e-07)
(41, 3.62201e-07)
(42, 2.31505e-07)
(43, 6.76658e-08)
(44, 4.21458e-08)
(45, 1.96367e-08)
(46, 1.63672e-08)
(47, 8.36682e-09)
(48, 4.5143e-09)
(49, 2.9064e-09)
(50, 3.33272e-09)
(51, 3.78898e-09)
(52, 6.87244e-09)
(53, 1.33406e-08)
(54, 8.37459e-09)
(55, 3.59639e-09)
(56, 3.67759e-09)
(57, 2.14643e-09)
(58, 8.1568e-10)
(59, 2.77374e-10)
(60, 1.21527e-10)
(61, 4.37334e-11)
(62, 2.72762e-11)
(63, 1.74843e-11)
(64, 1.89411e-11)
(65, 2.07455e-11)
(66, 2.03819e-11)
(67, 2.47681e-11)
(68, 3.02355e-11)
(69, 3.36868e-11)
(70, 3.2347e-11)
(71, 1.95043e-11)
(72, 1.63364e-11)
(73, 1.65046e-11)
(74, 1.64312e-11)
(75, 1.62954e-11)
(76, 1.686e-11)
(77, 1.66374e-11)
(78, 1.67369e-11)
(79, 1.6748e-11)
(80, 1.67202e-11)
(81, 1.70304e-11)
(82, 1.69825e-11)
(83, 1.73749e-11)
(84, 1.7485e-11)
(85, 1.73684e-11)
(86, 1.70019e-11)
(87, 1.68817e-11)
(88, 1.66527e-11)
(89, 1.66269e-11)
(90, 1.66269e-11)
(91, 1.66269e-11)
(92, 1.66269e-11)
}; \label{plot:fp16} 
\addplot[color=mydeepblue, line width=2.5pt, dashed] coordinates { 
(0, 1)
(1, 1.48544)
(2, 3.19641)
(3, 3.55056)
(4, 4.22653)
(5, 3.26341)
(6, 1.57429)
(7, 1.38719)
(8, 0.742365)
(9, 0.268803)
(10, 0.148026)
(11, 0.0494908)
(12, 0.0210536)
(13, 0.00908201)
(14, 0.00792442)
(15, 0.00246247)
(16, 0.00151582)
(17, 0.000553924)
(18, 0.000106187)
(19, 3.76011e-05)
(20, 6.86054e-06)
(21, 1.62399e-06)
(22, 2.77766e-07)
(23, 3.9098e-08)
(24, 6.10387e-09)
(25, 9.95682e-10)
(26, 1.12479e-10)
(27, 1.1348e-11)
(28, 9.29013e-12)
(29, 1.11346e-11)
(30, 1.1137e-11)
(31, 1.36392e-11)
(32, 1.64565e-11)
(33, 1.41571e-11)
(34, 1.37968e-11)
(35, 1.15366e-11)
(36, 1.05677e-11)
(37, 1.0918e-11)
(38, 1.11932e-11)
(39, 1.14285e-11)
(40, 1.14914e-11)
(41, 1.16382e-11)
(42, 1.16509e-11)
(43, 1.17061e-11)
(44, 1.16864e-11)
(45, 1.16864e-11)
(46, 1.16864e-11)
(47, 1.18138e-11)
(48, 1.20667e-11)
(49, 1.16506e-11)
(50, 1.16653e-11)
(51, 1.15283e-11)
(52, 1.15283e-11)
(53, 1.15283e-11)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=*, color=vtorange, mark options={ fill=vtorange}, line width=1.5pt] coordinates { 
 (19, 0.000106187) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=*, color=mygreen, mark options={ fill=mygreen}, line width=1.5pt] coordinates { 
 (22, 1.62399e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=square,  mark size=4pt, color=vtmaroon, mark options={ fill=vtmaroon}, line width=1.0pt] coordinates { 
 (22, 1.62399e-06) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/matrixCollectionTrueRes2.tex <==
\addplot[color=vtorange, line width=1.5pt] coordinates { 
(0, 1)
(1, 0.778697)
(2, 0.579372)
(3, 0.450932)
(4, 0.0779467)
(5, 0.0102075)
(6, 0.00296766)
(7, 0.00100495)
(8, 0.000446799)
(9, 0.000145747)
(10, 7.32036e-05)
(11, 1.20748e-05)
(12, 4.62444e-06)
(13, 1.61959e-06)
(14, 2.6628e-07)
(15, 1.62551e-07)
(16, 6.77682e-08)
(17, 1.60565e-08)
(18, 2.67954e-09)
(19, 2.63787e-10)
(20, 4.50896e-11)
(21, 1.26602e-11)
(22, 2.1809e-12)
(23, 3.68268e-13)
(24, 7.50818e-14)
(25, 4.60706e-14)
(26, 4.52119e-14)
(27, 4.59703e-14)
}; \label{plot:fp64} 
\addplot[ color=mygreen, line width=1.5pt, dotted] coordinates { 
(0, 1)
(1, 0.778697)
(2, 0.580599)
(3, 0.45189)
(4, 0.0779708)
(5, 0.0102539)
(6, 0.00297672)
(7, 0.00100759)
(8, 0.000448808)
(9, 0.0001469)
(10, 7.38231e-05)
(11, 1.2151e-05)
(12, 4.6659e-06)
(13, 1.68096e-06)
(14, 3.94159e-07)
(15, 4.35559e-07)
(16, 2.10514e-07)
(17, 1.16965e-07)
(18, 6.39305e-08)
(19, 1.59286e-08)
(20, 1.86377e-09)
(21, 2.24631e-10)
(22, 5.84779e-11)
(23, 1.10963e-11)
(24, 2.47671e-12)
(25, 8.31137e-13)
(26, 9.2024e-13)
(27, 6.28405e-13)
(28, 5.24531e-13)
(29, 5.21731e-13)
(30, 5.19863e-13)
(31, 5.20034e-13)
(32, 5.20153e-13)
(33, 5.2027e-13)
}; \label{plot:fp16} 
\addplot[color=mydeepblue, line width=2.5pt, dashed] coordinates { 
(0, 1)
(1, 0.778697)
(2, 0.579372)
(3, 0.450932)
(4, 0.0779467)
(5, 0.0102075)
(6, 0.00296766)
(7, 0.00100495)
(8, 0.000446799)
(9, 0.000145747)
(10, 7.32036e-05)
(11, 1.20748e-05)
(12, 4.62444e-06)
(13, 1.61959e-06)
(14, 2.6628e-07)
(15, 1.62565e-07)
(16, 6.78385e-08)
(17, 1.60919e-08)
(18, 2.6823e-09)
(19, 2.64264e-10)
(20, 4.51362e-11)
(21, 1.26942e-11)
(22, 2.20095e-12)
(23, 4.11379e-13)
(24, 1.98146e-13)
(25, 1.93036e-13)
(26, 1.70505e-13)
(27, 1.66499e-13)
(28, 1.6484e-13)
(29, 1.64111e-13)
(30, 1.63951e-13)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=*, color=vtorange, mark options={ fill=vtorange}, line width=1.5pt] coordinates { 
 (10, 0.000145747) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=*, color=mygreen, mark options={ fill=mygreen}, line width=1.5pt] coordinates { 
 (14, 1.61959e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=square,  mark size=4pt, color=vtmaroon, mark options={ fill=vtmaroon}, line width=1.0pt] coordinates { 
 (14, 1.61959e-06) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/matrixCollectionTrueRes3.tex <==
\addplot[color=vtorange, line width=1.5pt] coordinates { 
(0, 1)
(1, 1.42637)
(2, 0.878305)
(3, 0.660423)
(4, 0.621626)
(5, 0.617083)
(6, 0.444714)
(7, 0.3016)
(8, 0.236347)
(9, 0.261193)
(10, 0.352013)
(11, 0.297942)
(12, 0.28825)
(13, 0.287969)
(14, 0.33694)
(15, 0.370409)
(16, 0.407543)
(17, 0.420782)
(18, 0.539186)
(19, 0.542635)
(20, 0.542156)
(21, 0.409052)
(22, 0.363244)
(23, 0.476827)
(24, 0.467993)
(25, 0.369677)
(26, 0.261651)
(27, 0.231202)
(28, 0.20573)
(29, 0.215601)
(30, 0.207284)
(31, 0.197114)
(32, 0.19343)
(33, 0.225947)
(34, 0.219554)
(35, 0.216848)
(36, 0.213816)
(37, 0.179577)
(38, 0.168588)
(39, 0.177722)
(40, 0.20091)
(41, 0.245376)
(42, 0.307874)
(43, 0.343784)
(44, 0.3239)
(45, 0.310015)
(46, 0.381407)
(47, 0.394666)
(48, 0.412247)
(49, 0.414696)
(50, 0.350553)
(51, 0.28652)
(52, 0.347155)
(53, 0.356346)
(54, 0.432601)
(55, 0.420322)
(56, 0.403148)
(57, 0.353494)
(58, 0.290692)
(59, 0.336153)
(60, 0.314811)
(61, 0.304414)
(62, 0.262099)
(63, 0.219692)
(64, 0.161287)
(65, 0.150513)
(66, 0.144207)
(67, 0.145611)
(68, 0.157899)
(69, 0.173957)
(70, 0.185294)
(71, 0.158717)
(72, 0.141262)
(73, 0.149172)
(74, 0.15941)
(75, 0.141312)
(76, 0.134768)
(77, 0.12582)
(78, 0.11699)
(79, 0.124224)
(80, 0.121435)
(81, 0.100634)
(82, 0.0902935)
(83, 0.0932379)
(84, 0.0905371)
(85, 0.0865168)
(86, 0.0786874)
(87, 0.0771799)
(88, 0.0790719)
(89, 0.0922611)
(90, 0.123265)
(91, 0.149412)
(92, 0.162163)
(93, 0.192384)
(94, 0.159813)
(95, 0.127276)
(96, 0.105846)
(97, 0.102336)
(98, 0.0851896)
(99, 0.0702177)
(100, 0.06678)
(101, 0.0729973)
(102, 0.0579428)
(103, 0.0652762)
(104, 0.0623484)
(105, 0.0610203)
(106, 0.0746428)
(107, 0.0919592)
(108, 0.0959937)
(109, 0.132104)
(110, 0.142923)
(111, 0.153966)
(112, 0.161779)
(113, 0.150666)
(114, 0.143432)
(115, 0.116784)
(116, 0.108386)
(117, 0.10972)
(118, 0.113533)
(119, 0.113555)
(120, 0.0966089)
(121, 0.0930293)
(122, 0.0828717)
(123, 0.0742513)
(124, 0.0675264)
(125, 0.0580481)
(126, 0.0584521)
(127, 0.0463781)
(128, 0.0389031)
(129, 0.0305147)
(130, 0.0274424)
(131, 0.0233545)
(132, 0.0193726)
(133, 0.0202562)
(134, 0.0188696)
(135, 0.0195995)
(136, 0.020403)
(137, 0.0243228)
(138, 0.0235843)
(139, 0.0244297)
(140, 0.0267226)
(141, 0.0304593)
(142, 0.0388173)
(143, 0.0434623)
(144, 0.0493787)
(145, 0.0451681)
(146, 0.0367089)
(147, 0.02356)
(148, 0.0163057)
(149, 0.0118964)
(150, 0.00876251)
(151, 0.00818986)
(152, 0.00970798)
(153, 0.0111386)
(154, 0.01373)
(155, 0.0160522)
(156, 0.0177938)
(157, 0.0190229)
(158, 0.0242091)
(159, 0.0293)
(160, 0.0375718)
(161, 0.0332539)
(162, 0.0288242)
(163, 0.0237145)
(164, 0.0188621)
(165, 0.015623)
(166, 0.0123549)
(167, 0.0100467)
(168, 0.00788753)
(169, 0.0057471)
(170, 0.00544758)
(171, 0.00622627)
(172, 0.00736818)
(173, 0.00857822)
(174, 0.00884979)
(175, 0.00861999)
(176, 0.00907043)
(177, 0.0115219)
(178, 0.0140396)
(179, 0.01733)
(180, 0.0211218)
(181, 0.0202344)
(182, 0.0174074)
(183, 0.0142901)
(184, 0.0100696)
(185, 0.00742962)
(186, 0.00487273)
(187, 0.00344434)
(188, 0.00206944)
(189, 0.00148136)
(190, 0.00108805)
(191, 0.000778848)
(192, 0.00053916)
(193, 0.000403605)
(194, 0.000373124)
(195, 0.000380614)
(196, 0.000342803)
(197, 0.000334842)
(198, 0.000378981)
(199, 0.000437651)
(200, 0.000610479)
(201, 0.000784919)
(202, 0.00110406)
(203, 0.00157208)
(204, 0.00202965)
(205, 0.00267034)
(206, 0.00301075)
(207, 0.00305877)
(208, 0.00252005)
(209, 0.0019307)
(210, 0.00121207)
(211, 0.000826942)
(212, 0.000476651)
(213, 0.000272348)
(214, 0.000150423)
(215, 7.85885e-05)
(216, 4.16448e-05)
(217, 2.52592e-05)
(218, 1.42849e-05)
(219, 9.28334e-06)
(220, 5.73277e-06)
(221, 3.37778e-06)
(222, 2.01789e-06)
(223, 1.23495e-06)
(224, 7.0438e-07)
(225, 4.75967e-07)
(226, 3.40695e-07)
(227, 2.23559e-07)
(228, 1.35799e-07)
(229, 8.82757e-08)
(230, 6.25414e-08)
(231, 4.00625e-08)
(232, 2.31393e-08)
(233, 1.38717e-08)
(234, 8.68002e-09)
(235, 5.13066e-09)
(236, 2.72698e-09)
(237, 1.55943e-09)
(238, 1.00698e-09)
(239, 6.20418e-10)
(240, 3.98766e-10)
(241, 2.51457e-10)
(242, 1.83545e-10)
(243, 1.22314e-10)
(244, 9.87825e-11)
(245, 7.54801e-11)
(246, 6.2721e-11)
(247, 6.65061e-11)
(248, 7.94479e-11)
(249, 8.85307e-11)
(250, 9.5111e-11)
(251, 8.13855e-11)
(252, 5.46241e-11)
(253, 3.64126e-11)
(254, 2.21597e-11)
(255, 1.19859e-11)
(256, 7.94162e-12)
(257, 5.38208e-12)
(258, 4.48811e-12)
(259, 4.12952e-12)
(260, 5.00636e-12)
(261, 6.41657e-12)
(262, 8.201e-12)
(263, 7.37433e-12)
(264, 4.6244e-12)
(265, 3.12157e-12)
(266, 2.59079e-12)
(267, 2.38705e-12)
(268, 2.53716e-12)
(269, 2.81227e-12)
(270, 3.48174e-12)
(271, 3.43848e-12)
(272, 2.73745e-12)
(273, 2.21028e-12)
(274, 1.9556e-12)
(275, 1.80821e-12)
(276, 1.73402e-12)
(277, 1.72206e-12)
(278, 1.70133e-12)
(279, 1.69686e-12)
(280, 1.71015e-12)
(281, 1.6929e-12)
(282, 1.67448e-12)
(283, 1.70488e-12)
(284, 1.71605e-12)
(285, 1.72086e-12)
(286, 1.73678e-12)
(287, 1.72731e-12)
(288, 1.73636e-12)
(289, 1.73098e-12)
(290, 1.74305e-12)
(291, 1.74767e-12)
(292, 1.75863e-12)
(293, 1.75376e-12)
(294, 1.75492e-12)
(295, 1.74118e-12)
(296, 1.74009e-12)
(297, 1.74611e-12)
(298, 1.69305e-12)
(299, 1.71156e-12)
(300, 1.73181e-12)
(301, 1.73844e-12)
(302, 1.73343e-12)
(303, 1.72588e-12)
(304, 1.7619e-12)
(305, 1.71839e-12)
(306, 1.71539e-12)
(307, 1.73453e-12)
(308, 1.73796e-12)
(309, 1.74176e-12)
(310, 1.73825e-12)
(311, 1.73544e-12)
(312, 1.75635e-12)
(313, 1.75832e-12)
(314, 1.76514e-12)
(315, 1.76581e-12)
(316, 1.76552e-12)
(317, 1.76696e-12)
(318, 1.76555e-12)
(319, 1.76579e-12)
(320, 1.74268e-12)
(321, 1.75894e-12)
(322, 1.76745e-12)
(323, 1.76491e-12)
(324, 1.78943e-12)
(325, 1.79892e-12)
(326, 1.79754e-12)
(327, 1.79669e-12)
(328, 1.79277e-12)
(329, 1.78992e-12)
(330, 1.79176e-12)
(331, 1.79041e-12)
(332, 1.78522e-12)
(333, 1.7812e-12)
(334, 1.79886e-12)
(335, 1.80333e-12)
(336, 1.8219e-12)
(337, 1.821e-12)
(338, 1.80168e-12)
(339, 1.80011e-12)
(340, 1.80124e-12)
(341, 1.81851e-12)
(342, 1.8555e-12)
(343, 1.83596e-12)
(344, 1.84096e-12)
(345, 1.85451e-12)
(346, 1.85099e-12)
(347, 1.8507e-12)
(348, 1.85887e-12)
(349, 1.85782e-12)
(350, 1.85783e-12)
}; \label{plot:fp64} 
\addplot[ color=mygreen, line width=1.5pt, dotted] coordinates { 
(0, 1)
(1, 1.42637)
(2, 0.878307)
(3, 0.660887)
(4, 0.623283)
(5, 0.618855)
(6, 0.445565)
(7, 0.30116)
(8, 0.236006)
(9, 0.261402)
(10, 0.352634)
(11, 0.298786)
(12, 0.289633)
(13, 0.288953)
(14, 0.337607)
(15, 0.368303)
(16, 0.404125)
(17, 0.417083)
(18, 0.533332)
(19, 0.538878)
(20, 0.540553)
(21, 0.408687)
(22, 0.360587)
(23, 0.470801)
(24, 0.462375)
(25, 0.36646)
(26, 0.260727)
(27, 0.230126)
(28, 0.203112)
(29, 0.212649)
(30, 0.203857)
(31, 0.194616)
(32, 0.190238)
(33, 0.224395)
(34, 0.220496)
(35, 0.216509)
(36, 0.209771)
(37, 0.178901)
(38, 0.168335)
(39, 0.176294)
(40, 0.200458)
(41, 0.241412)
(42, 0.301184)
(43, 0.338061)
(44, 0.32249)
(45, 0.325061)
(46, 0.398813)
(47, 0.403455)
(48, 0.41255)
(49, 0.421946)
(50, 0.353297)
(51, 0.294528)
(52, 0.343042)
(53, 0.357927)
(54, 0.426865)
(55, 0.402068)
(56, 0.404711)
(57, 0.355707)
(58, 0.296065)
(59, 0.351443)
(60, 0.34828)
(61, 0.311596)
(62, 0.283169)
(63, 0.221355)
(64, 0.174176)
(65, 0.158367)
(66, 0.139721)
(67, 0.146986)
(68, 0.159777)
(69, 0.172325)
(70, 0.181094)
(71, 0.162666)
(72, 0.145112)
(73, 0.152674)
(74, 0.167388)
(75, 0.142805)
(76, 0.144019)
(77, 0.130304)
(78, 0.120645)
(79, 0.116413)
(80, 0.123547)
(81, 0.107886)
(82, 0.093208)
(83, 0.0905465)
(84, 0.0983509)
(85, 0.0858526)
(86, 0.0837765)
(87, 0.076961)
(88, 0.0811588)
(89, 0.0837728)
(90, 0.118591)
(91, 0.140036)
(92, 0.14867)
(93, 0.171326)
(94, 0.177759)
(95, 0.136495)
(96, 0.125348)
(97, 0.106921)
(98, 0.100353)
(99, 0.082458)
(100, 0.0697646)
(101, 0.0710792)
(102, 0.0694833)
(103, 0.0562643)
(104, 0.0657892)
(105, 0.0615676)
(106, 0.0639323)
(107, 0.0811637)
(108, 0.0961141)
(109, 0.105999)
(110, 0.144119)
(111, 0.145987)
(112, 0.160597)
(113, 0.161972)
(114, 0.14886)
(115, 0.137871)
(116, 0.113084)
(117, 0.114525)
(118, 0.117612)
(119, 0.124305)
(120, 0.11737)
(121, 0.0971443)
(122, 0.0978534)
(123, 0.0873749)
(124, 0.0777181)
(125, 0.068251)
(126, 0.0618016)
(127, 0.0610746)
(128, 0.0520452)
(129, 0.0421089)
(130, 0.0323474)
(131, 0.0296059)
(132, 0.0254351)
(133, 0.0225026)
(134, 0.0198388)
(135, 0.0212186)
(136, 0.0190033)
(137, 0.0200296)
(138, 0.0225404)
(139, 0.0264495)
(140, 0.0257329)
(141, 0.0259003)
(142, 0.0282943)
(143, 0.036159)
(144, 0.0434346)
(145, 0.0477672)
(146, 0.0537776)
(147, 0.0447276)
(148, 0.0336107)
(149, 0.0231863)
(150, 0.0153256)
(151, 0.0112328)
(152, 0.00938301)
(153, 0.00857272)
(154, 0.010607)
(155, 0.0123345)
(156, 0.0144695)
(157, 0.0172131)
(158, 0.0178444)
(159, 0.0203521)
(160, 0.0242631)
(161, 0.0287844)
(162, 0.0363654)
(163, 0.0368834)
(164, 0.0297856)
(165, 0.0247557)
(166, 0.0204965)
(167, 0.0175079)
(168, 0.01508)
(169, 0.0128131)
(170, 0.011223)
(171, 0.00947307)
(172, 0.00891168)
(173, 0.0105245)
(174, 0.0123284)
(175, 0.012366)
(176, 0.0111097)
(177, 0.00940878)
(178, 0.00794735)
(179, 0.0079161)
(180, 0.00912962)
(181, 0.00978485)
(182, 0.0105894)
(183, 0.010532)
(184, 0.00913995)
(185, 0.00839014)
(186, 0.00871035)
(187, 0.00910605)
(188, 0.0104233)
(189, 0.012407)
(190, 0.0125574)
(191, 0.0142031)
(192, 0.0146389)
(193, 0.0145421)
(194, 0.0110798)
(195, 0.00979813)
(196, 0.00899575)
(197, 0.00867178)
(198, 0.00824992)
(199, 0.00835608)
(200, 0.00866848)
(201, 0.00896887)
(202, 0.00755835)
(203, 0.00548216)
(204, 0.00431436)
(205, 0.00325346)
(206, 0.00274349)
(207, 0.00251936)
(208, 0.00240135)
(209, 0.00239041)
(210, 0.00230297)
(211, 0.00204119)
(212, 0.00194104)
(213, 0.00176818)
(214, 0.00167027)
(215, 0.00140477)
(216, 0.00123115)
(217, 0.00119992)
(218, 0.00113575)
(219, 0.00102291)
(220, 0.00105256)
(221, 0.00110065)
(222, 0.0010492)
(223, 0.00106737)
(224, 0.000915774)
(225, 0.00100547)
(226, 0.00101933)
(227, 0.000941211)
(228, 0.000772909)
(229, 0.000497339)
(230, 0.000352375)
(231, 0.000296391)
(232, 0.000327262)
(233, 0.000425225)
(234, 0.000598172)
(235, 0.000741828)
(236, 0.000827292)
(237, 0.000886195)
(238, 0.000925108)
(239, 0.000934018)
(240, 0.00100253)
(241, 0.0011767)
(242, 0.00142072)
(243, 0.00147191)
(244, 0.00136447)
(245, 0.0014375)
(246, 0.00164299)
(247, 0.00167948)
(248, 0.00188161)
(249, 0.00196727)
(250, 0.00158704)
(251, 0.0012561)
(252, 0.00117172)
(253, 0.00112743)
(254, 0.00109763)
(255, 0.00123599)
(256, 0.00107507)
(257, 0.000998674)
(258, 0.000802647)
(259, 0.000540418)
(260, 0.000370174)
(261, 0.000281446)
(262, 0.000227757)
(263, 0.000189322)
(264, 0.000174545)
(265, 0.000140637)
(266, 0.000103818)
(267, 8.42344e-05)
(268, 5.84647e-05)
(269, 5.1752e-05)
(270, 4.90923e-05)
(271, 5.97698e-05)
(272, 6.34291e-05)
(273, 6.78775e-05)
(274, 7.50931e-05)
(275, 7.86991e-05)
(276, 9.3312e-05)
(277, 0.000102461)
(278, 0.000106695)
(279, 0.000113979)
(280, 0.000112734)
(281, 8.80885e-05)
(282, 6.55745e-05)
(283, 5.45173e-05)
(284, 4.80152e-05)
(285, 3.42336e-05)
(286, 2.06361e-05)
(287, 1.44687e-05)
(288, 1.2856e-05)
(289, 1.30128e-05)
(290, 1.48284e-05)
(291, 1.68487e-05)
(292, 2.08193e-05)
(293, 2.18814e-05)
(294, 1.90255e-05)
(295, 1.55109e-05)
(296, 1.21603e-05)
(297, 1.18046e-05)
(298, 1.23168e-05)
(299, 1.47437e-05)
(300, 1.71382e-05)
(301, 1.88832e-05)
(302, 1.87031e-05)
(303, 1.58788e-05)
(304, 1.42463e-05)
(305, 1.81866e-05)
(306, 2.01108e-05)
(307, 2.28959e-05)
(308, 2.52592e-05)
(309, 2.43201e-05)
(310, 2.16978e-05)
(311, 2.11459e-05)
(312, 2.19453e-05)
(313, 1.83287e-05)
(314, 1.76873e-05)
(315, 1.55244e-05)
(316, 1.35104e-05)
(317, 1.38365e-05)
(318, 1.49381e-05)
(319, 1.44879e-05)
(320, 1.22932e-05)
(321, 1.02937e-05)
(322, 1.00179e-05)
(323, 1.11471e-05)
(324, 1.33383e-05)
(325, 1.48698e-05)
(326, 1.56999e-05)
(327, 1.7438e-05)
(328, 1.54648e-05)
(329, 1.8147e-05)
(330, 1.82187e-05)
(331, 1.9197e-05)
(332, 2.08936e-05)
(333, 2.15713e-05)
(334, 2.04734e-05)
(335, 2.0996e-05)
(336, 1.82513e-05)
(337, 2.0149e-05)
(338, 1.7123e-05)
(339, 1.51081e-05)
(340, 1.49571e-05)
(341, 1.59596e-05)
(342, 1.54184e-05)
(343, 1.4158e-05)
(344, 1.26788e-05)
(345, 1.08594e-05)
(346, 9.83671e-06)
(347, 7.93662e-06)
(348, 5.93834e-06)
(349, 4.85914e-06)
(350, 3.7385e-06)
(351, 3.59985e-06)
(352, 4.52355e-06)
(353, 5.32614e-06)
(354, 4.27346e-06)
(355, 3.28371e-06)
(356, 3.29867e-06)
(357, 3.52539e-06)
(358, 4.13437e-06)
(359, 4.21449e-06)
(360, 5.91037e-06)
(361, 7.8565e-06)
(362, 9.0793e-06)
(363, 8.22353e-06)
(364, 7.57779e-06)
(365, 6.16397e-06)
(366, 4.83229e-06)
(367, 4.13657e-06)
(368, 4.21314e-06)
(369, 4.98851e-06)
(370, 6.36829e-06)
(371, 7.01762e-06)
(372, 6.44678e-06)
(373, 6.51106e-06)
(374, 8.27091e-06)
(375, 1.1152e-05)
(376, 1.31792e-05)
(377, 1.40733e-05)
(378, 1.33447e-05)
(379, 1.20787e-05)
(380, 1.06686e-05)
(381, 8.55552e-06)
(382, 6.86539e-06)
(383, 6.22106e-06)
(384, 5.37399e-06)
(385, 3.73546e-06)
(386, 2.64807e-06)
(387, 2.37184e-06)
(388, 2.47947e-06)
(389, 2.44992e-06)
(390, 1.94264e-06)
(391, 1.47297e-06)
(392, 1.48866e-06)
(393, 1.60005e-06)
(394, 1.47349e-06)
(395, 2.03807e-06)
(396, 2.98431e-06)
(397, 3.89868e-06)
(398, 3.86704e-06)
(399, 3.51374e-06)
(400, 4.18958e-06)
(401, 4.79769e-06)
(402, 3.98423e-06)
(403, 2.75376e-06)
(404, 2.29154e-06)
(405, 2.10954e-06)
(406, 2.34872e-06)
(407, 2.89349e-06)
(408, 3.16474e-06)
(409, 2.88608e-06)
(410, 2.04011e-06)
(411, 1.50348e-06)
(412, 1.30336e-06)
(413, 1.25457e-06)
(414, 1.24656e-06)
(415, 1.11526e-06)
(416, 9.84654e-07)
(417, 9.8154e-07)
(418, 8.83463e-07)
(419, 1.03935e-06)
(420, 1.05292e-06)
(421, 1.01618e-06)
(422, 9.94472e-07)
(423, 9.28879e-07)
(424, 9.89384e-07)
(425, 1.19783e-06)
(426, 1.45517e-06)
(427, 1.54025e-06)
(428, 2.11901e-06)
(429, 2.41914e-06)
(430, 2.3806e-06)
(431, 2.23184e-06)
(432, 2.08887e-06)
(433, 2.31171e-06)
(434, 1.93588e-06)
(435, 1.45848e-06)
(436, 1.28518e-06)
(437, 1.15959e-06)
(438, 1.10025e-06)
(439, 9.63196e-07)
(440, 1.02538e-06)
(441, 1.34724e-06)
(442, 1.31626e-06)
(443, 9.68647e-07)
(444, 8.60284e-07)
(445, 8.85978e-07)
(446, 8.027e-07)
(447, 7.68557e-07)
(448, 7.92002e-07)
(449, 7.71475e-07)
(450, 6.99195e-07)
(451, 7.58644e-07)
(452, 9.31562e-07)
(453, 9.91236e-07)
(454, 1.10131e-06)
(455, 1.3748e-06)
(456, 1.49178e-06)
(457, 1.26788e-06)
(458, 1.08756e-06)
(459, 9.41446e-07)
(460, 8.21757e-07)
(461, 7.08506e-07)
(462, 7.57516e-07)
(463, 7.34257e-07)
(464, 6.61896e-07)
(465, 6.27114e-07)
(466, 6.19638e-07)
(467, 6.14592e-07)
(468, 5.87821e-07)
(469, 4.42016e-07)
(470, 3.08313e-07)
(471, 2.80758e-07)
(472, 2.89917e-07)
(473, 2.76435e-07)
(474, 2.60475e-07)
(475, 2.16332e-07)
(476, 2.02159e-07)
(477, 1.90004e-07)
(478, 1.70766e-07)
(479, 1.19102e-07)
(480, 1.15405e-07)
(481, 1.149e-07)
(482, 9.7898e-08)
(483, 8.01657e-08)
(484, 6.34207e-08)
(485, 4.64007e-08)
(486, 2.75532e-08)
(487, 2.24442e-08)
(488, 1.9978e-08)
(489, 1.95359e-08)
(490, 1.66472e-08)
(491, 1.44228e-08)
(492, 1.44732e-08)
(493, 1.35992e-08)
(494, 1.3356e-08)
(495, 1.5429e-08)
(496, 1.56833e-08)
(497, 1.7591e-08)
(498, 2.31429e-08)
(499, 2.88473e-08)
(500, 2.98781e-08)
}; \label{plot:fp16} 
\addplot[color=mydeepblue, line width=2.5pt, dashed] coordinates { 
(0, 1)
(1, 1.42637)
(2, 0.878305)
(3, 0.660423)
(4, 0.621626)
(5, 0.617083)
(6, 0.444714)
(7, 0.3016)
(8, 0.236347)
(9, 0.261193)
(10, 0.352013)
(11, 0.297942)
(12, 0.28825)
(13, 0.287969)
(14, 0.33694)
(15, 0.370409)
(16, 0.407543)
(17, 0.420782)
(18, 0.539186)
(19, 0.542635)
(20, 0.542156)
(21, 0.409052)
(22, 0.363244)
(23, 0.476827)
(24, 0.467993)
(25, 0.369677)
(26, 0.261651)
(27, 0.231202)
(28, 0.20573)
(29, 0.215601)
(30, 0.207284)
(31, 0.197114)
(32, 0.19343)
(33, 0.225947)
(34, 0.219554)
(35, 0.216848)
(36, 0.213816)
(37, 0.179577)
(38, 0.168588)
(39, 0.177722)
(40, 0.20091)
(41, 0.245376)
(42, 0.307874)
(43, 0.343784)
(44, 0.3239)
(45, 0.310015)
(46, 0.381407)
(47, 0.394666)
(48, 0.412247)
(49, 0.414696)
(50, 0.350553)
(51, 0.28652)
(52, 0.347155)
(53, 0.356346)
(54, 0.432601)
(55, 0.420322)
(56, 0.403148)
(57, 0.353494)
(58, 0.290692)
(59, 0.336153)
(60, 0.314811)
(61, 0.304414)
(62, 0.262099)
(63, 0.219692)
(64, 0.161287)
(65, 0.150513)
(66, 0.144207)
(67, 0.145611)
(68, 0.157899)
(69, 0.173957)
(70, 0.185294)
(71, 0.158717)
(72, 0.141262)
(73, 0.149172)
(74, 0.15941)
(75, 0.141312)
(76, 0.134768)
(77, 0.12582)
(78, 0.11699)
(79, 0.124224)
(80, 0.121435)
(81, 0.100634)
(82, 0.0902935)
(83, 0.0932379)
(84, 0.0905371)
(85, 0.0865168)
(86, 0.0786874)
(87, 0.0771799)
(88, 0.0790719)
(89, 0.0922611)
(90, 0.123265)
(91, 0.149412)
(92, 0.162163)
(93, 0.192384)
(94, 0.159813)
(95, 0.127276)
(96, 0.105846)
(97, 0.102336)
(98, 0.0851896)
(99, 0.0702177)
(100, 0.06678)
(101, 0.0729973)
(102, 0.0579428)
(103, 0.0652762)
(104, 0.0623484)
(105, 0.0610203)
(106, 0.0746428)
(107, 0.0919592)
(108, 0.0959937)
(109, 0.132104)
(110, 0.142923)
(111, 0.153966)
(112, 0.161779)
(113, 0.150666)
(114, 0.143432)
(115, 0.116784)
(116, 0.108386)
(117, 0.10972)
(118, 0.113533)
(119, 0.113555)
(120, 0.0966089)
(121, 0.0930293)
(122, 0.0828717)
(123, 0.0742513)
(124, 0.0675264)
(125, 0.0580481)
(126, 0.0584521)
(127, 0.0463781)
(128, 0.0389031)
(129, 0.0305147)
(130, 0.0274424)
(131, 0.0233545)
(132, 0.0193726)
(133, 0.0202562)
(134, 0.0188696)
(135, 0.0195995)
(136, 0.020403)
(137, 0.0243228)
(138, 0.0235843)
(139, 0.0244297)
(140, 0.0267226)
(141, 0.0304593)
(142, 0.0388173)
(143, 0.0434623)
(144, 0.0493787)
(145, 0.0451681)
(146, 0.0367089)
(147, 0.02356)
(148, 0.0163057)
(149, 0.0118964)
(150, 0.0087625)
(151, 0.00818985)
(152, 0.00970797)
(153, 0.0111386)
(154, 0.01373)
(155, 0.0160522)
(156, 0.0177937)
(157, 0.0190229)
(158, 0.0242091)
(159, 0.0292999)
(160, 0.0375718)
(161, 0.0332539)
(162, 0.0288241)
(163, 0.0237145)
(164, 0.0188621)
(165, 0.015623)
(166, 0.0123549)
(167, 0.0100467)
(168, 0.0078875)
(169, 0.00574708)
(170, 0.00544755)
(171, 0.00622625)
(172, 0.00736812)
(173, 0.00857812)
(174, 0.00884982)
(175, 0.00861998)
(176, 0.00907049)
(177, 0.011522)
(178, 0.0140397)
(179, 0.0173298)
(180, 0.0211215)
(181, 0.0202338)
(182, 0.0174071)
(183, 0.0142898)
(184, 0.0100694)
(185, 0.007429)
(186, 0.00487183)
(187, 0.00344402)
(188, 0.00206888)
(189, 0.00148059)
(190, 0.00108746)
(191, 0.000778097)
(192, 0.000538539)
(193, 0.000403058)
(194, 0.000372466)
(195, 0.000379839)
(196, 0.000341661)
(197, 0.000333302)
(198, 0.000376415)
(199, 0.000433661)
(200, 0.000604479)
(201, 0.00077484)
(202, 0.00108251)
(203, 0.00152912)
(204, 0.00194784)
(205, 0.00254187)
(206, 0.00283717)
(207, 0.00283378)
(208, 0.00227381)
(209, 0.00174958)
(210, 0.0011198)
(211, 0.000771758)
(212, 0.000447654)
(213, 0.000261124)
(214, 0.000152079)
(215, 8.06836e-05)
(216, 4.4154e-05)
(217, 2.70242e-05)
(218, 1.52633e-05)
(219, 9.93583e-06)
(220, 6.04245e-06)
(221, 3.53729e-06)
(222, 2.08749e-06)
(223, 1.26774e-06)
(224, 7.16593e-07)
(225, 4.8089e-07)
(226, 3.43188e-07)
(227, 2.24542e-07)
(228, 1.36145e-07)
(229, 8.82902e-08)
(230, 6.25255e-08)
(231, 4.00477e-08)
(232, 2.31158e-08)
(233, 1.38603e-08)
(234, 8.6742e-09)
(235, 5.12376e-09)
(236, 2.72204e-09)
(237, 1.55522e-09)
(238, 1.00354e-09)
(239, 6.17588e-10)
(240, 3.95649e-10)
(241, 2.47558e-10)
(242, 1.77658e-10)
(243, 1.1425e-10)
(244, 8.65346e-11)
(245, 5.94331e-11)
(246, 4.04075e-11)
(247, 3.37985e-11)
(248, 3.42572e-11)
(249, 3.83389e-11)
(250, 4.83701e-11)
(251, 5.64368e-11)
(252, 4.85815e-11)
(253, 3.72979e-11)
(254, 2.42842e-11)
(255, 1.30727e-11)
(256, 8.64218e-12)
(257, 5.36378e-12)
(258, 4.20729e-12)
(259, 3.19816e-12)
(260, 3.20436e-12)
(261, 3.38785e-12)
(262, 3.83354e-12)
(263, 3.67461e-12)
(264, 2.92195e-12)
(265, 2.4156e-12)
(266, 2.50823e-12)
(267, 2.55188e-12)
(268, 2.90663e-12)
(269, 2.80051e-12)
(270, 2.8172e-12)
(271, 2.42819e-12)
(272, 2.21535e-12)
(273, 2.10021e-12)
(274, 2.14874e-12)
(275, 2.16614e-12)
(276, 2.22002e-12)
(277, 2.12104e-12)
(278, 2.04742e-12)
(279, 1.93226e-12)
(280, 1.84688e-12)
(281, 1.86207e-12)
(282, 1.84886e-12)
(283, 1.87849e-12)
(284, 1.86698e-12)
(285, 1.89916e-12)
(286, 1.88867e-12)
(287, 1.87519e-12)
(288, 1.91614e-12)
(289, 1.92112e-12)
(290, 1.97725e-12)
(291, 1.96705e-12)
(292, 1.94688e-12)
(293, 1.93423e-12)
(294, 1.97271e-12)
(295, 1.97888e-12)
(296, 2.08215e-12)
(297, 2.20759e-12)
(298, 2.16609e-12)
(299, 2.22364e-12)
(300, 2.12064e-12)
(301, 2.14366e-12)
(302, 2.05868e-12)
(303, 2.08767e-12)
(304, 2.06666e-12)
(305, 1.98724e-12)
(306, 1.97811e-12)
(307, 1.94619e-12)
(308, 2.02814e-12)
(309, 1.98781e-12)
(310, 1.96281e-12)
(311, 1.96174e-12)
(312, 1.92175e-12)
(313, 1.99836e-12)
(314, 1.9953e-12)
(315, 2.10761e-12)
(316, 2.07455e-12)
(317, 2.10791e-12)
(318, 2.05618e-12)
(319, 1.98162e-12)
(320, 2.08356e-12)
(321, 2.05915e-12)
(322, 2.22305e-12)
(323, 2.07102e-12)
(324, 2.14643e-12)
(325, 2.07987e-12)
(326, 2.104e-12)
(327, 2.15958e-12)
(328, 2.05312e-12)
(329, 2.15272e-12)
(330, 2.01986e-12)
(331, 2.11319e-12)
(332, 2.06414e-12)
(333, 2.05711e-12)
(334, 2.10346e-12)
(335, 2.06154e-12)
(336, 2.10223e-12)
(337, 2.0432e-12)
(338, 2.09483e-12)
(339, 2.08602e-12)
(340, 2.05119e-12)
(341, 2.07622e-12)
(342, 2.06741e-12)
(343, 2.08345e-12)
(344, 2.0871e-12)
(345, 2.12969e-12)
(346, 2.12777e-12)
(347, 2.14748e-12)
(348, 2.0973e-12)
(349, 2.07347e-12)
(350, 2.1038e-12)
(351, 2.08577e-12)
(352, 2.13168e-12)
(353, 2.15128e-12)
(354, 2.13645e-12)
(355, 2.13943e-12)
(356, 2.15232e-12)
(357, 2.14622e-12)
(358, 2.14416e-12)
(359, 2.13254e-12)
(360, 2.15201e-12)
(361, 2.15368e-12)
(362, 2.14973e-12)
(363, 2.11973e-12)
(364, 2.13552e-12)
(365, 2.12256e-12)
(366, 2.11618e-12)
(367, 2.10758e-12)
(368, 2.10545e-12)
(369, 2.09508e-12)
(370, 2.11663e-12)
(371, 2.14247e-12)
(372, 2.09706e-12)
(373, 2.11658e-12)
(374, 2.12379e-12)
(375, 2.10288e-12)
(376, 2.11542e-12)
(377, 2.11424e-12)
(378, 2.13588e-12)
(379, 2.11021e-12)
(380, 2.11451e-12)
(381, 2.14551e-12)
(382, 2.11202e-12)
(383, 2.15174e-12)
(384, 2.13529e-12)
(385, 2.12742e-12)
(386, 2.13098e-12)
(387, 2.13038e-12)
(388, 2.14167e-12)
(389, 2.14598e-12)
(390, 2.12695e-12)
(391, 2.10516e-12)
(392, 2.10099e-12)
(393, 2.09339e-12)
(394, 2.07057e-12)
(395, 2.09452e-12)
(396, 2.10304e-12)
(397, 2.11065e-12)
(398, 2.10194e-12)
(399, 2.12087e-12)
(400, 2.09116e-12)
(401, 2.11918e-12)
(402, 2.11228e-12)
(403, 2.11164e-12)
(404, 2.11825e-12)
(405, 2.10106e-12)
(406, 2.14479e-12)
(407, 2.11342e-12)
(408, 2.11211e-12)
(409, 2.13304e-12)
(410, 2.13932e-12)
(411, 2.13144e-12)
(412, 2.13097e-12)
(413, 2.15125e-12)
(414, 2.16051e-12)
(415, 2.15503e-12)
(416, 2.15086e-12)
(417, 2.16412e-12)
(418, 2.1833e-12)
(419, 2.17593e-12)
(420, 2.18393e-12)
(421, 2.21401e-12)
(422, 2.20459e-12)
(423, 2.20687e-12)
(424, 2.23009e-12)
(425, 2.22768e-12)
(426, 2.22327e-12)
(427, 2.22167e-12)
(428, 2.2342e-12)
(429, 2.23397e-12)
(430, 2.21252e-12)
(431, 2.20424e-12)
(432, 2.21985e-12)
(433, 2.17976e-12)
(434, 2.19412e-12)
(435, 2.1985e-12)
(436, 2.21486e-12)
(437, 2.19301e-12)
(438, 2.1871e-12)
(439, 2.1817e-12)
(440, 2.20139e-12)
(441, 2.21854e-12)
(442, 2.23249e-12)
(443, 2.22958e-12)
(444, 2.25279e-12)
(445, 2.24916e-12)
(446, 2.21385e-12)
(447, 2.22267e-12)
(448, 2.2218e-12)
(449, 2.22081e-12)
(450, 2.20672e-12)
(451, 2.20807e-12)
(452, 2.19794e-12)
(453, 2.21634e-12)
(454, 2.21668e-12)
(455, 2.20455e-12)
(456, 2.22449e-12)
(457, 2.216e-12)
(458, 2.22438e-12)
(459, 2.24678e-12)
(460, 2.23396e-12)
(461, 2.25691e-12)
(462, 2.26867e-12)
(463, 2.28382e-12)
(464, 2.28325e-12)
(465, 2.27762e-12)
(466, 2.28231e-12)
(467, 2.26015e-12)
(468, 2.26538e-12)
(469, 2.27614e-12)
(470, 2.28489e-12)
(471, 2.28284e-12)
(472, 2.27827e-12)
(473, 2.26764e-12)
(474, 2.25758e-12)
(475, 2.27762e-12)
(476, 2.26532e-12)
(477, 2.23971e-12)
(478, 2.23286e-12)
(479, 2.24705e-12)
(480, 2.247e-12)
(481, 2.24634e-12)
(482, 2.24642e-12)
(483, 2.23378e-12)
(484, 2.24256e-12)
(485, 2.23546e-12)
(486, 2.25053e-12)
(487, 2.23618e-12)
(488, 2.26457e-12)
(489, 2.27327e-12)
(490, 2.2495e-12)
(491, 2.23393e-12)
(492, 2.2367e-12)
(493, 2.23313e-12)
(494, 2.22037e-12)
(495, 2.22766e-12)
(496, 2.20625e-12)
(497, 2.22086e-12)
(498, 2.23671e-12)
(499, 2.24414e-12)
(500, 2.23805e-12)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=*, color=vtorange, mark options={ fill=vtorange}, line width=1.5pt] coordinates { 
 (215, 0.000152079) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=*, color=mygreen, mark options={ fill=mygreen}, line width=1.5pt] coordinates { 
 (224, 1.26774e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=square,  mark size=4pt, color=vtmaroon, mark options={ fill=vtmaroon}, line width=1.0pt] coordinates { 
 (224, 1.26774e-06) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/negative.tex <==


\begin{figure}[h!]
    \centering
\begin{tikzpicture}
  % \begin{axis}[
  %   width=8cm,
  %   height=6cm,
  %   xlabel={Iteration},
  %   ylabel={Residual norm},
  %   ymode=log,
  %   legend style={
  %     legend pos=outer north west,
  %   },
  % ]
  \begin{axis}[
      width=8cm,
    height=6cm,
    xlabel={Iteration},
    ylabel={Residual norm},
    ymode=log,
    legend pos= outer north east,
    ymajorgrids=true,
    grid style=dashed,
    ]
\addplot[color=vtorange, line width=1.5pt] coordinates {

(0, 1)
(1, 4.39291)
(2, 5.29928)
(3, 5.21449)
(4, 4.54562)
(5, 3.62804)
(6, 2.70552)
(7, 1.91285)
(8, 1.29543)
(9, 0.84524)
(10, 0.531917)
(11, 0.321556)
(12, 0.184958)
(13, 0.099681)
(14, 0.174127)
(15, 0.0510999)
(16, 0.0333325)
(17, 0.0282839)
(18, 0.00916562)
(19, 0.0183916)
(20, 0.00272215)
(21, 0.00901182)
(22, 0.000704056)
(23, 0.00206541)
(24, 0.00024793)
(25, 0.000158747)
(26, 7.74768e-05)
(27, 2.83995e-05)
(28, 2.95487e-05)
(29, 2.48355e-05)
(30, 2.19603e-06)
(31, 1.12874e-05)
(32, 6.40124e-06)
(33, 1.62965e-07)
(34, 8.63702e-07)
(35, 4.31572e-07)
(36, 7.2287e-07)
(37, 8.17815e-09)
(38, 3.72419e-08)
(39, 5.16942e-08)
(40, 1.68054e-08)
(41, 2.59207e-10)
(42, 2.47856e-10)
(43, 2.98209e-10)
(44, 3.43917e-10)
(45, 2.03053e-10)
(46, 5.47096e-12)
(47, 2.84098e-12)
(48, 2.93526e-12)
(49, 4.92782e-12)
(50, 3.03295e-12)
(51, 7.36315e-14)
};
\addplot[ color=mydeepblue, line width=1.5pt, dashed] coordinates {
(0, 1)
(1, 4.39291)
(2, 5.29928)
(3, 5.21449)
(4, 4.54562)
(5, 3.62804)
(6, 2.70552)
(7, 1.91285)
(8, 1.29543)
(9, 0.84524)
(10, 0.531917)
(11, 0.321556)
(12, 0.184958)
(13, 0.099681)
(14, 0.174127)
(15, 0.0510999)
(16, 0.0333325)
(17, 0.0282839)
(18, 0.00916562)
(19, 0.0183916)
(20, 0.00272215)
(21, 0.00901182)
(22, 0.000704056)
(23, 0.00206541)
(24, 0.00024793)
(25, 0.000158747)
(26, 7.74768e-05)
(27, 2.83995e-05)
(28, 2.95487e-05)
(29, 2.48355e-05)
(30, 2.19603e-06)
(31, 1.12874e-05)
(32, 6.40381e-06)
(33, 5.67696e-06)
(34, 1.61181e-07)
(35, 1.14664e-06)
(36, 4.14371e-07)
(37, 7.66415e-07)
(38, 2.23643e-07)
(39, 8.48957e-08)
(40, 9.3406e-09)
(41, 1.49664e-08)
(42, 9.05771e-08)
(43, 2.22359e-08)
(44, 1.88775e-08)
(45, 8.14352e-09)
(46, 2.80152e-10)
(47, 8.95278e-10)
(48, 1.11703e-09)
(49, 1.00301e-09)
(50, 1.08361e-09)
(51, 1.53455e-09)
(52, 8.73765e-11)
(53, 1.95517e-10)
(54, 8.88636e-11)
(55, 1.20119e-10)
(56, 4.08607e-11)
(57, 1.13132e-11)
(58, 6.16509e-12)
(59, 4.36378e-11)
(60, 1.44985e-11)
(61, 3.46236e-11)
(62, 2.45959e-11)
(63, 7.77186e-12)
(64, 9.13421e-12)
(65, 8.44823e-12)
(66, 1.75804e-12)
(67, 1.11963e-12)
(68, 1.3862e-12)
(69, 2.32896e-12)
(70, 1.46472e-12)
(71, 1.10645e-12)
(72, 5.38431e-13)
(73, 2.28945e-13)
(74, 4.90588e-13)
(75, 3.14922e-13)
(76, 2.83078e-13)
(77, 1.50575e-13)
(78, 2.23941e-13)
(79, 1.16565e-13)
(80, 1.66001e-13)
(81, 1.30908e-13)
(82, 1.34578e-13)
(83, 2.66338e-13)
(84, 1.13075e-13)
(85, 1.96513e-13)
(86, 4.97638e-14)
};
\addplot[ color=mygreen, line width=1.5pt, dotted] coordinates {
(0, 1)
(1, 4.39291)
(2, 5.29939)
(3, 5.21243)
(4, 4.54498)
(5, 3.62706)
(6, 2.70789)
(7, 2.26629)
(8, 2.90012)
(9, 1.31666)
(10, 2.37906)
(11, 0.839853)
(12, 0.924542)
(13, 0.588899)
(14, 1.29061)
(15, 0.462889)
(16, 0.426657)
(17, 0.778407)
(18, 0.177205)
(19, 0.838142)
(20, 0.248882)
(21, 0.168745)
(22, 0.129838)
(23, 0.261046)
(24, 0.166816)
(25, 0.185487)
(26, 0.0889451)
(27, 0.0555511)
(28, 0.0845644)
(29, 0.193856)
(30, 0.0600376)
(31, 0.0210839)
(32, 0.0708511)
(33, 0.0511212)
(34, 0.0318104)
(35, 0.0498354)
(36, 0.0090338)
(37, 0.0154955)
(38, 0.0160006)
(39, 0.046004)
(40, 0.00860136)
(41, 0.00918582)
(42, 0.00573743)
(43, 0.00704192)
(44, 0.00593376)
(45, 0.00392315)
(46, 0.00433232)
(47, 0.00466797)
(48, 0.00261614)
(49, 0.00594564)
(50, 0.00466326)
(51, 0.00376255)
(52, 0.00177447)
(53, 0.000563226)
(54, 0.00172389)
(55, 0.00111372)
(56, 0.00324232)
(57, 0.000826084)
(58, 0.000550792)
(59, 0.000769758)
(60, 0.000739273)
(61, 0.000257976)
(62, 0.000300671)
(63, 0.000117183)
(64, 0.000224303)
(65, 0.000237893)
(66, 0.00028336)
(67, 0.000732852)
(68, 4.36676e-05)
(69, 5.53852e-05)
(70, 8.73095e-05)
(71, 2.45243e-05)
(72, 4.35301e-05)
(73, 8.22089e-05)
(74, 2.09235e-05)
(75, 2.59516e-05)
(76, 3.16094e-05)
(77, 2.8011e-05)
(78, 3.09188e-05)
(79, 4.29999e-05)
(80, 5.44565e-05)
(81, 1.29039e-05)
(82, 1.00813e-05)
(83, 1.38333e-05)
(84, 8.88069e-06)
(85, 4.60907e-06)
(86, 2.55043e-06)
(87, 3.91218e-06)
(88, 8.46849e-06)
(89, 4.07867e-06)
(90, 1.18984e-06)
(91, 2.84977e-06)
(92, 2.86838e-06)
(93, 1.06876e-06)
(94, 3.25651e-06)
(95, 2.93812e-06)
(96, 1.79993e-06)
(97, 1.85105e-06)
(98, 1.88529e-06)
(99, 1.41663e-06)
(100, 7.37935e-07)
(101, 7.03545e-07)
(102, 4.60921e-07)
(103, 5.62417e-07)
(104, 6.14943e-07)
(105, 1.1265e-06)
(106, 2.09621e-07)
(107, 1.39424e-07)
(108, 6.54013e-08)
(109, 7.32255e-08)
(110, 9.12104e-08)
(111, 2.7046e-07)
(112, 2.87636e-07)
(113, 1.00899e-07)
(114, 4.28723e-08)
(115, 2.38796e-08)
(116, 4.47775e-08)
(117, 4.25712e-08)
(118, 2.57387e-08)
(119, 3.6848e-08)
(120, 3.9035e-08)
(121, 3.39226e-08)
(122, 4.11288e-08)
(123, 1.90621e-08)
(124, 9.97094e-09)
(125, 1.29582e-08)
(126, 1.00396e-08)
(127, 8.34904e-09)
(128, 7.57528e-09)
(129, 3.78792e-09)
(130, 1.08685e-08)
(131, 2.43643e-09)
(132, 1.69293e-09)
(133, 1.95197e-09)
(134, 6.72258e-09)
(135, 1.90158e-09)
(136, 3.19998e-09)
(137, 3.91822e-09)
(138, 4.10732e-09)
(139, 2.88777e-09)
(140, 3.38001e-09)
(141, 4.8917e-10)
(142, 2.28128e-10)
(143, 4.5433e-10)
(144, 1.70388e-10)
(145, 3.22831e-10)
(146, 1.82006e-10)
(147, 4.94493e-10)
(148, 3.19336e-10)
(149, 5.7711e-11)
(150, 1.31461e-10)
(151, 1.60471e-10)
(152, 8.23251e-11)
(153, 9.99625e-11)
(154, 1.02906e-10)
(155, 6.57807e-11)
(156, 1.15683e-10)
(157, 4.73029e-11)
(158, 6.15428e-11)
(159, 6.33456e-11)
(160, 2.04693e-11)
(161, 3.00601e-11)
(162, 3.63647e-11)
(163, 3.91846e-11)
(164, 3.30869e-11)
(165, 1.49034e-11)
(166, 1.57312e-11)
(167, 1.1804e-11)
(168, 1.26303e-11)
(169, 2.18181e-11)
(170, 4.12506e-11)
(171, 1.44639e-11)
(172, 7.44557e-12)
(173, 2.84467e-12)
(174, 3.80471e-12)
(175, 3.61086e-12)
(176, 2.36078e-12)
(177, 1.80928e-12)
(178, 1.32121e-12)
(179, 3.33099e-12)
(180, 2.92038e-12)
(181, 1.3521e-12)
(182, 2.07659e-12)
(183, 2.65273e-12)
(184, 1.96267e-12)
(185, 1.9235e-12)
(186, 6.1152e-13)
(187, 4.77327e-13)
(188, 4.60126e-13)
(189, 3.69883e-13)
(190, 2.58227e-13)
(191, 2.97966e-13)
(192, 1.30796e-13)
(193, 2.1054e-13)
(194, 1.72182e-13)
(195, 4.43643e-13)
(196, 3.02285e-13)
(197, 1.75793e-13)
(198, 1.83748e-13)
(199, 1.2241e-13)
(200, 6.0585e-14)
};
\addplot[only marks, mark=*, color=vtorange, mark options={ fill=vtorange}, line width=1.5pt] coordinates {
(27, 2.83995e-05)
};
\addplot[
    only marks, mark=*,
    color=mygreen,
    mark options={fill=mygreen},
    line width=1.5pt
] coordinates {
    (46, 2.80152e-10)
};
\legend{
    {doublePCG},
    {AMPDS-PCG $\lp\text{PS}_1 \rp$},
    {AMPDS-PCG $\lp\text{PS}_2 \rp$},
    {$\lp u_{z,k},u_{r,k} \rp=(\mathrm{FP32},\, \mathrm{FP32})$},
    {$\lp u_{z,k},u_{r,k} \rp=(\mathrm{FP16},\, \mathrm{FP32})$},
}
    \end{axis}
\end{tikzpicture}
\caption{Convergence curves for PCG: A comparison of four PCG variants—fully double-precision PCG, naive half-precision PCG, AMPDS-PCG with the $\text{PS}_1$ precision selector, and AMPDS-PCG with $\text{PS}_2$. The matrix $\BA$ is generated using MATLAB's \texttt{gallery(`poisson', 30)} function, and the right-hand side vector $\Bb$ is an all-ones vector. In the naive half-precision PCG, $\Bz_k$ becomes too small after 69 iterations, leading to underflow (blue dot). In the AMPDS-PCG with $\text{PS}_2$, the orange dot indicates where $u_{z,k}$ and $u_{r,k}$ switch to FP32, and the green dot indicates where $u_{z,k}$ switches to FP16.}
\end{figure}



==> 5.Numerical/data/okCond_1_2.tex <==
\addplot[color=myyellow, line width=1.0pt] coordinates { 
(0, 1)
(1, 0.549476)
(2, 0.384681)
(3, 0.286103)
(4, 0.192441)
(5, 0.166271)
(6, 0.155366)
(7, 0.157332)
(8, 0.139599)
(9, 0.11068)
(10, 0.109239)
(11, 0.0940287)
(12, 0.0960165)
(13, 0.106487)
(14, 0.112336)
(15, 0.115761)
(16, 0.124842)
(17, 0.0988582)
(18, 0.101978)
(19, 0.123992)
(20, 0.128558)
(21, 0.137682)
(22, 0.136072)
(23, 0.151975)
(24, 0.123303)
(25, 0.103884)
(26, 0.0920547)
(27, 0.0784574)
(28, 0.0690504)
(29, 0.0664938)
(30, 0.0575491)
(31, 0.0434721)
(32, 0.0301231)
(33, 0.0157622)
(34, 0.00972499)
(35, 0.00520532)
(36, 0.00308372)
(37, 0.00203262)
(38, 0.00142149)
(39, 0.000960471)
(40, 0.0006672)
(41, 0.000467397)
(42, 0.000257394)
(43, 0.000149224)
(44, 8.99516e-05)
(45, 5.28653e-05)
(46, 3.36123e-05)
(47, 2.12833e-05)
(48, 1.2537e-05)
(49, 6.81793e-06)
(50, 4.84943e-06)
(51, 2.69707e-06)
(52, 1.72817e-06)
(53, 1.19771e-06)
(54, 9.43307e-07)
(55, 6.35216e-07)
(56, 4.44909e-07)
(57, 3.35503e-07)
(58, 1.55763e-07)
(59, 1.13248e-07)
(60, 5.85045e-08)
(61, 2.81909e-08)
(62, 1.30518e-08)
(63, 6.32586e-09)
(64, 2.52838e-09)
(65, 1.12653e-09)
(66, 5.06307e-10)
(67, 2.11781e-10)
(68, 8.63643e-11)
}; \label{plot:fp64} 
\addplot[color=mydeepblue, dashed, line width=1.0pt] coordinates { 
(0, 1)
(1, 0.549476)
(2, 0.384681)
(3, 0.286103)
(4, 0.192441)
(5, 0.166271)
(6, 0.155366)
(7, 0.157332)
(8, 0.139599)
(9, 0.11068)
(10, 0.109239)
(11, 0.0940287)
(12, 0.0960165)
(13, 0.106487)
(14, 0.112336)
(15, 0.115761)
(16, 0.124842)
(17, 0.0988582)
(18, 0.101978)
(19, 0.123992)
(20, 0.128558)
(21, 0.137682)
(22, 0.136072)
(23, 0.151975)
(24, 0.123303)
(25, 0.103884)
(26, 0.0920547)
(27, 0.0784574)
(28, 0.0690504)
(29, 0.0664938)
(30, 0.0575491)
(31, 0.0434721)
(32, 0.0301231)
(33, 0.0157622)
(34, 0.00972499)
(35, 0.00520532)
(36, 0.00308372)
(37, 0.00203262)
(38, 0.00142149)
(39, 0.000960471)
(40, 0.0006672)
(41, 0.000467397)
(42, 0.000257394)
(43, 0.000149224)
(44, 8.99516e-05)
(45, 5.28653e-05)
(46, 3.36123e-05)
(47, 2.12833e-05)
(48, 1.2537e-05)
(49, 6.81793e-06)
(50, 4.84943e-06)
(51, 2.69707e-06)
(52, 1.72817e-06)
(53, 1.19771e-06)
(54, 9.43307e-07)
(55, 6.35213e-07)
(56, 4.4492e-07)
(57, 3.35549e-07)
(58, 1.55818e-07)
(59, 1.13313e-07)
(60, 5.85215e-08)
(61, 2.8194e-08)
(62, 1.30569e-08)
(63, 6.3331e-09)
(64, 2.55375e-09)
(65, 1.17995e-09)
(66, 6.34759e-10)
(67, 2.80708e-10)
(68, 1.26589e-10)
(69, 4.43663e-11)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=x, color=red,  mark size=3pt,  line width=1.5pt] coordinates { 
 (44, 8.99516e-05) 
}; \label{plot:fp32tofp16} 
 \addplot[only marks, mark=x, color=black,  mark size=3pt,  line width=1.5pt] coordinates { 
 (54, 9.43307e-07) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=o, color=blue,  mark size=3pt, line width=1.0pt] coordinates { 
 (56, 4.4492e-07) 
}; \label{plot:residualfp64tofp32} 
\addplot[ color=mygreen, line width=1.0pt, dotted] coordinates { 
(0, 1)
(1, 0.549476)
(2, 0.384705)
(3, 0.286077)
(4, 0.192424)
(5, 0.166276)
(6, 0.155363)
(7, 0.157334)
(8, 0.139611)
(9, 0.110692)
(10, 0.109217)
(11, 0.0940074)
(12, 0.0959975)
(13, 0.106455)
(14, 0.112284)
(15, 0.115703)
(16, 0.124778)
(17, 0.0988005)
(18, 0.101938)
(19, 0.123949)
(20, 0.1284)
(21, 0.137589)
(22, 0.136029)
(23, 0.151871)
(24, 0.12339)
(25, 0.103885)
(26, 0.09202)
(27, 0.0785085)
(28, 0.0690658)
(29, 0.0665483)
(30, 0.0575951)
(31, 0.0435669)
(32, 0.0304129)
(33, 0.0160343)
(34, 0.00994094)
(35, 0.00536876)
(36, 0.00319847)
(37, 0.0020699)
(38, 0.00152033)
(39, 0.00100677)
(40, 0.000706966)
(41, 0.000506835)
(42, 0.000279424)
(43, 0.000174132)
(44, 0.000110011)
(45, 5.71943e-05)
(46, 4.01303e-05)
(47, 2.51425e-05)
(48, 1.89519e-05)
(49, 1.34289e-05)
(50, 1.32885e-05)
(51, 1.52579e-05)
(52, 2.00941e-05)
(53, 2.80111e-05)
(54, 3.24736e-05)
(55, 3.21473e-05)
(56, 2.66503e-05)
(57, 2.31293e-05)
(58, 2.04476e-05)
(59, 2.08798e-05)
(60, 2.45591e-05)
(61, 2.20982e-05)
(62, 2.27867e-05)
(63, 2.09684e-05)
(64, 1.7356e-05)
(65, 1.59538e-05)
(66, 1.57487e-05)
(67, 1.16173e-05)
(68, 7.8388e-06)
(69, 3.98738e-06)
(70, 2.10988e-06)
(71, 1.32805e-06)
(72, 1.11538e-06)
(73, 1.20854e-06)
(74, 1.18406e-06)
(75, 1.0165e-06)
(76, 4.65636e-07)
(77, 1.69866e-07)
(78, 9.19056e-08)
(79, 5.33793e-08)
(80, 3.97854e-08)
(81, 3.13929e-08)
(82, 3.23255e-08)
(83, 2.1662e-08)
(84, 1.36207e-08)
(85, 6.60186e-09)
(86, 4.14719e-09)
(87, 2.63355e-09)
(88, 2.68264e-09)
(89, 2.03965e-09)
(90, 1.43429e-09)
(91, 1.43215e-09)
(92, 2.18271e-09)
(93, 3.89643e-09)
(94, 4.32185e-09)
(95, 4.50333e-09)
(96, 4.92541e-09)
(97, 4.47986e-09)
(98, 3.25325e-09)
(99, 1.70795e-09)
(100, 1.26105e-09)
(101, 1.12084e-09)
(102, 1.01771e-09)
(103, 7.19266e-10)
(104, 5.93442e-10)
(105, 7.17488e-10)
(106, 7.35314e-10)
(107, 4.56269e-10)
(108, 4.73745e-10)
(109, 3.71168e-10)
(110, 2.05819e-10)
(111, 1.29025e-10)
(112, 1.03846e-10)
(113, 1.12547e-10)
(114, 9.07095e-11)
}; \label{plot:fp16} 


==> 5.Numerical/data/okCond_1_res.tex <==
\addplot[color=myyellow, line width=1.0pt] coordinates {
(0, 1)
(1, 0.508761)
(2, 0.44966)
(3, 0.349696)
(4, 0.291644)
(5, 0.268619)
(6, 0.223722)
(7, 0.242503)
(8, 0.231782)
(9, 0.138892)
(10, 0.11607)
(11, 0.0887681)
(12, 0.0779323)
(13, 0.0757631)
(14, 0.061475)
(15, 0.0545092)
(16, 0.048355)
(17, 0.0471564)
(18, 0.0392887)
(19, 0.0293365)
(20, 0.0340883)
(21, 0.0405514)
(22, 0.0398602)
(23, 0.0448877)
(24, 0.0515839)
(25, 0.062466)
(26, 0.0805603)
(27, 0.0753342)
(28, 0.0584599)
(29, 0.0419472)
(30, 0.040101)
(31, 0.0402179)
(32, 0.0328947)
(33, 0.0179779)
(34, 0.00953373)
(35, 0.00583711)
(36, 0.00400151)
(37, 0.00286008)
(38, 0.00208185)
(39, 0.00151107)
(40, 0.00101964)
(41, 0.000783152)
(42, 0.000545674)
(43, 0.000286461)
(44, 0.000161402)
(45, 9.65703e-05)
(46, 5.68827e-05)
(47, 3.41162e-05)
(48, 2.01048e-05)
(49, 1.28003e-05)
(50, 7.24484e-06)
(51, 5.09833e-06)
(52, 3.07686e-06)
(53, 1.96368e-06)
(54, 1.18927e-06)
(55, 6.91013e-07)
(56, 3.12934e-07)
(57, 1.53712e-07)
(58, 6.79667e-08)
(59, 3.16718e-08)
(60, 1.36249e-08)
(61, 5.81022e-09)
(62, 2.68302e-09)
(63, 1.16564e-09)
(64, 5.60513e-10)
(65, 2.5726e-10)
(66, 1.23199e-10)
(67, 6.87877e-11)
(68, 3.10235e-11)
(69, 1.52654e-11)
(70, 6.94029e-12)
(71, 2.39174e-12)
(72, 1.17617e-12)
(73, 6.04598e-13)
(74, 3.42378e-13)
(75, 1.69222e-13)
(76, 6.11568e-14)
(77, 2.45626e-14)
(78, 9.56606e-15)
(79, 4.27475e-15)
(80, 1.63441e-15)
(81, 6.07954e-16)
}; \label{plot:fp64}
\addplot[ color=mydeepblue, line width=1.0pt, dashed] coordinates {
(0, 1)
(1, 0.508761)
(2, 0.44966)
(3, 0.349696)
(4, 0.291644)
(5, 0.268619)
(6, 0.223722)
(7, 0.242503)
(8, 0.231782)
(9, 0.138892)
(10, 0.11607)
(11, 0.0887681)
(12, 0.0779323)
(13, 0.0757631)
(14, 0.061475)
(15, 0.0545092)
(16, 0.048355)
(17, 0.0471564)
(18, 0.0392887)
(19, 0.0293365)
(20, 0.0340883)
(21, 0.0405514)
(22, 0.0398602)
(23, 0.0448877)
(24, 0.0515839)
(25, 0.062466)
(26, 0.0805603)
(27, 0.0753342)
(28, 0.0584599)
(29, 0.0419472)
(30, 0.040101)
(31, 0.0402179)
(32, 0.0328947)
(33, 0.0179779)
(34, 0.00953373)
(35, 0.00583711)
(36, 0.00400151)
(37, 0.00286008)
(38, 0.00208185)
(39, 0.00151107)
(40, 0.00101964)
(41, 0.000783152)
(42, 0.000545674)
(43, 0.000286461)
(44, 0.000161402)
(45, 9.65703e-05)
(46, 5.68827e-05)
(47, 3.41162e-05)
(48, 2.01048e-05)
(49, 1.28003e-05)
(50, 7.24484e-06)
(51, 5.09833e-06)
(52, 3.07686e-06)
(53, 1.96368e-06)
(54, 1.18927e-06)
(55, 6.91013e-07)
(56, 3.12934e-07)
(57, 1.53712e-07)
(58, 6.79667e-08)
(59, 3.16718e-08)
(60, 1.36249e-08)
(61, 5.81022e-09)
(62, 2.68302e-09)
(63, 1.16564e-09)
(64, 5.60513e-10)
(65, 2.57261e-10)
(66, 1.23201e-10)
(67, 6.87908e-11)
(68, 3.10302e-11)
(69, 1.52765e-11)
(70, 6.96597e-12)
(71, 2.44703e-12)
(72, 1.27667e-12)
(73, 7.33438e-13)
(74, 4.34545e-13)
(75, 2.31642e-13)
(76, 9.68978e-14)
(77, 4.01193e-14)
(78, 2.10338e-14)
(79, 1.7544e-14)
(80, 2.39667e-14)
(81, 3.03875e-14)
(82, 2.35744e-14)
(83, 1.28489e-14)
(84, 1.11737e-14)
(85, 1.74629e-14)
(86, 2.72606e-14)
(87, 2.06944e-14)
(88, 1.16732e-14)
(89, 1.50943e-14)
(90, 3.14406e-14)
(91, 3.20852e-14)
(92, 1.94474e-14)
(93, 1.39297e-14)
(94, 2.19904e-14)
(95, 2.38138e-14)
(96, 1.46078e-14)
(97, 8.80597e-15)
(98, 9.44724e-15)
(99, 8.37584e-15)
(100, 3.96263e-15)
}; \label{plot:fp64mixed}
\addplot[ color=mygreen, line width=1.0pt, dotted] coordinates {
(0, 1)
(1, 0.508761)
(2, 0.449663)
(3, 0.349701)
(4, 0.291626)
(5, 0.268615)
(6, 0.223726)
(7, 0.242459)
(8, 0.231744)
(9, 0.138955)
(10, 0.116091)
(11, 0.0887584)
(12, 0.0779365)
(13, 0.0757666)
(14, 0.0615014)
(15, 0.0545232)
(16, 0.0483377)
(17, 0.0471458)
(18, 0.0392601)
(19, 0.0293557)
(20, 0.034079)
(21, 0.0405421)
(22, 0.0398484)
(23, 0.0449017)
(24, 0.0515972)
(25, 0.0624052)
(26, 0.08048)
(27, 0.0753471)
(28, 0.0584667)
(29, 0.0419686)
(30, 0.0401287)
(31, 0.040251)
(32, 0.0329653)
(33, 0.0180942)
(34, 0.00963143)
(35, 0.00593691)
(36, 0.00413576)
(37, 0.00298374)
(38, 0.00241909)
(39, 0.00163325)
(40, 0.00109334)
(41, 0.000804596)
(42, 0.000582375)
(43, 0.000311442)
(44, 0.000177204)
(45, 0.000116689)
(46, 6.5735e-05)
(47, 4.28175e-05)
(48, 2.61878e-05)
(49, 2.10963e-05)
(50, 1.79167e-05)
(51, 2.0187e-05)
(52, 2.47305e-05)
(53, 2.84019e-05)
(54, 3.59054e-05)
(55, 3.49338e-05)
(56, 3.43485e-05)
(57, 3.08862e-05)
(58, 2.72622e-05)
(59, 2.29323e-05)
(60, 2.29822e-05)
(61, 3.32223e-05)
(62, 4.599e-05)
(63, 4.64507e-05)
(64, 3.04182e-05)
(65, 1.46621e-05)
(66, 7.69351e-06)
(67, 3.7112e-06)
(68, 2.4834e-06)
(69, 2.18936e-06)
(70, 2.40893e-06)
(71, 2.30059e-06)
(72, 1.65432e-06)
(73, 8.38712e-07)
(74, 4.84959e-07)
(75, 2.82044e-07)
(76, 2.14335e-07)
(77, 1.65884e-07)
(78, 1.17075e-07)
(79, 8.04973e-08)
(80, 5.07016e-08)
(81, 2.98267e-08)
(82, 1.81384e-08)
(83, 1.3907e-08)
(84, 1.52888e-08)
(85, 1.29976e-08)
(86, 8.03079e-09)
(87, 5.02487e-09)
(88, 4.73069e-09)
(89, 4.58893e-09)
(90, 5.65035e-09)
(91, 5.87443e-09)
(92, 6.90998e-09)
(93, 8.51198e-09)
(94, 7.56086e-09)
(95, 6.18728e-09)
(96, 5.31633e-09)
(97, 5.59548e-09)
(98, 6.33071e-09)
(99, 5.90316e-09)
(100, 9.23632e-09)
}; \label{plot:fp16}
\addplot[only marks, mark=x, color=red,   mark size=3pt, line width=1.5pt] coordinates {
(50, 7.24484e-06)
}; \label{plot:fp64tofp32}
\addplot[only marks,mark=x, color=black,   mark size=3pt,line width=1.5pt] coordinates {
(55, 6.91013e-07)
};\label{plot:fp32tofp16}
\addplot[only marks, mark=o, color=blue,  mark size=3pt,line width=1.5pt] coordinates {
(61, 5.81022e-09)
};\label{plot:residualfp64tofp32} 





==> 5.Numerical/data/okCond_1_trueRes.tex <==
\addplot[color=myyellow, line width=1.0pt] coordinates {
(0, 1)
(1, 0.508761)
(2, 0.44966)
(3, 0.349696)
(4, 0.291644)
(5, 0.268619)
(6, 0.223722)
(7, 0.242503)
(8, 0.231782)
(9, 0.138892)
(10, 0.11607)
(11, 0.0887681)
(12, 0.0779323)
(13, 0.0757631)
(14, 0.061475)
(15, 0.0545092)
(16, 0.048355)
(17, 0.0471564)
(18, 0.0392887)
(19, 0.0293365)
(20, 0.0340883)
(21, 0.0405514)
(22, 0.0398602)
(23, 0.0448877)
(24, 0.0515839)
(25, 0.062466)
(26, 0.0805603)
(27, 0.0753342)
(28, 0.0584599)
(29, 0.0419472)
(30, 0.040101)
(31, 0.0402179)
(32, 0.0328947)
(33, 0.0179779)
(34, 0.00953373)
(35, 0.00583711)
(36, 0.00400151)
(37, 0.00286008)
(38, 0.00208185)
(39, 0.00151107)
(40, 0.00101964)
(41, 0.000783152)
(42, 0.000545674)
(43, 0.000286461)
(44, 0.000161402)
(45, 9.65703e-05)
(46, 5.68827e-05)
(47, 3.41162e-05)
(48, 2.01048e-05)
(49, 1.28003e-05)
(50, 7.24484e-06)
(51, 5.09833e-06)
(52, 3.07686e-06)
(53, 1.96368e-06)
(54, 1.18927e-06)
(55, 6.91013e-07)
(56, 3.12934e-07)
(57, 1.53712e-07)
(58, 6.79667e-08)
(59, 3.16718e-08)
(60, 1.36249e-08)
(61, 5.81022e-09)
(62, 2.68302e-09)
(63, 1.16564e-09)
(64, 5.60513e-10)
(65, 2.57259e-10)
(66, 1.23199e-10)
(67, 6.87882e-11)
(68, 3.10232e-11)
(69, 1.52656e-11)
(70, 6.94029e-12)
(71, 2.39141e-12)
(72, 1.17632e-12)
(73, 6.04559e-13)
(74, 3.41869e-13)
(75, 1.69421e-13)
(76, 6.16199e-14)
(77, 2.48632e-14)
(78, 1.06259e-14)
(79, 6.86654e-15)
(80, 5.87011e-15)
(81, 5.44162e-15)
}; \label{plot:fp64}
\addplot[ color=mydeepblue, line width=1.0pt, dashed] coordinates {
(0, 1)
(1, 0.508761)
(2, 0.44966)
(3, 0.349696)
(4, 0.291644)
(5, 0.268619)
(6, 0.223722)
(7, 0.242503)
(8, 0.231782)
(9, 0.138892)
(10, 0.11607)
(11, 0.0887681)
(12, 0.0779323)
(13, 0.0757631)
(14, 0.061475)
(15, 0.0545092)
(16, 0.048355)
(17, 0.0471564)
(18, 0.0392887)
(19, 0.0293365)
(20, 0.0340883)
(21, 0.0405514)
(22, 0.0398602)
(23, 0.0448877)
(24, 0.0515839)
(25, 0.062466)
(26, 0.0805603)
(27, 0.0753342)
(28, 0.0584599)
(29, 0.0419472)
(30, 0.040101)
(31, 0.0402179)
(32, 0.0328947)
(33, 0.0179779)
(34, 0.00953373)
(35, 0.00583711)
(36, 0.00400151)
(37, 0.00286008)
(38, 0.00208185)
(39, 0.00151107)
(40, 0.00101964)
(41, 0.000783152)
(42, 0.000545674)
(43, 0.000286461)
(44, 0.000161402)
(45, 9.65703e-05)
(46, 5.68827e-05)
(47, 3.41162e-05)
(48, 2.01048e-05)
(49, 1.28003e-05)
(50, 7.24484e-06)
(51, 5.09833e-06)
(52, 3.07686e-06)
(53, 1.96368e-06)
(54, 1.18927e-06)
(55, 6.91013e-07)
(56, 3.12934e-07)
(57, 1.53712e-07)
(58, 6.79667e-08)
(59, 3.16718e-08)
(60, 1.36249e-08)
(61, 5.81022e-09)
(62, 2.68302e-09)
(63, 1.16564e-09)
(64, 5.60514e-10)
(65, 2.5726e-10)
(66, 1.23201e-10)
(67, 6.87905e-11)
(68, 3.10308e-11)
(69, 1.52762e-11)
(70, 6.96707e-12)
(71, 2.44656e-12)
(72, 1.27626e-12)
(73, 7.34687e-13)
(74, 4.34154e-13)
(75, 2.3136e-13)
(76, 9.75192e-14)
(77, 4.00273e-14)
(78, 2.2516e-14)
(79, 1.73416e-14)
(80, 2.59457e-14)
(81, 2.97295e-14)
(82, 2.47602e-14)
(83, 1.35852e-14)
(84, 1.30088e-14)
(85, 1.92071e-14)
(86, 2.78449e-14)
(87, 2.14387e-14)
(88, 1.39945e-14)
(89, 1.68301e-14)
(90, 3.16969e-14)
(91, 3.29193e-14)
(92, 2.10591e-14)
(93, 1.61721e-14)
(94, 2.33833e-14)
(95, 2.42216e-14)
(96, 1.53573e-14)
(97, 1.18299e-14)
(98, 1.11016e-14)
(99, 1.08059e-14)
(100, 7.91535e-15)
}; \label{plot:fp64mixed}
\addplot[ color=mygreen, line width=1.0pt, dotted] coordinates {
(0, 1)
(1, 0.508761)
(2, 0.449663)
(3, 0.349701)
(4, 0.291626)
(5, 0.268615)
(6, 0.223726)
(7, 0.242459)
(8, 0.231744)
(9, 0.138955)
(10, 0.116091)
(11, 0.0887584)
(12, 0.0779365)
(13, 0.0757666)
(14, 0.0615014)
(15, 0.0545232)
(16, 0.0483377)
(17, 0.0471458)
(18, 0.0392601)
(19, 0.0293557)
(20, 0.034079)
(21, 0.0405421)
(22, 0.0398484)
(23, 0.0449017)
(24, 0.0515972)
(25, 0.0624052)
(26, 0.08048)
(27, 0.0753471)
(28, 0.0584667)
(29, 0.0419686)
(30, 0.0401287)
(31, 0.040251)
(32, 0.0329653)
(33, 0.0180942)
(34, 0.00963143)
(35, 0.00593691)
(36, 0.00413576)
(37, 0.00298374)
(38, 0.00241909)
(39, 0.00163325)
(40, 0.00109334)
(41, 0.000804596)
(42, 0.000582375)
(43, 0.000311442)
(44, 0.000177204)
(45, 0.000116689)
(46, 6.5735e-05)
(47, 4.28175e-05)
(48, 2.61878e-05)
(49, 2.10963e-05)
(50, 1.79167e-05)
(51, 2.0187e-05)
(52, 2.47305e-05)
(53, 2.84019e-05)
(54, 3.59054e-05)
(55, 3.49338e-05)
(56, 3.43485e-05)
(57, 3.08862e-05)
(58, 2.72622e-05)
(59, 2.29323e-05)
(60, 2.29822e-05)
(61, 3.32223e-05)
(62, 4.599e-05)
(63, 4.64507e-05)
(64, 3.04182e-05)
(65, 1.46621e-05)
(66, 7.69351e-06)
(67, 3.7112e-06)
(68, 2.4834e-06)
(69, 2.18936e-06)
(70, 2.40893e-06)
(71, 2.30059e-06)
(72, 1.65432e-06)
(73, 8.38712e-07)
(74, 4.84959e-07)
(75, 2.82044e-07)
(76, 2.14335e-07)
(77, 1.65884e-07)
(78, 1.17075e-07)
(79, 8.04973e-08)
(80, 5.07016e-08)
(81, 2.98267e-08)
(82, 1.81384e-08)
(83, 1.3907e-08)
(84, 1.52888e-08)
(85, 1.29976e-08)
(86, 8.03079e-09)
(87, 5.02487e-09)
(88, 4.7307e-09)
(89, 4.58893e-09)
(90, 5.65035e-09)
(91, 5.87443e-09)
(92, 6.90998e-09)
(93, 8.51198e-09)
(94, 7.56086e-09)
(95, 6.18728e-09)
(96, 5.31632e-09)
(97, 5.59548e-09)
(98, 6.33071e-09)
(99, 5.90316e-09)
(100, 9.23631e-09)
}; \label{plot:fp16}
\addplot[only marks, mark=x, color=red,   mark size=3pt, line width=1.5pt] coordinates {
(50, 7.24484e-06)
}; \label{plot:fp64tofp32}
\addplot[only marks,mark=x, color=black,   mark size=3pt,line width=1.5pt] coordinates {
(55, 6.91013e-07)
};\label{plot:fp32tofp16}
\addplot[only marks,  mark=o, color=blue,   mark size=3pt,line width=1.5pt] coordinates {
(61, 5.81022e-09)
};\label{plot:residualfp64tofp32} 





==> 5.Numerical/data/okCond_2_2.tex <==
\addplot[color=myyellow, line width=1.0pt] coordinates { 
(0, 1)
(1, 0.681568)
(2, 0.6116)
(3, 0.521932)
(4, 0.527948)
(5, 0.503438)
(6, 0.325529)
(7, 0.210832)
(8, 0.190517)
(9, 0.177036)
(10, 0.159594)
(11, 0.167152)
(12, 0.17431)
(13, 0.139829)
(14, 0.128789)
(15, 0.125414)
(16, 0.113435)
(17, 0.0999879)
(18, 0.092236)
(19, 0.0704062)
(20, 0.0580627)
(21, 0.058013)
(22, 0.045871)
(23, 0.0382201)
(24, 0.0387893)
(25, 0.0431711)
(26, 0.0370462)
(27, 0.0345881)
(28, 0.0313396)
(29, 0.0312144)
(30, 0.0319794)
(31, 0.0335025)
(32, 0.0321677)
(33, 0.0362448)
(34, 0.0385604)
(35, 0.0353065)
(36, 0.0384504)
(37, 0.0424632)
(38, 0.0408398)
(39, 0.0384249)
(40, 0.0406182)
(41, 0.0499357)
(42, 0.0513765)
(43, 0.041487)
(44, 0.0435903)
(45, 0.0422826)
(46, 0.0430387)
(47, 0.0454391)
(48, 0.0402987)
(49, 0.0285398)
(50, 0.0281085)
(51, 0.0305228)
(52, 0.0324275)
(53, 0.0332092)
(54, 0.0304166)
(55, 0.0286448)
(56, 0.0326135)
(57, 0.0361308)
(58, 0.0331682)
(59, 0.0272824)
(60, 0.025733)
(61, 0.020249)
(62, 0.0170552)
(63, 0.0172962)
(64, 0.0146849)
(65, 0.0112239)
(66, 0.0101619)
(67, 0.0097784)
(68, 0.00872151)
(69, 0.00645569)
(70, 0.00510935)
(71, 0.00466583)
(72, 0.00453858)
(73, 0.00440182)
(74, 0.00405334)
(75, 0.00364219)
(76, 0.00335539)
(77, 0.00353573)
(78, 0.00346986)
(79, 0.00300718)
(80, 0.0027545)
(81, 0.00224157)
(82, 0.00181056)
(83, 0.0013852)
(84, 0.00120047)
(85, 0.0011174)
(86, 0.000948172)
(87, 0.000796206)
(88, 0.000700024)
(89, 0.000544359)
(90, 0.000411195)
(91, 0.000294258)
(92, 0.000240449)
(93, 0.000187907)
(94, 0.000157868)
(95, 0.000137723)
(96, 0.000104924)
(97, 8.15283e-05)
(98, 7.58698e-05)
(99, 7.10544e-05)
(100, 6.10853e-05)
(101, 5.63456e-05)
(102, 5.08166e-05)
(103, 5.00438e-05)
(104, 4.96376e-05)
(105, 4.37422e-05)
(106, 3.39283e-05)
(107, 3.19694e-05)
(108, 3.20036e-05)
(109, 2.35297e-05)
(110, 1.83877e-05)
(111, 1.38536e-05)
(112, 1.04085e-05)
(113, 8.97587e-06)
(114, 8.12891e-06)
(115, 6.90245e-06)
(116, 5.68196e-06)
(117, 4.52655e-06)
(118, 3.2706e-06)
(119, 2.49739e-06)
(120, 2.31156e-06)
(121, 2.42444e-06)
(122, 2.45024e-06)
(123, 2.31458e-06)
(124, 2.02281e-06)
(125, 1.92237e-06)
(126, 1.84812e-06)
(127, 1.80263e-06)
(128, 1.74287e-06)
(129, 1.566e-06)
(130, 1.31267e-06)
(131, 1.12574e-06)
(132, 1.02863e-06)
(133, 9.43943e-07)
(134, 8.15228e-07)
(135, 6.50087e-07)
(136, 5.2092e-07)
(137, 4.55738e-07)
(138, 3.73483e-07)
(139, 2.85252e-07)
(140, 2.46108e-07)
(141, 2.06638e-07)
(142, 1.6108e-07)
(143, 1.34777e-07)
(144, 1.32837e-07)
(145, 1.22626e-07)
(146, 9.94415e-08)
(147, 9.55179e-08)
(148, 8.68929e-08)
(149, 7.1121e-08)
(150, 6.85154e-08)
(151, 6.9839e-08)
(152, 5.88546e-08)
(153, 4.69494e-08)
(154, 4.14622e-08)
(155, 3.8003e-08)
(156, 3.15766e-08)
(157, 2.96831e-08)
(158, 2.65674e-08)
(159, 2.1999e-08)
(160, 1.64667e-08)
(161, 1.38051e-08)
(162, 1.17904e-08)
(163, 1.02705e-08)
(164, 8.42101e-09)
(165, 7.35195e-09)
(166, 6.22901e-09)
(167, 4.75387e-09)
(168, 3.82605e-09)
(169, 3.72588e-09)
(170, 3.59672e-09)
(171, 2.81256e-09)
(172, 2.1866e-09)
(173, 1.74983e-09)
(174, 1.36671e-09)
(175, 1.05666e-09)
(176, 9.7262e-10)
(177, 9.48515e-10)
(178, 8.11829e-10)
(179, 6.04381e-10)
(180, 4.63354e-10)
(181, 3.35548e-10)
(182, 2.77481e-10)
(183, 2.74415e-10)
(184, 2.73202e-10)
(185, 2.3525e-10)
(186, 1.92645e-10)
(187, 1.74083e-10)
(188, 1.82797e-10)
(189, 1.97583e-10)
(190, 2.14017e-10)
(191, 2.07123e-10)
(192, 1.88558e-10)
(193, 1.61744e-10)
(194, 1.32162e-10)
(195, 1.17768e-10)
(196, 9.48508e-11)
}; \label{plot:fp64} 
\addplot[ color=mygreen, line width=1.0pt, dotted] coordinates { 
(0, 1)
(1, 0.681568)
(2, 0.61159)
(3, 0.521931)
(4, 0.527971)
(5, 0.503432)
(6, 0.325577)
(7, 0.210899)
(8, 0.190549)
(9, 0.177021)
(10, 0.159581)
(11, 0.167148)
(12, 0.17451)
(13, 0.140482)
(14, 0.130824)
(15, 0.135987)
(16, 0.130005)
(17, 0.109079)
(18, 0.0933794)
(19, 0.0750098)
(20, 0.0626601)
(21, 0.0614663)
(22, 0.0552618)
(23, 0.040074)
(24, 0.0384704)
(25, 0.0417574)
(26, 0.0458347)
(27, 0.0391185)
(28, 0.03441)
(29, 0.0323887)
(30, 0.032262)
(31, 0.0325897)
(32, 0.0326604)
(33, 0.0330966)
(34, 0.036279)
(35, 0.0395868)
(36, 0.0407822)
(37, 0.0391233)
(38, 0.0451208)
(39, 0.0449533)
(40, 0.0426389)
(41, 0.0388936)
(42, 0.0414605)
(43, 0.0458215)
(44, 0.0460197)
(45, 0.0444062)
(46, 0.0440536)
(47, 0.0422676)
(48, 0.0503502)
(49, 0.0482798)
(50, 0.0481631)
(51, 0.0372749)
(52, 0.0286519)
(53, 0.0285609)
(54, 0.0315481)
(55, 0.0330484)
(56, 0.0322109)
(57, 0.0306979)
(58, 0.0290366)
(59, 0.0341703)
(60, 0.0420796)
(61, 0.0383463)
(62, 0.0308352)
(63, 0.0269162)
(64, 0.0249819)
(65, 0.0191882)
(66, 0.0173433)
(67, 0.017394)
(68, 0.015154)
(69, 0.0112603)
(70, 0.0098073)
(71, 0.0102378)
(72, 0.00956725)
(73, 0.00778699)
(74, 0.00576321)
(75, 0.00484956)
(76, 0.0046053)
(77, 0.0045186)
(78, 0.00431782)
(79, 0.0036049)
(80, 0.00327643)
(81, 0.00342723)
(82, 0.00376623)
(83, 0.00344068)
(84, 0.00281883)
(85, 0.00257956)
(86, 0.00203942)
(87, 0.00158306)
(88, 0.00127671)
(89, 0.00123008)
(90, 0.00117237)
(91, 0.000940265)
(92, 0.00082199)
(93, 0.000718063)
(94, 0.000579854)
(95, 0.000440098)
(96, 0.00035398)
(97, 0.000268262)
(98, 0.000216428)
(99, 0.000180616)
(100, 0.000154714)
(101, 0.000147957)
(102, 0.000121494)
(103, 8.87788e-05)
(104, 7.44025e-05)
(105, 7.4163e-05)
(106, 6.87887e-05)
(107, 6.22304e-05)
(108, 5.45915e-05)
(109, 5.24004e-05)
(110, 5.06181e-05)
(111, 5.0865e-05)
(112, 4.82505e-05)
(113, 4.17131e-05)
(114, 3.17311e-05)
(115, 2.65851e-05)
(116, 2.42431e-05)
(117, 1.89389e-05)
(118, 1.54488e-05)
(119, 1.26862e-05)
(120, 9.94807e-06)
(121, 9.0517e-06)
(122, 8.22506e-06)
(123, 7.66058e-06)
(124, 6.83064e-06)
(125, 6.30049e-06)
(126, 5.56568e-06)
(127, 4.98528e-06)
(128, 5.2535e-06)
(129, 6.4124e-06)
(130, 7.49007e-06)
(131, 7.79864e-06)
(132, 8.24173e-06)
(133, 9.0801e-06)
(134, 1.01495e-05)
(135, 1.0031e-05)
(136, 1.06083e-05)
(137, 1.17034e-05)
(138, 1.0054e-05)
(139, 8.78177e-06)
(140, 8.18822e-06)
(141, 8.48671e-06)
(142, 8.8868e-06)
(143, 8.62258e-06)
(144, 8.25532e-06)
(145, 7.69994e-06)
(146, 8.02174e-06)
(147, 8.7615e-06)
(148, 8.96675e-06)
(149, 8.56282e-06)
(150, 8.80943e-06)
(151, 8.71319e-06)
(152, 8.19705e-06)
(153, 7.71588e-06)
(154, 7.76815e-06)
(155, 7.15334e-06)
(156, 6.29553e-06)
(157, 6.06206e-06)
(158, 5.18555e-06)
(159, 4.03469e-06)
(160, 3.38673e-06)
(161, 3.20109e-06)
(162, 2.71676e-06)
(163, 1.87793e-06)
(164, 1.57192e-06)
(165, 1.60813e-06)
(166, 1.55491e-06)
(167, 1.4643e-06)
(168, 1.24942e-06)
(169, 1.06816e-06)
(170, 8.99544e-07)
(171, 7.54793e-07)
(172, 6.72944e-07)
(173, 6.51472e-07)
(174, 6.01328e-07)
(175, 5.07879e-07)
(176, 4.96075e-07)
(177, 4.74615e-07)
(178, 3.89154e-07)
(179, 3.36338e-07)
(180, 2.99406e-07)
(181, 2.91864e-07)
(182, 2.50758e-07)
(183, 1.97975e-07)
(184, 1.54188e-07)
(185, 1.3421e-07)
(186, 1.35847e-07)
(187, 1.27622e-07)
(188, 1.08163e-07)
(189, 9.59907e-08)
(190, 7.88209e-08)
(191, 6.03697e-08)
(192, 4.81847e-08)
(193, 4.37939e-08)
(194, 4.02862e-08)
(195, 4.22581e-08)
(196, 3.38673e-08)
(197, 2.26236e-08)
(198, 1.59557e-08)
(199, 1.28873e-08)
(200, 1.15161e-08)
(201, 1.02202e-08)
(202, 9.10267e-09)
(203, 7.71832e-09)
(204, 6.42051e-09)
(205, 5.6067e-09)
(206, 4.53778e-09)
(207, 4.23101e-09)
(208, 4.5622e-09)
(209, 4.57359e-09)
(210, 4.40653e-09)
(211, 4.14877e-09)
(212, 4.43573e-09)
(213, 5.18813e-09)
(214, 5.08013e-09)
(215, 4.5964e-09)
(216, 3.79617e-09)
(217, 3.14923e-09)
(218, 2.95799e-09)
(219, 2.47875e-09)
(220, 1.87314e-09)
(221, 1.47353e-09)
(222, 1.34711e-09)
(223, 1.3631e-09)
(224, 1.335e-09)
(225, 1.35823e-09)
(226, 1.29684e-09)
(227, 1.31603e-09)
(228, 1.51113e-09)
(229, 1.77268e-09)
(230, 2.22992e-09)
(231, 2.64105e-09)
(232, 2.7242e-09)
(233, 2.64171e-09)
(234, 2.58378e-09)
(235, 2.64478e-09)
(236, 2.81361e-09)
(237, 2.64396e-09)
(238, 2.39317e-09)
(239, 2.30102e-09)
(240, 2.12883e-09)
(241, 1.80125e-09)
(242, 1.47046e-09)
(243, 1.19896e-09)
(244, 1.2399e-09)
(245, 1.45705e-09)
(246, 1.5971e-09)
(247, 1.82238e-09)
(248, 1.89095e-09)
(249, 1.74908e-09)
(250, 1.71896e-09)
(251, 1.66944e-09)
(252, 1.50853e-09)
(253, 1.53477e-09)
(254, 1.34796e-09)
(255, 9.78715e-10)
(256, 6.52834e-10)
(257, 5.4246e-10)
(258, 5.57983e-10)
(259, 5.79644e-10)
(260, 4.80923e-10)
(261, 3.40041e-10)
(262, 2.29265e-10)
(263, 1.98445e-10)
(264, 1.84025e-10)
(265, 1.89895e-10)
(266, 2.05313e-10)
(267, 1.75091e-10)
(268, 1.61257e-10)
(269, 1.30556e-10)
(270, 1.18816e-10)
(271, 1.18481e-10)
(272, 1.40846e-10)
(273, 1.27167e-10)
(274, 9.90458e-11)
}; \label{plot:fp16} 
\addplot[color=mydeepblue, line width=1.0pt, dashed] coordinates { 
(0, 1)
(1, 0.681568)
(2, 0.6116)
(3, 0.521932)
(4, 0.527948)
(5, 0.503438)
(6, 0.325529)
(7, 0.210832)
(8, 0.190517)
(9, 0.177036)
(10, 0.159594)
(11, 0.167152)
(12, 0.17431)
(13, 0.139829)
(14, 0.128789)
(15, 0.125414)
(16, 0.113435)
(17, 0.0999879)
(18, 0.092236)
(19, 0.0704062)
(20, 0.0580627)
(21, 0.058013)
(22, 0.045871)
(23, 0.0382201)
(24, 0.0387893)
(25, 0.0431711)
(26, 0.0370462)
(27, 0.0345881)
(28, 0.0313396)
(29, 0.0312144)
(30, 0.0319794)
(31, 0.0335025)
(32, 0.0321677)
(33, 0.0362448)
(34, 0.0385604)
(35, 0.0353065)
(36, 0.0384504)
(37, 0.0424631)
(38, 0.0408381)
(39, 0.0384103)
(40, 0.040525)
(41, 0.0495543)
(42, 0.0518671)
(43, 0.0415673)
(44, 0.0435966)
(45, 0.0422835)
(46, 0.0430388)
(47, 0.0454391)
(48, 0.0402987)
(49, 0.0285398)
(50, 0.0281085)
(51, 0.0305228)
(52, 0.0324275)
(53, 0.0332092)
(54, 0.0304166)
(55, 0.0286448)
(56, 0.0326135)
(57, 0.0361308)
(58, 0.0331682)
(59, 0.0272825)
(60, 0.0257337)
(61, 0.0202522)
(62, 0.0170672)
(63, 0.0173657)
(64, 0.0151872)
(65, 0.011924)
(66, 0.0100806)
(67, 0.00944218)
(68, 0.00864265)
(69, 0.00644889)
(70, 0.00511088)
(71, 0.00467774)
(72, 0.00460743)
(73, 0.00473735)
(74, 0.00415117)
(75, 0.00360447)
(76, 0.00342526)
(77, 0.00335851)
(78, 0.00339737)
(79, 0.0029931)
(80, 0.00275387)
(81, 0.00224785)
(82, 0.00183232)
(83, 0.00142705)
(84, 0.00125449)
(85, 0.00113521)
(86, 0.000926294)
(87, 0.000784948)
(88, 0.000697735)
(89, 0.000543852)
(90, 0.00041112)
(91, 0.000294246)
(92, 0.000240446)
(93, 0.000187907)
(94, 0.000157868)
(95, 0.000137723)
(96, 0.000104924)
(97, 8.15283e-05)
(98, 7.58698e-05)
(99, 7.10544e-05)
(100, 6.10853e-05)
(101, 5.63456e-05)
(102, 5.08167e-05)
(103, 5.0045e-05)
(104, 4.96523e-05)
(105, 4.3908e-05)
(106, 3.54377e-05)
(107, 3.47917e-05)
(108, 2.95674e-05)
(109, 2.31862e-05)
(110, 1.83544e-05)
(111, 1.3829e-05)
(112, 1.03529e-05)
(113, 8.85608e-06)
(114, 8.01579e-06)
(115, 6.82358e-06)
(116, 5.68122e-06)
(117, 4.55402e-06)
(118, 3.28711e-06)
(119, 2.53823e-06)
(120, 2.44336e-06)
(121, 2.55352e-06)
(122, 2.45592e-06)
(123, 2.21446e-06)
(124, 1.97574e-06)
(125, 2.16824e-06)
(126, 2.20088e-06)
(127, 1.80979e-06)
(128, 1.83014e-06)
(129, 1.80762e-06)
(130, 1.62923e-06)
(131, 1.33883e-06)
(132, 1.1022e-06)
(133, 9.49264e-07)
(134, 8.41296e-07)
(135, 7.33056e-07)
(136, 5.78962e-07)
(137, 4.93567e-07)
(138, 4.35779e-07)
(139, 3.58219e-07)
(140, 2.95875e-07)
(141, 2.60638e-07)
(142, 2.47165e-07)
(143, 1.88905e-07)
(144, 1.44561e-07)
(145, 1.23401e-07)
(146, 1.08713e-07)
(147, 9.48622e-08)
(148, 9.30448e-08)
(149, 9.14465e-08)
(150, 7.9437e-08)
(151, 7.19496e-08)
(152, 7.82366e-08)
(153, 7.03609e-08)
(154, 5.33398e-08)
(155, 4.18334e-08)
(156, 3.85859e-08)
(157, 3.62662e-08)
(158, 3.20634e-08)
(159, 3.11932e-08)
(160, 2.78522e-08)
(161, 2.50051e-08)
(162, 2.00257e-08)
(163, 1.48575e-08)
(164, 1.28643e-08)
(165, 1.12108e-08)
(166, 9.59926e-09)
(167, 8.08359e-09)
(168, 7.5204e-09)
(169, 6.09854e-09)
(170, 5.15442e-09)
(171, 4.4113e-09)
(172, 3.63987e-09)
(173, 3.64387e-09)
(174, 3.03068e-09)
(175, 2.28039e-09)
(176, 1.89499e-09)
(177, 1.63036e-09)
(178, 1.26334e-09)
(179, 1.01387e-09)
(180, 9.64824e-10)
(181, 8.32844e-10)
(182, 7.15414e-10)
(183, 5.84071e-10)
(184, 4.00628e-10)
(185, 2.82763e-10)
(186, 2.73907e-10)
(187, 2.94822e-10)
(188, 2.83501e-10)
(189, 2.35399e-10)
(190, 1.91974e-10)
(191, 1.74053e-10)
(192, 1.83982e-10)
(193, 2.00111e-10)
(194, 2.17015e-10)
(195, 2.12509e-10)
(196, 1.85968e-10)
(197, 1.64933e-10)
(198, 1.47585e-10)
(199, 1.35003e-10)
(200, 1.10095e-10)
(201, 8.35009e-11)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=x, color=red, mark size=3pt, line width=1.5pt] coordinates { 
 (97, 0.000104924) 
}; \label{plot:fp32tofp16} 
 \addplot[only marks, mark=x, color=black, mark size=3pt, line width=1.5pt] coordinates { 
 (133, 1.1022e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=o, mark size=3pt, color=blue, line width=1.0pt] coordinates { 
 (120, 2.53823e-06) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/okCond_2_res.tex <==
\addplot[color=myyellow, line width=1.0pt] coordinates { 
(0, 1)
(1, 0.0863842)
(2, 0.0983036)
(3, 0.0449711)
(4, 0.033689)
(5, 0.0259928)
(6, 0.013564)
(7, 0.0106732)
(8, 0.00436318)
(9, 0.00439181)
(10, 0.0025118)
(11, 0.00176127)
(12, 0.00097145)
(13, 0.00112778)
(14, 0.00144348)
(15, 0.00241814)
(16, 0.00380538)
(17, 0.00683736)
(18, 0.0100275)
(19, 0.0158171)
(20, 0.0201795)
(21, 0.0263859)
(22, 0.0301931)
(23, 0.0254603)
(24, 0.0214222)
(25, 0.0160478)
(26, 0.0148486)
(27, 0.0206199)
(28, 0.03409)
(29, 0.0366507)
(30, 0.0270341)
(31, 0.0198461)
(32, 0.0220075)
(33, 0.0190393)
(34, 0.0277447)
(35, 0.0259836)
(36, 0.0278785)
(37, 0.0283952)
(38, 0.0299492)
(39, 0.0310101)
(40, 0.0334878)
(41, 0.0434039)
(42, 0.0464134)
(43, 0.0507541)
(44, 0.0491429)
(45, 0.0579679)
(46, 0.0724889)
(47, 0.102809)
(48, 0.135016)
(49, 0.135459)
(50, 0.14576)
(51, 0.196335)
(52, 0.202924)
(53, 0.194249)
(54, 0.13598)
(55, 0.0950816)
(56, 0.0802758)
(57, 0.0590886)
(58, 0.047177)
(59, 0.0391927)
(60, 0.0249646)
(61, 0.0162851)
(62, 0.0122572)
(63, 0.00920036)
(64, 0.00570305)
(65, 0.00348975)
(66, 0.00209996)
(67, 0.00114438)
(68, 0.000830539)
(69, 0.000711579)
(70, 0.000611439)
(71, 0.000382451)
(72, 0.000258637)
(73, 0.000129812)
(74, 8.93638e-05)
(75, 5.28728e-05)
(76, 3.86444e-05)
(77, 2.49692e-05)
(78, 1.51632e-05)
(79, 9.30836e-06)
(80, 4.62493e-06)
(81, 3.14587e-06)
(82, 1.71748e-06)
(83, 1.25372e-06)
(84, 6.6265e-07)
(85, 3.86144e-07)
(86, 2.06437e-07)
(87, 1.25254e-07)
(88, 7.20137e-08)
(89, 3.61535e-08)
(90, 2.13287e-08)
(91, 1.42904e-08)
(92, 1.15626e-08)
(93, 6.9716e-09)
(94, 3.63502e-09)
(95, 1.39162e-09)
(96, 5.90018e-10)
(97, 2.56781e-10)
(98, 1.45756e-10)
(99, 9.05685e-11)
(100, 6.25545e-11)
(101, 3.33439e-11)
(102, 2.1258e-11)
(103, 1.05188e-11)
(104, 5.63981e-12)
(105, 3.51901e-12)
(106, 2.69938e-12)
(107, 1.82497e-12)
(108, 6.00667e-13)
(109, 3.16405e-13)
(110, 1.99137e-13)
(111, 1.46211e-13)
(112, 1.00107e-13)
(113, 7.61974e-14)
(114, 1.08716e-13)
(115, 1.9473e-13)
(116, 3.23055e-13)
(117, 3.09068e-13)
(118, 1.93947e-13)
(119, 1.37388e-13)
(120, 9.52712e-14)
(121, 6.09561e-14)
(122, 8.24513e-14)
(123, 1.26038e-13)
(124, 1.45909e-13)
(125, 8.54911e-14)
(126, 4.14234e-14)
(127, 1.94369e-14)
(128, 1.05114e-14)
(129, 5.43919e-15)
(130, 3.27083e-15)
(131, 2.44618e-15)
(132, 2.78943e-15)
(133, 3.54671e-15)
(134, 3.10487e-15)
(135, 2.07598e-15)
(136, 1.1835e-15)
(137, 7.52967e-16)
}; \label{plot:fp64} 
\addplot[ color=mygreen, line width=1.0pt, dotted] coordinates { 
(0, 1)
(1, 0.0863842)
(2, 0.0983178)
(3, 0.0449742)
(4, 0.0336921)
(5, 0.0259981)
(6, 0.0135711)
(7, 0.0106814)
(8, 0.004363)
(9, 0.00439304)
(10, 0.00251243)
(11, 0.00176258)
(12, 0.000971175)
(13, 0.00112837)
(14, 0.00144336)
(15, 0.00242062)
(16, 0.00380643)
(17, 0.00684088)
(18, 0.0100224)
(19, 0.0158163)
(20, 0.0201836)
(21, 0.0263944)
(22, 0.0302536)
(23, 0.0254992)
(24, 0.0214696)
(25, 0.0160414)
(26, 0.0148449)
(27, 0.0206921)
(28, 0.0342201)
(29, 0.0368306)
(30, 0.0272254)
(31, 0.0200601)
(32, 0.0222054)
(33, 0.0190523)
(34, 0.0272214)
(35, 0.0259583)
(36, 0.0278462)
(37, 0.0285769)
(38, 0.0298471)
(39, 0.0308077)
(40, 0.0331101)
(41, 0.0429583)
(42, 0.0458453)
(43, 0.0505955)
(44, 0.0494328)
(45, 0.0577913)
(46, 0.0721381)
(47, 0.0971237)
(48, 0.135333)
(49, 0.126257)
(50, 0.145353)
(51, 0.187315)
(52, 0.214848)
(53, 0.203357)
(54, 0.156524)
(55, 0.110798)
(56, 0.089)
(57, 0.0775954)
(58, 0.0596542)
(59, 0.0473743)
(60, 0.0386595)
(61, 0.0250278)
(62, 0.0177406)
(63, 0.0142925)
(64, 0.0112486)
(65, 0.00811931)
(66, 0.00574584)
(67, 0.00484504)
(68, 0.00470984)
(69, 0.00521986)
(70, 0.00650079)
(71, 0.00630612)
(72, 0.00471246)
(73, 0.00358549)
(74, 0.00315548)
(75, 0.00287142)
(76, 0.00276004)
(77, 0.00208592)
(78, 0.0018843)
(79, 0.00165414)
(80, 0.00171461)
(81, 0.00195043)
(82, 0.00214367)
(83, 0.00241672)
(84, 0.0025729)
(85, 0.00276626)
(86, 0.00294306)
(87, 0.00255383)
(88, 0.00246761)
(89, 0.00202173)
(90, 0.00194334)
(91, 0.00202011)
(92, 0.00193366)
(93, 0.00189)
(94, 0.00160035)
(95, 0.00137785)
(96, 0.00100388)
(97, 0.000725585)
(98, 0.000566387)
(99, 0.000497851)
(100, 0.000410584)
(101, 0.000322343)
(102, 0.000268873)
(103, 0.000246738)
(104, 0.000193087)
(105, 0.000139315)
(106, 9.71584e-05)
(107, 9.22054e-05)
(108, 0.000126637)
(109, 0.00018436)
(110, 0.000209091)
(111, 0.000270271)
(112, 0.000365642)
(113, 0.000467719)
(114, 0.000506946)
(115, 0.000514431)
(116, 0.000586458)
(117, 0.000548085)
(118, 0.000503034)
(119, 0.000492219)
(120, 0.000593627)
(121, 0.000778939)
(122, 0.00111537)
(123, 0.00161967)
(124, 0.00181296)
(125, 0.0018657)
(126, 0.00245003)
(127, 0.00366543)
(128, 0.00384907)
(129, 0.0037764)
(130, 0.00395972)
(131, 0.00403763)
(132, 0.00386055)
(133, 0.00294176)
(134, 0.00276697)
(135, 0.00246929)
(136, 0.00234921)
(137, 0.00228865)
(138, 0.0022569)
(139, 0.00282013)
(140, 0.00278576)
(141, 0.00304247)
(142, 0.00354162)
(143, 0.00331069)
(144, 0.00321244)
(145, 0.0039996)
(146, 0.0058207)
(147, 0.00748623)
(148, 0.00782387)
(149, 0.00817518)
(150, 0.00905863)
(151, 0.0102683)
(152, 0.0122433)
(153, 0.0138148)
(154, 0.0125885)
(155, 0.0112795)
(156, 0.0108358)
(157, 0.00948797)
(158, 0.0075231)
(159, 0.00540897)
(160, 0.00364119)
(161, 0.00301614)
(162, 0.00269391)
(163, 0.00247261)
(164, 0.00265848)
(165, 0.00253712)
(166, 0.00244186)
(167, 0.00238952)
(168, 0.00243463)
(169, 0.00201493)
(170, 0.00152442)
(171, 0.00126446)
(172, 0.000787534)
(173, 0.000511989)
(174, 0.000346395)
(175, 0.000263757)
(176, 0.000272837)
(177, 0.000265839)
(178, 0.000279315)
(179, 0.000253643)
(180, 0.000233129)
(181, 0.000235789)
(182, 0.000229001)
(183, 0.000266148)
(184, 0.000355635)
(185, 0.000404884)
(186, 0.000383791)
(187, 0.000366604)
(188, 0.000331839)
(189, 0.000281712)
(190, 0.000262314)
(191, 0.000265309)
(192, 0.00025454)
(193, 0.000226629)
(194, 0.000216566)
(195, 0.000189314)
(196, 0.000154261)
(197, 0.000118645)
(198, 0.000102163)
(199, 9.42869e-05)
(200, 8.25776e-05)
(201, 5.83679e-05)
(202, 5.10209e-05)
(203, 4.64029e-05)
(204, 4.09373e-05)
(205, 3.6373e-05)
(206, 3.36389e-05)
(207, 3.37443e-05)
(208, 4.06361e-05)
(209, 3.87046e-05)
(210, 3.0783e-05)
(211, 2.25511e-05)
(212, 1.98733e-05)
(213, 1.92588e-05)
(214, 1.62932e-05)
(215, 1.41196e-05)
(216, 1.2897e-05)
(217, 1.29985e-05)
(218, 1.73091e-05)
(219, 2.22135e-05)
(220, 3.38345e-05)
(221, 4.61262e-05)
(222, 5.46357e-05)
(223, 6.23552e-05)
(224, 7.99394e-05)
(225, 0.000104137)
(226, 0.000128287)
(227, 0.000150836)
(228, 0.000166421)
(229, 0.000164585)
(230, 0.000165426)
(231, 0.000132143)
(232, 0.000122442)
(233, 0.000129132)
(234, 0.000111217)
(235, 0.000103933)
(236, 0.000124144)
(237, 0.000143601)
(238, 0.00014485)
(239, 0.000122367)
(240, 0.000113489)
(241, 0.00013506)
(242, 0.000153674)
(243, 0.000176442)
(244, 0.0001699)
(245, 0.000172576)
(246, 0.000189816)
(247, 0.000199537)
(248, 0.000221545)
(249, 0.000228375)
(250, 0.000254037)
(251, 0.000333782)
(252, 0.000403427)
(253, 0.000489381)
(254, 0.00052281)
(255, 0.000466062)
(256, 0.000416283)
(257, 0.000489532)
(258, 0.000613779)
(259, 0.000880184)
(260, 0.00113458)
(261, 0.00128119)
(262, 0.00143084)
(263, 0.00166536)
(264, 0.00172777)
(265, 0.00139501)
(266, 0.000919986)
(267, 0.000688043)
(268, 0.000519287)
(269, 0.000379379)
(270, 0.000310958)
(271, 0.000283655)
(272, 0.000227619)
(273, 0.000190243)
(274, 0.000162972)
(275, 0.000138209)
(276, 0.000112957)
(277, 0.000117894)
(278, 0.000118148)
(279, 0.000111601)
(280, 0.000104954)
(281, 9.30422e-05)
(282, 8.23987e-05)
(283, 8.08872e-05)
(284, 6.50962e-05)
(285, 5.63608e-05)
(286, 4.89319e-05)
(287, 4.14056e-05)
(288, 3.53114e-05)
(289, 2.89445e-05)
(290, 3.33479e-05)
(291, 3.87418e-05)
(292, 3.69621e-05)
(293, 3.72364e-05)
(294, 3.60332e-05)
(295, 3.66084e-05)
(296, 4.016e-05)
(297, 3.84028e-05)
(298, 3.85897e-05)
(299, 4.23919e-05)
(300, 4.32496e-05)
(301, 4.07009e-05)
(302, 3.76773e-05)
(303, 3.55073e-05)
(304, 3.49802e-05)
(305, 3.55001e-05)
(306, 2.86511e-05)
(307, 2.48812e-05)
(308, 2.17384e-05)
(309, 1.82686e-05)
(310, 1.33985e-05)
(311, 9.51395e-06)
(312, 5.60445e-06)
(313, 3.82543e-06)
(314, 2.94126e-06)
(315, 3.0638e-06)
(316, 2.89812e-06)
(317, 2.9001e-06)
(318, 2.7948e-06)
(319, 2.84159e-06)
(320, 3.27011e-06)
(321, 3.75323e-06)
(322, 3.74702e-06)
(323, 3.73601e-06)
(324, 3.41622e-06)
(325, 2.79052e-06)
(326, 2.53073e-06)
(327, 2.90004e-06)
(328, 3.75776e-06)
(329, 4.06635e-06)
(330, 4.44961e-06)
(331, 5.48581e-06)
(332, 6.0375e-06)
(333, 7.76043e-06)
(334, 1.05074e-05)
(335, 1.38234e-05)
(336, 1.71601e-05)
(337, 1.90281e-05)
(338, 2.31651e-05)
}; \label{plot:fp16} 
\addplot[color=mydeepblue, line width=1.0pt, dashed] coordinates { 
(0, 1)
(1, 0.0863842)
(2, 0.0983036)
(3, 0.0449711)
(4, 0.033689)
(5, 0.0259928)
(6, 0.013564)
(7, 0.0106732)
(8, 0.00436318)
(9, 0.00439181)
(10, 0.0025118)
(11, 0.00176127)
(12, 0.00097145)
(13, 0.00112778)
(14, 0.00144348)
(15, 0.00241814)
(16, 0.00380538)
(17, 0.00683736)
(18, 0.0100275)
(19, 0.0158171)
(20, 0.0201795)
(21, 0.0263859)
(22, 0.0301931)
(23, 0.0254603)
(24, 0.0214222)
(25, 0.0160478)
(26, 0.0148486)
(27, 0.0206199)
(28, 0.03409)
(29, 0.0366507)
(30, 0.0270341)
(31, 0.0198461)
(32, 0.0220075)
(33, 0.0190393)
(34, 0.0277447)
(35, 0.0259836)
(36, 0.0278785)
(37, 0.0283952)
(38, 0.0299492)
(39, 0.0310101)
(40, 0.0334878)
(41, 0.0434039)
(42, 0.0464134)
(43, 0.0507541)
(44, 0.0491429)
(45, 0.0579679)
(46, 0.0724889)
(47, 0.102809)
(48, 0.135016)
(49, 0.135459)
(50, 0.14576)
(51, 0.196335)
(52, 0.202924)
(53, 0.194249)
(54, 0.13598)
(55, 0.0950816)
(56, 0.0802758)
(57, 0.0590886)
(58, 0.047177)
(59, 0.0391927)
(60, 0.0249646)
(61, 0.0162851)
(62, 0.0122572)
(63, 0.00920036)
(64, 0.00570305)
(65, 0.00348975)
(66, 0.00209996)
(67, 0.00114438)
(68, 0.000830539)
(69, 0.000711579)
(70, 0.000611439)
(71, 0.000382451)
(72, 0.000258637)
(73, 0.000129812)
(74, 8.93638e-05)
(75, 5.28728e-05)
(76, 3.86444e-05)
(77, 2.49692e-05)
(78, 1.51632e-05)
(79, 9.30836e-06)
(80, 4.62493e-06)
(81, 3.14587e-06)
(82, 1.71748e-06)
(83, 1.25372e-06)
(84, 6.6265e-07)
(85, 3.86144e-07)
(86, 2.06437e-07)
(87, 1.25254e-07)
(88, 7.20137e-08)
(89, 3.61535e-08)
(90, 2.13287e-08)
(91, 1.42904e-08)
(92, 1.15626e-08)
(93, 6.9716e-09)
(94, 3.63503e-09)
(95, 1.39162e-09)
(96, 5.90022e-10)
(97, 2.56785e-10)
(98, 1.45763e-10)
(99, 9.05856e-11)
(100, 6.25803e-11)
(101, 3.33729e-11)
(102, 2.13157e-11)
(103, 1.05818e-11)
(104, 5.71331e-12)
(105, 3.72954e-12)
(106, 2.96487e-12)
(107, 1.88372e-12)
(108, 6.04555e-13)
(109, 3.12585e-13)
(110, 1.89324e-13)
(111, 1.28359e-13)
(112, 7.34769e-14)
(113, 3.44797e-14)
(114, 2.2478e-14)
(115, 2.25755e-14)
(116, 3.35418e-14)
(117, 6.09458e-14)
(118, 6.85105e-14)
(119, 5.77324e-14)
(120, 4.62893e-14)
(121, 2.51432e-14)
(122, 2.46727e-14)
(123, 3.12065e-14)
(124, 6.0789e-14)
(125, 4.78091e-14)
(126, 2.78705e-14)
(127, 1.84622e-14)
(128, 1.87675e-14)
(129, 2.17208e-14)
(130, 2.0075e-14)
(131, 1.81921e-14)
(132, 1.38562e-14)
(133, 9.97171e-15)
(134, 8.18451e-15)
(135, 8.70915e-15)
(136, 8.73107e-15)
(137, 6.54458e-15)
(138, 3.68397e-15)
(139, 2.32675e-15)
(140, 1.19355e-15)
(141, 1.22878e-15)
(142, 1.14254e-15)
(143, 9.9522e-16)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=x, color=red,   mark size=3pt, line width=1.5pt] coordinates { 
 (74, 0.000129812) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=x, color=black,   mark size=3pt, line width=1.5pt] coordinates { 
 (84, 1.25372e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=o, color=blue,    mark size=3pt,line width=1.0pt] coordinates { 
 (93, 1.15626e-08) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/okCond_2_trueRes.tex <==
\addplot[color=myyellow, line width=1.5pt] coordinates { 
(0, 1)
(1, 0.0863842)
(2, 0.0983036)
(3, 0.0449711)
(4, 0.033689)
(5, 0.0259928)
(6, 0.013564)
(7, 0.0106732)
(8, 0.00436318)
(9, 0.00439181)
(10, 0.0025118)
(11, 0.00176127)
(12, 0.00097145)
(13, 0.00112778)
(14, 0.00144348)
(15, 0.00241814)
(16, 0.00380538)
(17, 0.00683736)
(18, 0.0100275)
(19, 0.0158171)
(20, 0.0201795)
(21, 0.0263859)
(22, 0.0301931)
(23, 0.0254603)
(24, 0.0214222)
(25, 0.0160478)
(26, 0.0148486)
(27, 0.0206199)
(28, 0.03409)
(29, 0.0366507)
(30, 0.0270341)
(31, 0.0198461)
(32, 0.0220075)
(33, 0.0190393)
(34, 0.0277447)
(35, 0.0259836)
(36, 0.0278785)
(37, 0.0283952)
(38, 0.0299492)
(39, 0.0310101)
(40, 0.0334878)
(41, 0.0434039)
(42, 0.0464134)
(43, 0.0507541)
(44, 0.0491429)
(45, 0.0579679)
(46, 0.0724889)
(47, 0.102809)
(48, 0.135016)
(49, 0.135459)
(50, 0.14576)
(51, 0.196335)
(52, 0.202924)
(53, 0.194249)
(54, 0.13598)
(55, 0.0950816)
(56, 0.0802758)
(57, 0.0590886)
(58, 0.047177)
(59, 0.0391927)
(60, 0.0249646)
(61, 0.0162851)
(62, 0.0122572)
(63, 0.00920036)
(64, 0.00570305)
(65, 0.00348975)
(66, 0.00209996)
(67, 0.00114438)
(68, 0.000830539)
(69, 0.000711579)
(70, 0.000611439)
(71, 0.000382451)
(72, 0.000258637)
(73, 0.000129812)
(74, 8.93638e-05)
(75, 5.28728e-05)
(76, 3.86444e-05)
(77, 2.49692e-05)
(78, 1.51632e-05)
(79, 9.30836e-06)
(80, 4.62493e-06)
(81, 3.14587e-06)
(82, 1.71748e-06)
(83, 1.25372e-06)
(84, 6.6265e-07)
(85, 3.86144e-07)
(86, 2.06437e-07)
(87, 1.25254e-07)
(88, 7.20137e-08)
(89, 3.61535e-08)
(90, 2.13287e-08)
(91, 1.42904e-08)
(92, 1.15626e-08)
(93, 6.9716e-09)
(94, 3.63502e-09)
(95, 1.39163e-09)
(96, 5.90018e-10)
(97, 2.56782e-10)
(98, 1.45752e-10)
(99, 9.0568e-11)
(100, 6.25655e-11)
(101, 3.33414e-11)
(102, 2.12661e-11)
(103, 1.05176e-11)
(104, 5.65934e-12)
(105, 3.53738e-12)
(106, 2.73437e-12)
(107, 1.87201e-12)
(108, 6.91319e-13)
(109, 5.23285e-13)
(110, 4.22307e-13)
(111, 4.39358e-13)
(112, 4.09062e-13)
(113, 4.25582e-13)
(114, 4.21796e-13)
(115, 4.77266e-13)
(116, 5.26589e-13)
(117, 5.3441e-13)
(118, 4.60675e-13)
(119, 4.42697e-13)
(120, 4.404e-13)
(121, 4.32515e-13)
(122, 4.40376e-13)
(123, 4.45108e-13)
(124, 4.57156e-13)
(125, 4.53735e-13)
(126, 4.39097e-13)
(127, 4.46868e-13)
(128, 4.49786e-13)
(129, 4.49731e-13)
(130, 4.49719e-13)
(131, 4.49718e-13)
(132, 4.49719e-13)
(133, 4.49721e-13)
(134, 4.49719e-13)
(135, 4.49717e-13)
(136, 4.49716e-13)
(137, 4.49716e-13)
}; \label{plot:fp64} 
\addplot[ color=mygreen, line width=1.0pt, dotted] coordinates { 
(0, 1)
(1, 0.0863842)
(2, 0.0983178)
(3, 0.0449742)
(4, 0.0336921)
(5, 0.0259981)
(6, 0.0135711)
(7, 0.0106814)
(8, 0.004363)
(9, 0.00439304)
(10, 0.00251243)
(11, 0.00176258)
(12, 0.000971175)
(13, 0.00112837)
(14, 0.00144336)
(15, 0.00242062)
(16, 0.00380643)
(17, 0.00684088)
(18, 0.0100224)
(19, 0.0158163)
(20, 0.0201836)
(21, 0.0263944)
(22, 0.0302536)
(23, 0.0254992)
(24, 0.0214696)
(25, 0.0160414)
(26, 0.0148449)
(27, 0.0206921)
(28, 0.0342201)
(29, 0.0368306)
(30, 0.0272254)
(31, 0.0200601)
(32, 0.0222054)
(33, 0.0190523)
(34, 0.0272214)
(35, 0.0259583)
(36, 0.0278462)
(37, 0.0285769)
(38, 0.0298471)
(39, 0.0308077)
(40, 0.0331101)
(41, 0.0429583)
(42, 0.0458453)
(43, 0.0505955)
(44, 0.0494328)
(45, 0.0577913)
(46, 0.0721381)
(47, 0.0971237)
(48, 0.135333)
(49, 0.126257)
(50, 0.145353)
(51, 0.187315)
(52, 0.214848)
(53, 0.203357)
(54, 0.156524)
(55, 0.110798)
(56, 0.089)
(57, 0.0775954)
(58, 0.0596542)
(59, 0.0473743)
(60, 0.0386595)
(61, 0.0250278)
(62, 0.0177406)
(63, 0.0142925)
(64, 0.0112486)
(65, 0.00811931)
(66, 0.00574584)
(67, 0.00484504)
(68, 0.00470984)
(69, 0.00521986)
(70, 0.00650079)
(71, 0.00630612)
(72, 0.00471246)
(73, 0.00358549)
(74, 0.00315548)
(75, 0.00287142)
(76, 0.00276004)
(77, 0.00208592)
(78, 0.0018843)
(79, 0.00165414)
(80, 0.00171461)
(81, 0.00195043)
(82, 0.00214367)
(83, 0.00241672)
(84, 0.0025729)
(85, 0.00276626)
(86, 0.00294306)
(87, 0.00255383)
(88, 0.00246761)
(89, 0.00202173)
(90, 0.00194334)
(91, 0.00202011)
(92, 0.00193366)
(93, 0.00189)
(94, 0.00160035)
(95, 0.00137785)
(96, 0.00100388)
(97, 0.000725585)
(98, 0.000566387)
(99, 0.000497851)
(100, 0.000410584)
(101, 0.000322343)
(102, 0.000268873)
(103, 0.000246738)
(104, 0.000193087)
(105, 0.000139315)
(106, 9.71584e-05)
(107, 9.22054e-05)
(108, 0.000126637)
(109, 0.00018436)
(110, 0.000209091)
(111, 0.000270271)
(112, 0.000365642)
(113, 0.000467719)
(114, 0.000506946)
(115, 0.000514431)
(116, 0.000586458)
(117, 0.000548085)
(118, 0.000503034)
(119, 0.000492219)
(120, 0.000593627)
(121, 0.000778939)
(122, 0.00111537)
(123, 0.00161967)
(124, 0.00181296)
(125, 0.0018657)
(126, 0.00245003)
(127, 0.00366543)
(128, 0.00384907)
(129, 0.0037764)
(130, 0.00395972)
(131, 0.00403763)
(132, 0.00386055)
(133, 0.00294176)
(134, 0.00276697)
(135, 0.00246929)
(136, 0.00234921)
(137, 0.00228865)
(138, 0.0022569)
(139, 0.00282013)
(140, 0.00278576)
(141, 0.00304247)
(142, 0.00354162)
(143, 0.00331069)
(144, 0.00321244)
(145, 0.0039996)
(146, 0.0058207)
(147, 0.00748623)
(148, 0.00782387)
(149, 0.00817518)
(150, 0.00905863)
(151, 0.0102683)
(152, 0.0122433)
(153, 0.0138148)
(154, 0.0125885)
(155, 0.0112795)
(156, 0.0108358)
(157, 0.00948797)
(158, 0.0075231)
(159, 0.00540897)
(160, 0.00364119)
(161, 0.00301614)
(162, 0.00269391)
(163, 0.00247261)
(164, 0.00265848)
(165, 0.00253712)
(166, 0.00244186)
(167, 0.00238952)
(168, 0.00243463)
(169, 0.00201493)
(170, 0.00152442)
(171, 0.00126446)
(172, 0.000787534)
(173, 0.000511989)
(174, 0.000346395)
(175, 0.000263757)
(176, 0.000272837)
(177, 0.000265839)
(178, 0.000279315)
(179, 0.000253643)
(180, 0.000233129)
(181, 0.000235789)
(182, 0.000229001)
(183, 0.000266148)
(184, 0.000355635)
(185, 0.000404884)
(186, 0.000383791)
(187, 0.000366604)
(188, 0.000331839)
(189, 0.000281712)
(190, 0.000262314)
(191, 0.000265309)
(192, 0.00025454)
(193, 0.000226629)
(194, 0.000216566)
(195, 0.000189314)
(196, 0.000154261)
(197, 0.000118645)
(198, 0.000102163)
(199, 9.42869e-05)
(200, 8.25776e-05)
(201, 5.83679e-05)
(202, 5.10209e-05)
(203, 4.64029e-05)
(204, 4.09373e-05)
(205, 3.6373e-05)
(206, 3.36389e-05)
(207, 3.37443e-05)
(208, 4.06361e-05)
(209, 3.87046e-05)
(210, 3.0783e-05)
(211, 2.25511e-05)
(212, 1.98733e-05)
(213, 1.92588e-05)
(214, 1.62932e-05)
(215, 1.41196e-05)
(216, 1.2897e-05)
(217, 1.29985e-05)
(218, 1.73091e-05)
(219, 2.22135e-05)
(220, 3.38345e-05)
(221, 4.61262e-05)
(222, 5.46357e-05)
(223, 6.23552e-05)
(224, 7.99394e-05)
(225, 0.000104137)
(226, 0.000128287)
(227, 0.000150836)
(228, 0.000166421)
(229, 0.000164585)
(230, 0.000165426)
(231, 0.000132143)
(232, 0.000122442)
(233, 0.000129132)
(234, 0.000111217)
(235, 0.000103933)
(236, 0.000124144)
(237, 0.000143601)
(238, 0.00014485)
(239, 0.000122367)
(240, 0.000113489)
(241, 0.00013506)
(242, 0.000153674)
(243, 0.000176442)
(244, 0.0001699)
(245, 0.000172576)
(246, 0.000189816)
(247, 0.000199537)
(248, 0.000221545)
(249, 0.000228375)
(250, 0.000254037)
(251, 0.000333782)
(252, 0.000403427)
(253, 0.000489381)
(254, 0.00052281)
(255, 0.000466062)
(256, 0.000416283)
(257, 0.000489532)
(258, 0.000613779)
(259, 0.000880184)
(260, 0.00113458)
(261, 0.00128119)
(262, 0.00143084)
(263, 0.00166536)
(264, 0.00172777)
(265, 0.00139501)
(266, 0.000919986)
(267, 0.000688043)
(268, 0.000519287)
(269, 0.000379379)
(270, 0.000310958)
(271, 0.000283655)
(272, 0.000227619)
(273, 0.000190243)
(274, 0.000162972)
(275, 0.000138209)
(276, 0.000112957)
(277, 0.000117894)
(278, 0.000118148)
(279, 0.000111601)
(280, 0.000104954)
(281, 9.30422e-05)
(282, 8.23987e-05)
(283, 8.08872e-05)
(284, 6.50962e-05)
(285, 5.63608e-05)
(286, 4.89319e-05)
(287, 4.14056e-05)
(288, 3.53114e-05)
(289, 2.89445e-05)
(290, 3.33479e-05)
(291, 3.87418e-05)
(292, 3.69621e-05)
(293, 3.72364e-05)
(294, 3.60332e-05)
(295, 3.66084e-05)
(296, 4.016e-05)
(297, 3.84028e-05)
(298, 3.85897e-05)
(299, 4.23919e-05)
(300, 4.32496e-05)
(301, 4.07009e-05)
(302, 3.76773e-05)
(303, 3.55073e-05)
(304, 3.49802e-05)
(305, 3.55001e-05)
(306, 2.86511e-05)
(307, 2.48812e-05)
(308, 2.17384e-05)
(309, 1.82686e-05)
(310, 1.33985e-05)
(311, 9.51395e-06)
(312, 5.60445e-06)
(313, 3.82543e-06)
(314, 2.94126e-06)
(315, 3.0638e-06)
(316, 2.89812e-06)
(317, 2.9001e-06)
(318, 2.7948e-06)
(319, 2.84159e-06)
(320, 3.27011e-06)
(321, 3.75323e-06)
(322, 3.74702e-06)
(323, 3.73601e-06)
(324, 3.41622e-06)
(325, 2.79052e-06)
(326, 2.53073e-06)
(327, 2.90004e-06)
(328, 3.75776e-06)
(329, 4.06635e-06)
(330, 4.44961e-06)
(331, 5.48581e-06)
(332, 6.0375e-06)
(333, 7.76043e-06)
(334, 1.05074e-05)
(335, 1.38234e-05)
(336, 1.71601e-05)
(337, 1.90281e-05)
(338, 2.31651e-05)
}; \label{plot:fp16} 
\addplot[color=mydeepblue, line width=1.0pt, dashed] coordinates { 
(0, 1)
(1, 0.0863842)
(2, 0.0983036)
(3, 0.0449711)
(4, 0.033689)
(5, 0.0259928)
(6, 0.013564)
(7, 0.0106732)
(8, 0.00436318)
(9, 0.00439181)
(10, 0.0025118)
(11, 0.00176127)
(12, 0.00097145)
(13, 0.00112778)
(14, 0.00144348)
(15, 0.00241814)
(16, 0.00380538)
(17, 0.00683736)
(18, 0.0100275)
(19, 0.0158171)
(20, 0.0201795)
(21, 0.0263859)
(22, 0.0301931)
(23, 0.0254603)
(24, 0.0214222)
(25, 0.0160478)
(26, 0.0148486)
(27, 0.0206199)
(28, 0.03409)
(29, 0.0366507)
(30, 0.0270341)
(31, 0.0198461)
(32, 0.0220075)
(33, 0.0190393)
(34, 0.0277447)
(35, 0.0259836)
(36, 0.0278785)
(37, 0.0283952)
(38, 0.0299492)
(39, 0.0310101)
(40, 0.0334878)
(41, 0.0434039)
(42, 0.0464134)
(43, 0.0507541)
(44, 0.0491429)
(45, 0.0579679)
(46, 0.0724889)
(47, 0.102809)
(48, 0.135016)
(49, 0.135459)
(50, 0.14576)
(51, 0.196335)
(52, 0.202924)
(53, 0.194249)
(54, 0.13598)
(55, 0.0950816)
(56, 0.0802758)
(57, 0.0590886)
(58, 0.047177)
(59, 0.0391927)
(60, 0.0249646)
(61, 0.0162851)
(62, 0.0122572)
(63, 0.00920036)
(64, 0.00570305)
(65, 0.00348975)
(66, 0.00209996)
(67, 0.00114438)
(68, 0.000830539)
(69, 0.000711579)
(70, 0.000611439)
(71, 0.000382451)
(72, 0.000258637)
(73, 0.000129812)
(74, 8.93638e-05)
(75, 5.28728e-05)
(76, 3.86444e-05)
(77, 2.49692e-05)
(78, 1.51632e-05)
(79, 9.30836e-06)
(80, 4.62493e-06)
(81, 3.14587e-06)
(82, 1.71748e-06)
(83, 1.25372e-06)
(84, 6.6265e-07)
(85, 3.86144e-07)
(86, 2.06437e-07)
(87, 1.25254e-07)
(88, 7.20137e-08)
(89, 3.61535e-08)
(90, 2.13287e-08)
(91, 1.42904e-08)
(92, 1.15626e-08)
(93, 6.9716e-09)
(94, 3.63502e-09)
(95, 1.39162e-09)
(96, 5.90025e-10)
(97, 2.56782e-10)
(98, 1.45763e-10)
(99, 9.05811e-11)
(100, 6.25848e-11)
(101, 3.33731e-11)
(102, 2.13099e-11)
(103, 1.05902e-11)
(104, 5.71158e-12)
(105, 3.75207e-12)
(106, 2.94961e-12)
(107, 1.9156e-12)
(108, 6.74586e-13)
(109, 4.12544e-13)
(110, 3.78004e-13)
(111, 3.33908e-13)
(112, 3.18705e-13)
(113, 3.11302e-13)
(114, 3.15631e-13)
(115, 3.17154e-13)
(116, 3.01511e-13)
(117, 3.26326e-13)
(118, 3.1729e-13)
(119, 3.24546e-13)
(120, 3.24357e-13)
(121, 3.2548e-13)
(122, 3.25092e-13)
(123, 3.22487e-13)
(124, 3.36009e-13)
(125, 3.26926e-13)
(126, 3.38615e-13)
(127, 3.37163e-13)
(128, 3.31111e-13)
(129, 3.3179e-13)
(130, 3.36037e-13)
(131, 3.35908e-13)
(132, 3.40466e-13)
(133, 3.39674e-13)
(134, 3.38118e-13)
(135, 3.44112e-13)
(136, 3.44212e-13)
(137, 3.48198e-13)
(138, 3.47703e-13)
(139, 3.47698e-13)
(140, 3.47696e-13)
(141, 3.47696e-13)
(142, 3.47696e-13)
(143, 3.47695e-13)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=x, color=red,   mark size=3pt, line width=1.0pt] coordinates { 
 (74, 0.000129812) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=x, color=black,   mark size=3pt, line width=1.5pt] coordinates { 
 (84, 1.25372e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks,  mark=o, color=blue,   mark size=3pt,line width=1.0pt] coordinates { 
 (93, 1.15626e-08) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/okCond_3_2.tex <==
\addplot[color=myyellow, line width=1.0pt] coordinates { 
(0, 1)
(1, 1.33556)
(2, 2.34271)
(3, 2.00356)
(4, 1.88812)
(5, 1.52919)
(6, 1.80888)
(7, 1.74588)
(8, 2.03366)
(9, 1.98919)
(10, 1.99434)
(11, 2.08282)
(12, 2.08405)
(13, 2.16367)
(14, 2.26627)
(15, 2.53868)
(16, 2.70097)
(17, 3.23814)
(18, 3.69585)
(19, 3.68005)
(20, 3.71119)
(21, 4.05793)
(22, 4.772)
(23, 5.16491)
(24, 6.08244)
(25, 7.00913)
(26, 7.19744)
(27, 6.95715)
(28, 7.01886)
(29, 6.87139)
(30, 6.63115)
(31, 6.24729)
(32, 6.7499)
(33, 6.81362)
(34, 6.8042)
(35, 6.34767)
(36, 6.35304)
(37, 7.03258)
(38, 7.30091)
(39, 7.28864)
(40, 7.65178)
(41, 6.93239)
(42, 7.34389)
(43, 6.56486)
(44, 6.58119)
(45, 6.01171)
(46, 5.85005)
(47, 5.86606)
(48, 5.56246)
(49, 4.91215)
(50, 5.29456)
(51, 5.51394)
(52, 5.80018)
(53, 5.17596)
(54, 4.76071)
(55, 4.59519)
(56, 4.53007)
(57, 4.81523)
(58, 4.36954)
(59, 3.9574)
(60, 3.94644)
(61, 3.94101)
(62, 3.8707)
(63, 3.7478)
(64, 3.54673)
(65, 3.21534)
(66, 3.41732)
(67, 3.48488)
(68, 2.96929)
(69, 2.87137)
(70, 2.89663)
(71, 2.86473)
(72, 2.90224)
(73, 2.95552)
(74, 3.11219)
(75, 2.91314)
(76, 2.52656)
(77, 2.40835)
(78, 2.30936)
(79, 2.24853)
(80, 2.3737)
(81, 2.48118)
(82, 2.40924)
(83, 2.46638)
(84, 2.52448)
(85, 2.35455)
(86, 2.47586)
(87, 2.21742)
(88, 2.17286)
(89, 2.3174)
(90, 2.40726)
(91, 2.42197)
(92, 2.32482)
(93, 2.23515)
(94, 2.08309)
(95, 1.95269)
(96, 1.83474)
(97, 1.77061)
(98, 1.82235)
(99, 1.84877)
(100, 1.82369)
(101, 1.66133)
(102, 1.60346)
(103, 1.46135)
(104, 1.30608)
(105, 1.16408)
(106, 1.13154)
(107, 1.01079)
(108, 1.00375)
(109, 0.997137)
(110, 0.91872)
(111, 0.848205)
(112, 0.837909)
(113, 0.746271)
(114, 0.658014)
(115, 0.609168)
(116, 0.58198)
(117, 0.517678)
(118, 0.479006)
(119, 0.391947)
(120, 0.313403)
(121, 0.303015)
(122, 0.250355)
(123, 0.21115)
(124, 0.182425)
(125, 0.158178)
(126, 0.1542)
(127, 0.132414)
(128, 0.104561)
(129, 0.0916794)
(130, 0.0793385)
(131, 0.0672901)
(132, 0.0602747)
(133, 0.0504348)
(134, 0.0424119)
(135, 0.0380302)
(136, 0.0347312)
(137, 0.0312654)
(138, 0.0265289)
(139, 0.02499)
(140, 0.0216186)
(141, 0.0180809)
(142, 0.0141602)
(143, 0.0127788)
(144, 0.0101788)
(145, 0.00896668)
(146, 0.00874611)
(147, 0.00836246)
(148, 0.00748573)
(149, 0.00634869)
(150, 0.00549501)
(151, 0.00526751)
(152, 0.00498922)
(153, 0.00415059)
(154, 0.00335096)
(155, 0.00295825)
(156, 0.00246074)
(157, 0.00227625)
(158, 0.00209191)
(159, 0.00195571)
(160, 0.00173612)
(161, 0.00162263)
(162, 0.00150957)
(163, 0.00130222)
(164, 0.00119023)
(165, 0.0010539)
(166, 0.00101806)
(167, 0.000855919)
(168, 0.000643459)
(169, 0.000560059)
(170, 0.000496871)
(171, 0.00042989)
(172, 0.000396182)
(173, 0.000372)
(174, 0.000333789)
(175, 0.000279515)
(176, 0.000224673)
(177, 0.00019988)
(178, 0.00017459)
(179, 0.000152264)
(180, 0.000132406)
(181, 0.000102008)
(182, 9.01878e-05)
(183, 7.20084e-05)
(184, 5.7468e-05)
(185, 4.93948e-05)
(186, 4.02305e-05)
(187, 3.344e-05)
(188, 2.81604e-05)
(189, 2.27249e-05)
(190, 1.82924e-05)
(191, 1.50869e-05)
(192, 1.11803e-05)
(193, 8.98e-06)
(194, 7.54722e-06)
(195, 5.70391e-06)
(196, 4.30989e-06)
(197, 3.64073e-06)
(198, 3.24024e-06)
(199, 2.33478e-06)
(200, 1.80205e-06)
(201, 1.48176e-06)
(202, 1.23493e-06)
(203, 1.14556e-06)
(204, 9.60005e-07)
(205, 7.2657e-07)
(206, 6.29281e-07)
(207, 4.98708e-07)
(208, 4.28332e-07)
(209, 3.89714e-07)
(210, 2.91423e-07)
(211, 2.34614e-07)
(212, 1.99646e-07)
(213, 1.68413e-07)
(214, 1.45034e-07)
(215, 1.22317e-07)
(216, 9.22428e-08)
(217, 7.3106e-08)
(218, 6.32718e-08)
(219, 5.38594e-08)
(220, 4.77322e-08)
(221, 3.84845e-08)
(222, 3.30651e-08)
(223, 2.48294e-08)
(224, 2.26119e-08)
(225, 2.12429e-08)
(226, 1.49028e-08)
(227, 1.4117e-08)
(228, 1.1612e-08)
(229, 8.80144e-09)
(230, 7.79978e-09)
(231, 6.88441e-09)
(232, 5.64541e-09)
(233, 4.70125e-09)
(234, 3.6452e-09)
(235, 2.75672e-09)
(236, 2.17427e-09)
(237, 1.7613e-09)
(238, 1.41438e-09)
(239, 1.12712e-09)
(240, 8.64065e-10)
(241, 7.04884e-10)
(242, 5.67708e-10)
(243, 5.2687e-10)
(244, 4.2067e-10)
(245, 3.42663e-10)
(246, 2.65308e-10)
(247, 2.23762e-10)
(248, 1.9418e-10)
(249, 1.52694e-10)
(250, 1.34224e-10)
(251, 1.11174e-10)
(252, 9.05135e-11)
}; \label{plot:fp64} 
\addplot[ color=mygreen, line width=1.0pt, dotted] coordinates { 
(0, 1)
(1, 1.33556)
(2, 2.34272)
(3, 2.00382)
(4, 1.88827)
(5, 1.52901)
(6, 1.80911)
(7, 1.74578)
(8, 2.0339)
(9, 1.98969)
(10, 1.99463)
(11, 2.08339)
(12, 2.0847)
(13, 2.16529)
(14, 2.26736)
(15, 2.53937)
(16, 2.70113)
(17, 3.23899)
(18, 3.69746)
(19, 3.68063)
(20, 3.71223)
(21, 4.05735)
(22, 4.77433)
(23, 5.16619)
(24, 6.08367)
(25, 7.01004)
(26, 7.19238)
(27, 6.95416)
(28, 7.02404)
(29, 6.87115)
(30, 6.63819)
(31, 6.25327)
(32, 6.75099)
(33, 6.81657)
(34, 6.80322)
(35, 6.35648)
(36, 6.35539)
(37, 7.03742)
(38, 7.32339)
(39, 7.2946)
(40, 7.66217)
(41, 6.94912)
(42, 7.35795)
(43, 6.58327)
(44, 6.60207)
(45, 6.03143)
(46, 5.86525)
(47, 5.87478)
(48, 5.5741)
(49, 4.91706)
(50, 5.28632)
(51, 5.51197)
(52, 5.80145)
(53, 5.18553)
(54, 4.75833)
(55, 4.5938)
(56, 4.53367)
(57, 4.83342)
(58, 4.39075)
(59, 3.96188)
(60, 3.95541)
(61, 3.94656)
(62, 3.87611)
(63, 3.76808)
(64, 3.55394)
(65, 3.2237)
(66, 3.40865)
(67, 3.51794)
(68, 3.0177)
(69, 2.86851)
(70, 2.91386)
(71, 2.86701)
(72, 2.90883)
(73, 2.96896)
(74, 3.11302)
(75, 2.95232)
(76, 2.54552)
(77, 2.42157)
(78, 2.33369)
(79, 2.26256)
(80, 2.35062)
(81, 2.49902)
(82, 2.37778)
(83, 2.48674)
(84, 2.53666)
(85, 2.33876)
(86, 2.51806)
(87, 2.23734)
(88, 2.18549)
(89, 2.29352)
(90, 2.3748)
(91, 2.46723)
(92, 2.32206)
(93, 2.26091)
(94, 2.12247)
(95, 1.9835)
(96, 1.84516)
(97, 1.76925)
(98, 1.82432)
(99, 1.7947)
(100, 1.88318)
(101, 1.70214)
(102, 1.61148)
(103, 1.46241)
(104, 1.39806)
(105, 1.16439)
(106, 1.15146)
(107, 1.03147)
(108, 1.02297)
(109, 0.987455)
(110, 0.965271)
(111, 0.847637)
(112, 0.851474)
(113, 0.793657)
(114, 0.673932)
(115, 0.620131)
(116, 0.602723)
(117, 0.525924)
(118, 0.502118)
(119, 0.42365)
(120, 0.335733)
(121, 0.301658)
(122, 0.272735)
(123, 0.226024)
(124, 0.190756)
(125, 0.166949)
(126, 0.154064)
(127, 0.141637)
(128, 0.117913)
(129, 0.0947604)
(130, 0.0842806)
(131, 0.0745572)
(132, 0.062441)
(133, 0.0556436)
(134, 0.0452092)
(135, 0.0403892)
(136, 0.0351333)
(137, 0.033974)
(138, 0.0285395)
(139, 0.0255458)
(140, 0.0234016)
(141, 0.019641)
(142, 0.0160461)
(143, 0.0134114)
(144, 0.0116725)
(145, 0.0095294)
(146, 0.00918907)
(147, 0.00865079)
(148, 0.00842846)
(149, 0.00712138)
(150, 0.00618165)
(151, 0.00576729)
(152, 0.00563077)
(153, 0.00516358)
(154, 0.00430716)
(155, 0.003708)
(156, 0.00329814)
(157, 0.00310545)
(158, 0.00300875)
(159, 0.00302962)
(160, 0.0030355)
(161, 0.00281003)
(162, 0.00304124)
(163, 0.00284742)
(164, 0.00283716)
(165, 0.00285331)
(166, 0.00288759)
(167, 0.00310397)
(168, 0.00268916)
(169, 0.00257713)
(170, 0.00282086)
(171, 0.00308629)
(172, 0.00327378)
(173, 0.00369819)
(174, 0.0039456)
(175, 0.00401145)
(176, 0.00383128)
(177, 0.00381804)
(178, 0.00417359)
(179, 0.00420339)
(180, 0.00426255)
(181, 0.00415719)
(182, 0.00390603)
(183, 0.00416996)
(184, 0.00380678)
(185, 0.00376522)
(186, 0.00375324)
(187, 0.00348506)
(188, 0.00330288)
(189, 0.00304929)
(190, 0.00269763)
(191, 0.00248569)
(192, 0.00231176)
(193, 0.00207401)
(194, 0.0021301)
(195, 0.00199514)
(196, 0.00184818)
(197, 0.001887)
(198, 0.00203303)
(199, 0.0019857)
(200, 0.00192169)
(201, 0.00234156)
(202, 0.00270126)
(203, 0.00302757)
(204, 0.00332748)
(205, 0.00330981)
(206, 0.00383694)
(207, 0.00441024)
(208, 0.00442513)
(209, 0.00437654)
(210, 0.00393968)
(211, 0.00335598)
(212, 0.00338457)
(213, 0.00307232)
(214, 0.00268173)
(215, 0.00255763)
(216, 0.00242921)
(217, 0.00256236)
(218, 0.00292808)
(219, 0.00310273)
(220, 0.00324715)
(221, 0.00372078)
(222, 0.00434404)
(223, 0.00539207)
(224, 0.00615905)
(225, 0.00755797)
(226, 0.00750489)
(227, 0.00817092)
(228, 0.0103261)
(229, 0.00940621)
(230, 0.0101796)
(231, 0.0103722)
(232, 0.00902133)
(233, 0.00847815)
(234, 0.00811571)
(235, 0.00713251)
(236, 0.00639707)
(237, 0.0053622)
(238, 0.00436241)
(239, 0.00373699)
(240, 0.00327235)
(241, 0.00290909)
(242, 0.00267561)
(243, 0.00231638)
(244, 0.00204357)
(245, 0.00176021)
(246, 0.0018015)
(247, 0.00166367)
(248, 0.00156101)
(249, 0.00147814)
(250, 0.00150619)
(251, 0.00162631)
(252, 0.00160077)
(253, 0.00155016)
(254, 0.00143087)
(255, 0.00128862)
(256, 0.00107862)
(257, 0.000944307)
(258, 0.000886821)
(259, 0.000777124)
(260, 0.000616267)
(261, 0.00053947)
(262, 0.000491289)
(263, 0.000441454)
(264, 0.000349168)
(265, 0.000308256)
(266, 0.000293001)
(267, 0.000244111)
(268, 0.00017821)
(269, 0.000161656)
(270, 0.00015895)
(271, 0.000116114)
(272, 9.96946e-05)
(273, 8.46008e-05)
(274, 5.91438e-05)
(275, 4.40555e-05)
(276, 4.29337e-05)
(277, 3.59582e-05)
(278, 3.13031e-05)
(279, 2.41434e-05)
(280, 2.31155e-05)
(281, 2.06787e-05)
(282, 1.82337e-05)
(283, 1.76525e-05)
(284, 1.65562e-05)
(285, 1.80567e-05)
(286, 1.89721e-05)
(287, 1.97981e-05)
(288, 2.09309e-05)
(289, 2.17861e-05)
(290, 2.32824e-05)
(291, 2.82868e-05)
(292, 3.16666e-05)
(293, 3.1986e-05)
(294, 3.28742e-05)
(295, 3.12241e-05)
(296, 3.19725e-05)
(297, 2.87777e-05)
(298, 2.73429e-05)
(299, 2.97448e-05)
(300, 2.67468e-05)
(301, 2.31765e-05)
(302, 1.93668e-05)
(303, 1.64151e-05)
(304, 1.53456e-05)
(305, 1.36283e-05)
(306, 1.23764e-05)
(307, 1.19784e-05)
(308, 1.05239e-05)
(309, 1.02636e-05)
(310, 1.19959e-05)
(311, 1.264e-05)
(312, 1.29917e-05)
(313, 1.33289e-05)
(314, 1.29601e-05)
(315, 1.20205e-05)
(316, 1.15373e-05)
(317, 1.09591e-05)
(318, 1.05146e-05)
(319, 1.05412e-05)
(320, 9.05686e-06)
(321, 9.22443e-06)
(322, 8.877e-06)
(323, 8.31588e-06)
(324, 7.63785e-06)
(325, 8.74111e-06)
(326, 9.54568e-06)
(327, 9.60604e-06)
(328, 9.25999e-06)
(329, 9.32517e-06)
(330, 8.74645e-06)
(331, 7.72038e-06)
(332, 6.28229e-06)
(333, 4.67947e-06)
(334, 4.5243e-06)
(335, 3.84329e-06)
(336, 3.87142e-06)
(337, 4.2309e-06)
(338, 4.74018e-06)
(339, 5.68063e-06)
(340, 6.27306e-06)
(341, 7.1833e-06)
(342, 7.69103e-06)
(343, 8.06114e-06)
(344, 8.55736e-06)
(345, 9.1238e-06)
(346, 9.89586e-06)
(347, 9.94013e-06)
(348, 1.10887e-05)
(349, 1.23986e-05)
(350, 1.22846e-05)
(351, 1.32212e-05)
(352, 1.32218e-05)
(353, 1.42103e-05)
(354, 1.41646e-05)
(355, 1.74323e-05)
(356, 1.78901e-05)
(357, 1.78288e-05)
(358, 2.0784e-05)
(359, 2.46317e-05)
(360, 3.09144e-05)
(361, 3.11577e-05)
(362, 3.45516e-05)
(363, 3.12639e-05)
(364, 2.95397e-05)
(365, 2.93717e-05)
(366, 2.40849e-05)
(367, 1.86472e-05)
(368, 1.73587e-05)
(369, 1.58111e-05)
(370, 1.44899e-05)
(371, 1.39558e-05)
(372, 1.36404e-05)
(373, 1.36559e-05)
(374, 1.29583e-05)
(375, 1.20262e-05)
(376, 9.11237e-06)
(377, 8.1651e-06)
(378, 9.01439e-06)
(379, 7.58047e-06)
(380, 6.05845e-06)
(381, 5.42126e-06)
(382, 4.83973e-06)
(383, 5.09494e-06)
(384, 4.62065e-06)
(385, 3.61638e-06)
(386, 2.92536e-06)
(387, 2.59035e-06)
(388, 2.28311e-06)
(389, 2.33148e-06)
(390, 2.10505e-06)
(391, 2.00034e-06)
(392, 1.9262e-06)
(393, 1.72539e-06)
(394, 1.53775e-06)
(395, 1.4049e-06)
(396, 1.35161e-06)
(397, 1.17174e-06)
(398, 1.18891e-06)
(399, 1.12587e-06)
(400, 1.02068e-06)
}; \label{plot:fp16} 
\addplot[color=mydeepblue, line width=1.0pt, dashed] coordinates { 
(0, 1)
(1, 1.33556)
(2, 2.34271)
(3, 2.00356)
(4, 1.88812)
(5, 1.52919)
(6, 1.80888)
(7, 1.74588)
(8, 2.03366)
(9, 1.98919)
(10, 1.99434)
(11, 2.08282)
(12, 2.08405)
(13, 2.16367)
(14, 2.26627)
(15, 2.53868)
(16, 2.70097)
(17, 3.23814)
(18, 3.69585)
(19, 3.68005)
(20, 3.71119)
(21, 4.05793)
(22, 4.772)
(23, 5.16491)
(24, 6.08244)
(25, 7.00913)
(26, 7.19744)
(27, 6.95715)
(28, 7.01886)
(29, 6.87139)
(30, 6.63115)
(31, 6.24729)
(32, 6.7499)
(33, 6.81362)
(34, 6.8042)
(35, 6.34767)
(36, 6.35304)
(37, 7.03258)
(38, 7.30091)
(39, 7.28864)
(40, 7.65178)
(41, 6.93239)
(42, 7.34389)
(43, 6.56486)
(44, 6.58119)
(45, 6.01171)
(46, 5.85005)
(47, 5.86606)
(48, 5.56246)
(49, 4.91215)
(50, 5.29456)
(51, 5.51394)
(52, 5.80018)
(53, 5.17596)
(54, 4.76071)
(55, 4.59519)
(56, 4.53007)
(57, 4.81523)
(58, 4.36954)
(59, 3.9574)
(60, 3.94644)
(61, 3.94101)
(62, 3.8707)
(63, 3.7478)
(64, 3.54673)
(65, 3.21534)
(66, 3.41732)
(67, 3.48488)
(68, 2.96929)
(69, 2.87137)
(70, 2.89663)
(71, 2.86473)
(72, 2.90224)
(73, 2.95552)
(74, 3.11219)
(75, 2.91314)
(76, 2.52656)
(77, 2.40835)
(78, 2.30936)
(79, 2.24853)
(80, 2.3737)
(81, 2.48118)
(82, 2.40924)
(83, 2.46638)
(84, 2.52448)
(85, 2.35455)
(86, 2.47586)
(87, 2.21742)
(88, 2.17286)
(89, 2.3174)
(90, 2.40726)
(91, 2.42197)
(92, 2.32482)
(93, 2.23515)
(94, 2.08309)
(95, 1.95269)
(96, 1.83474)
(97, 1.77061)
(98, 1.82235)
(99, 1.84877)
(100, 1.82369)
(101, 1.66133)
(102, 1.60346)
(103, 1.46135)
(104, 1.30608)
(105, 1.16408)
(106, 1.13154)
(107, 1.01079)
(108, 1.00375)
(109, 0.997137)
(110, 0.91872)
(111, 0.848205)
(112, 0.837909)
(113, 0.746271)
(114, 0.658014)
(115, 0.609168)
(116, 0.58198)
(117, 0.517678)
(118, 0.479006)
(119, 0.391947)
(120, 0.313403)
(121, 0.303015)
(122, 0.250355)
(123, 0.21115)
(124, 0.182425)
(125, 0.158178)
(126, 0.1542)
(127, 0.132414)
(128, 0.104561)
(129, 0.0916794)
(130, 0.0793385)
(131, 0.0672901)
(132, 0.0602747)
(133, 0.0504348)
(134, 0.0424119)
(135, 0.0380302)
(136, 0.0347312)
(137, 0.0312654)
(138, 0.0265289)
(139, 0.02499)
(140, 0.0216186)
(141, 0.0180809)
(142, 0.0141602)
(143, 0.0127788)
(144, 0.0101788)
(145, 0.00896668)
(146, 0.00874611)
(147, 0.00836246)
(148, 0.00748573)
(149, 0.00634869)
(150, 0.00549501)
(151, 0.00526751)
(152, 0.00498922)
(153, 0.00415059)
(154, 0.00335096)
(155, 0.00295825)
(156, 0.00246074)
(157, 0.00227625)
(158, 0.00209191)
(159, 0.00195571)
(160, 0.00173612)
(161, 0.00162263)
(162, 0.00150957)
(163, 0.00130222)
(164, 0.00119023)
(165, 0.0010539)
(166, 0.00101806)
(167, 0.000855919)
(168, 0.000643459)
(169, 0.000560059)
(170, 0.000496871)
(171, 0.00042989)
(172, 0.000396182)
(173, 0.000372)
(174, 0.000333789)
(175, 0.000279515)
(176, 0.000224673)
(177, 0.00019988)
(178, 0.00017459)
(179, 0.000152264)
(180, 0.000132406)
(181, 0.000102008)
(182, 9.01878e-05)
(183, 7.20084e-05)
(184, 5.74679e-05)
(185, 4.93947e-05)
(186, 4.02305e-05)
(187, 3.34399e-05)
(188, 2.81603e-05)
(189, 2.27248e-05)
(190, 1.82922e-05)
(191, 1.50867e-05)
(192, 1.11799e-05)
(193, 8.9798e-06)
(194, 7.5467e-06)
(195, 5.7034e-06)
(196, 4.30931e-06)
(197, 3.6402e-06)
(198, 3.23932e-06)
(199, 2.33288e-06)
(200, 1.8003e-06)
(201, 1.47989e-06)
(202, 1.23329e-06)
(203, 1.14454e-06)
(204, 9.56868e-07)
(205, 7.25525e-07)
(206, 6.26295e-07)
(207, 4.98043e-07)
(208, 4.27749e-07)
(209, 3.89323e-07)
(210, 2.91148e-07)
(211, 2.34261e-07)
(212, 1.99604e-07)
(213, 1.68389e-07)
(214, 1.45073e-07)
(215, 1.22316e-07)
(216, 9.22521e-08)
(217, 7.31178e-08)
(218, 6.3277e-08)
(219, 5.38712e-08)
(220, 4.77385e-08)
(221, 3.84865e-08)
(222, 3.30642e-08)
(223, 2.48311e-08)
(224, 2.26121e-08)
(225, 2.1248e-08)
(226, 1.49082e-08)
(227, 1.41201e-08)
(228, 1.1618e-08)
(229, 8.80745e-09)
(230, 7.80521e-09)
(231, 6.89138e-09)
(232, 5.65583e-09)
(233, 4.7129e-09)
(234, 3.65628e-09)
(235, 2.77073e-09)
(236, 2.19666e-09)
(237, 1.78546e-09)
(238, 1.43255e-09)
(239, 1.15087e-09)
(240, 8.85795e-10)
(241, 7.23536e-10)
(242, 5.76784e-10)
(243, 5.33283e-10)
(244, 4.28879e-10)
(245, 3.44455e-10)
(246, 2.74245e-10)
(247, 2.24521e-10)
(248, 1.95733e-10)
(249, 1.54553e-10)
(250, 1.36015e-10)
(251, 1.11887e-10)
(252, 9.45164e-11)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=x, color=red, mark size=3pt, line width=1.5pt] coordinates { 
 (182, 0.000102008) 
}; \label{plot:fp32tofp16} 
 \addplot[only marks, mark=x, color=black, mark size=3pt, line width=1.5pt] coordinates { 
 (204, 1.14454e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=o, mark size=3pt, color=blue, line width=1.0pt] coordinates { 
 (199, 3.23932e-06) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/okCond_3_res.tex <==
\addplot[color=myyellow, line width=1.0pt] coordinates { 
(0, 1)
(1, 0.657097)
(2, 0.626965)
(3, 0.612147)
(4, 0.887326)
(5, 0.744882)
(6, 0.751643)
(7, 0.651591)
(8, 0.705007)
(9, 0.607611)
(10, 0.682987)
(11, 0.451794)
(12, 0.577344)
(13, 0.673018)
(14, 0.687341)
(15, 0.796501)
(16, 0.52864)
(17, 0.71715)
(18, 0.813362)
(19, 0.751568)
(20, 0.646775)
(21, 0.497938)
(22, 0.348251)
(23, 0.436799)
(24, 0.412782)
(25, 0.301714)
(26, 0.264768)
(27, 0.279855)
(28, 0.30366)
(29, 0.364867)
(30, 0.351715)
(31, 0.492873)
(32, 0.52018)
(33, 0.44369)
(34, 0.29178)
(35, 0.322314)
(36, 0.293845)
(37, 0.346179)
(38, 0.325833)
(39, 0.245966)
(40, 0.206203)
(41, 0.27924)
(42, 0.149116)
(43, 0.166875)
(44, 0.191896)
(45, 0.165155)
(46, 0.163154)
(47, 0.15222)
(48, 0.277802)
(49, 0.316657)
(50, 0.283461)
(51, 0.24363)
(52, 0.234253)
(53, 0.375595)
(54, 0.37043)
(55, 0.243425)
(56, 0.239563)
(57, 0.352944)
(58, 0.247774)
(59, 0.168471)
(60, 0.123437)
(61, 0.146105)
(62, 0.218556)
(63, 0.242172)
(64, 0.191306)
(65, 0.185013)
(66, 0.186682)
(67, 0.199486)
(68, 0.0916318)
(69, 0.143667)
(70, 0.15015)
(71, 0.0733129)
(72, 0.0587494)
(73, 0.0723524)
(74, 0.0803343)
(75, 0.0508311)
(76, 0.0385857)
(77, 0.0375881)
(78, 0.0805716)
(79, 0.0625984)
(80, 0.0280928)
(81, 0.0442261)
(82, 0.101735)
(83, 0.141375)
(84, 0.183947)
(85, 0.109199)
(86, 0.125388)
(87, 0.287517)
(88, 0.121051)
(89, 0.155141)
(90, 0.13267)
(91, 0.0791222)
(92, 0.185556)
(93, 0.0738948)
(94, 0.115187)
(95, 0.0644363)
(96, 0.0517909)
(97, 0.0254997)
(98, 0.0296805)
(99, 0.0624145)
(100, 0.0490592)
(101, 0.0567303)
(102, 0.0578281)
(103, 0.12262)
(104, 0.0835629)
(105, 0.0298219)
(106, 0.0245132)
(107, 0.0512089)
(108, 0.0232443)
(109, 0.0186591)
(110, 0.0181014)
(111, 0.00681872)
(112, 0.000518876)
(113, 0.00512431)
(114, 0.00263268)
(115, 0.000460935)
(116, 0.000321684)
(117, 0.000726678)
(118, 0.00138042)
(119, 0.000406283)
(120, 0.00016828)
(121, 0.000581363)
(122, 0.000669597)
(123, 0.000328319)
(124, 7.00672e-05)
(125, 3.9676e-05)
(126, 3.30864e-05)
(127, 0.000103518)
(128, 9.56321e-05)
(129, 2.18721e-05)
(130, 6.83033e-06)
(131, 1.77798e-06)
(132, 7.31555e-07)
(133, 1.16603e-07)
(134, 1.48807e-07)
(135, 7.32755e-08)
(136, 2.34471e-07)
(137, 1.74986e-07)
(138, 2.83145e-07)
(139, 5.06056e-07)
(140, 7.6323e-07)
(141, 1.14375e-06)
(142, 5.74382e-07)
(143, 2.02297e-07)
(144, 1.28236e-07)
(145, 6.83471e-08)
(146, 6.40223e-08)
(147, 2.27104e-08)
(148, 1.88314e-08)
(149, 2.21392e-08)
(150, 4.11452e-08)
(151, 6.29169e-08)
(152, 7.40709e-08)
(153, 5.68269e-08)
(154, 3.67616e-08)
(155, 3.44727e-08)
(156, 1.77146e-08)
(157, 8.85564e-09)
(158, 7.86055e-09)
(159, 6.78322e-09)
(160, 4.23093e-09)
(161, 3.5973e-09)
(162, 8.76387e-09)
(163, 6.62564e-09)
(164, 1.29547e-08)
(165, 9.80454e-09)
(166, 2.51149e-08)
(167, 3.15071e-08)
(168, 3.40151e-08)
(169, 3.06253e-08)
(170, 3.57897e-08)
(171, 4.96371e-08)
(172, 1.23641e-08)
(173, 2.46365e-09)
(174, 2.18559e-09)
(175, 1.39896e-09)
(176, 1.73858e-09)
(177, 1.29759e-09)
(178, 1.26945e-09)
(179, 7.48842e-10)
(180, 4.03261e-10)
(181, 4.89399e-10)
(182, 3.34187e-10)
(183, 1.2464e-10)
(184, 1.09102e-10)
(185, 7.89013e-11)
(186, 7.82174e-11)
(187, 3.82954e-11)
(188, 2.21234e-11)
(189, 3.25673e-11)
(190, 2.23146e-11)
(191, 7.59698e-12)
(192, 1.01093e-11)
(193, 1.16412e-11)
(194, 1.18935e-11)
(195, 3.43372e-12)
(196, 3.12136e-12)
(197, 1.86279e-12)
(198, 1.724e-12)
(199, 3.43041e-12)
(200, 1.30004e-12)
(201, 1.27675e-12)
(202, 3.86084e-13)
(203, 2.51138e-13)
(204, 1.69635e-13)
(205, 2.00594e-13)
(206, 7.80635e-14)
(207, 1.6472e-13)
(208, 1.36049e-13)
(209, 6.99973e-15)
(210, 9.016e-15)
(211, 8.53439e-15)
(212, 7.27096e-15)
(213, 2.86167e-15)
(214, 3.40914e-15)
(215, 4.63055e-15)
(216, 3.61933e-15)
(217, 2.59493e-15)
(218, 1.60723e-15)
(219, 8.3623e-16)
}; \label{plot:fp64} 
\addplot[ color=mygreen, line width=1.0pt, dotted] coordinates { 
(0, 1)
(1, 0.657097)
(2, 0.626969)
(3, 0.61218)
(4, 0.887379)
(5, 0.745014)
(6, 0.751659)
(7, 0.651488)
(8, 0.702497)
(9, 0.608023)
(10, 0.683546)
(11, 0.451404)
(12, 0.576561)
(13, 0.675273)
(14, 0.686542)
(15, 0.797353)
(16, 0.528316)
(17, 0.717824)
(18, 0.814784)
(19, 0.749718)
(20, 0.645813)
(21, 0.501879)
(22, 0.360253)
(23, 0.475967)
(24, 0.441865)
(25, 0.358917)
(26, 0.272075)
(27, 0.26025)
(28, 0.345323)
(29, 0.349715)
(30, 0.413883)
(31, 0.338758)
(32, 0.525408)
(33, 0.490206)
(34, 0.459016)
(35, 0.306141)
(36, 0.33388)
(37, 0.377177)
(38, 0.327658)
(39, 0.344489)
(40, 0.287659)
(41, 0.246799)
(42, 0.223234)
(43, 0.262885)
(44, 0.151199)
(45, 0.16697)
(46, 0.227659)
(47, 0.186428)
(48, 0.149042)
(49, 0.153463)
(50, 0.235352)
(51, 0.395348)
(52, 0.354909)
(53, 0.318032)
(54, 0.293851)
(55, 0.285128)
(56, 0.27573)
(57, 0.398938)
(58, 0.364097)
(59, 0.265041)
(60, 0.23663)
(61, 0.407671)
(62, 0.346657)
(63, 0.191204)
(64, 0.131047)
(65, 0.151038)
(66, 0.18035)
(67, 0.204915)
(68, 0.254313)
(69, 0.276857)
(70, 0.230446)
(71, 0.156691)
(72, 0.241321)
(73, 0.197491)
(74, 0.161452)
(75, 0.112267)
(76, 0.110158)
(77, 0.163728)
(78, 0.128158)
(79, 0.0582655)
(80, 0.0719907)
(81, 0.0798942)
(82, 0.0733285)
(83, 0.0660826)
(84, 0.0491526)
(85, 0.0415009)
(86, 0.0437196)
(87, 0.0727482)
(88, 0.0694106)
(89, 0.0606406)
(90, 0.0463726)
(91, 0.04118)
(92, 0.05611)
(93, 0.0734821)
(94, 0.121503)
(95, 0.165021)
(96, 0.154955)
(97, 0.248766)
(98, 0.186978)
(99, 0.168763)
(100, 0.14713)
(101, 0.158156)
(102, 0.240663)
(103, 0.231845)
(104, 0.0911499)
(105, 0.0891435)
(106, 0.125788)
(107, 0.134883)
(108, 0.0995881)
(109, 0.0762989)
(110, 0.10029)
(111, 0.0695702)
(112, 0.0597155)
(113, 0.0277987)
(114, 0.0342365)
(115, 0.0414481)
(116, 0.0526087)
(117, 0.055459)
(118, 0.0586795)
(119, 0.0763456)
(120, 0.086003)
(121, 0.0952145)
(122, 0.0838606)
(123, 0.0627222)
(124, 0.0449958)
(125, 0.03479)
(126, 0.0468655)
(127, 0.0248035)
(128, 0.0194014)
(129, 0.022732)
(130, 0.0311905)
(131, 0.0253338)
(132, 0.0120972)
(133, 0.00996289)
(134, 0.00729308)
(135, 0.0081289)
(136, 0.00432915)
(137, 0.00291245)
(138, 0.0031448)
(139, 0.00205045)
(140, 0.00166908)
(141, 0.00183198)
(142, 0.00139866)
(143, 0.00145038)
(144, 0.00155495)
(145, 0.002431)
(146, 0.00414268)
(147, 0.00437671)
(148, 0.00278427)
(149, 0.00175121)
(150, 0.00142702)
(151, 0.00107574)
(152, 0.000823156)
(153, 0.00102347)
(154, 0.000825843)
(155, 0.00136171)
(156, 0.00164836)
(157, 0.00106561)
(158, 0.000783001)
(159, 0.00110235)
(160, 0.00156627)
(161, 0.00174186)
(162, 0.0012144)
(163, 0.000680383)
(164, 0.000658718)
(165, 0.000577024)
(166, 0.000527569)
(167, 0.000562807)
(168, 0.000432107)
(169, 0.000270122)
(170, 0.000285096)
(171, 0.000219786)
(172, 0.000269713)
(173, 0.000285803)
(174, 0.000177004)
(175, 0.00016318)
(176, 0.000259984)
(177, 0.000291178)
(178, 0.000275319)
(179, 0.000133054)
(180, 0.00013372)
(181, 0.00016597)
(182, 0.000154126)
(183, 0.000171118)
(184, 0.00018344)
(185, 0.000184857)
(186, 0.000186448)
(187, 0.00026275)
(188, 0.00021361)
(189, 0.000118083)
(190, 9.47075e-05)
(191, 0.00015621)
(192, 0.00015466)
(193, 0.000149827)
(194, 0.000155008)
(195, 0.000180638)
(196, 0.000178174)
(197, 0.000111621)
(198, 0.00012683)
(199, 0.000159786)
(200, 0.000342895)
(201, 0.000377378)
(202, 0.000246136)
(203, 0.000281835)
(204, 0.000370639)
(205, 0.00048835)
(206, 0.00022412)
(207, 0.00017977)
(208, 0.000115431)
(209, 8.76503e-05)
(210, 0.00010416)
(211, 8.19819e-05)
(212, 8.14726e-05)
(213, 6.91338e-05)
(214, 6.26496e-05)
(215, 6.73172e-05)
(216, 7.07225e-05)
(217, 4.6813e-05)
(218, 4.53506e-05)
(219, 4.37181e-05)
(220, 3.34886e-05)
(221, 3.32309e-05)
(222, 3.64862e-05)
(223, 2.77668e-05)
(224, 4.03581e-05)
(225, 7.29366e-05)
(226, 0.000119618)
(227, 0.000100149)
(228, 9.5503e-05)
(229, 0.000125064)
(230, 0.000223553)
(231, 0.00022621)
(232, 0.000165505)
(233, 0.000193941)
(234, 0.000165927)
(235, 0.000158285)
(236, 0.000114016)
(237, 9.41096e-05)
(238, 5.53697e-05)
(239, 7.52328e-05)
(240, 9.88481e-05)
(241, 8.22906e-05)
(242, 5.85942e-05)
(243, 3.30033e-05)
(244, 3.19633e-05)
(245, 3.09533e-05)
(246, 2.06743e-05)
(247, 1.65598e-05)
}; \label{plot:fp16} 
\addplot[color=mydeepblue, line width=1.0pt, dashed] coordinates { 
(0, 1)
(1, 0.657097)
(2, 0.626965)
(3, 0.612147)
(4, 0.887326)
(5, 0.744882)
(6, 0.751643)
(7, 0.651591)
(8, 0.705007)
(9, 0.607611)
(10, 0.682987)
(11, 0.451794)
(12, 0.577344)
(13, 0.673018)
(14, 0.687341)
(15, 0.796501)
(16, 0.52864)
(17, 0.71715)
(18, 0.813362)
(19, 0.751568)
(20, 0.646775)
(21, 0.497938)
(22, 0.348251)
(23, 0.436799)
(24, 0.412782)
(25, 0.301714)
(26, 0.264768)
(27, 0.279855)
(28, 0.30366)
(29, 0.364867)
(30, 0.351715)
(31, 0.492873)
(32, 0.52018)
(33, 0.44369)
(34, 0.29178)
(35, 0.322314)
(36, 0.293845)
(37, 0.346179)
(38, 0.325833)
(39, 0.245966)
(40, 0.206203)
(41, 0.27924)
(42, 0.149116)
(43, 0.166875)
(44, 0.191896)
(45, 0.165157)
(46, 0.163155)
(47, 0.152217)
(48, 0.277801)
(49, 0.316657)
(50, 0.28346)
(51, 0.243625)
(52, 0.234157)
(53, 0.373968)
(54, 0.339603)
(55, 0.252306)
(56, 0.241582)
(57, 0.353012)
(58, 0.247743)
(59, 0.16842)
(60, 0.123326)
(61, 0.14221)
(62, 0.228992)
(63, 0.248467)
(64, 0.191381)
(65, 0.185029)
(66, 0.186684)
(67, 0.199492)
(68, 0.0917623)
(69, 0.143239)
(70, 0.150069)
(71, 0.0733334)
(72, 0.0589253)
(73, 0.0833711)
(74, 0.0705768)
(75, 0.0507061)
(76, 0.0393728)
(77, 0.0383904)
(78, 0.0686544)
(79, 0.0418337)
(80, 0.0303812)
(81, 0.0513325)
(82, 0.100524)
(83, 0.131614)
(84, 0.226641)
(85, 0.111584)
(86, 0.148111)
(87, 0.178572)
(88, 0.120635)
(89, 0.157127)
(90, 0.214589)
(91, 0.0700793)
(92, 0.155447)
(93, 0.0782487)
(94, 0.118014)
(95, 0.0790907)
(96, 0.046681)
(97, 0.0222818)
(98, 0.0385128)
(99, 0.0629179)
(100, 0.0459744)
(101, 0.0504867)
(102, 0.0808305)
(103, 0.123965)
(104, 0.0830965)
(105, 0.0260945)
(106, 0.0274134)
(107, 0.032265)
(108, 0.0190329)
(109, 0.0160611)
(110, 0.0381793)
(111, 0.010062)
(112, 0.00051849)
(113, 0.00733314)
(114, 0.00343915)
(115, 0.00116387)
(116, 0.000310481)
(117, 0.000444095)
(118, 0.00121948)
(119, 0.000453085)
(120, 0.000238609)
(121, 0.000215127)
(122, 0.000860479)
(123, 0.000346307)
(124, 4.86395e-05)
(125, 4.35674e-05)
(126, 4.02351e-05)
(127, 5.99801e-05)
(128, 0.000184685)
(129, 7.46821e-05)
(130, 1.01367e-05)
(131, 3.50417e-06)
(132, 1.87506e-06)
(133, 5.07827e-07)
(134, 4.80525e-07)
(135, 6.28776e-08)
(136, 1.2597e-07)
(137, 1.5747e-07)
(138, 3.70535e-07)
(139, 5.86938e-07)
(140, 8.88571e-07)
(141, 1.10419e-06)
(142, 2.59454e-07)
(143, 1.64997e-07)
(144, 7.82534e-08)
(145, 6.21855e-08)
(146, 4.47874e-08)
(147, 1.66631e-08)
(148, 2.13804e-08)
(149, 3.04461e-08)
(150, 7.54495e-08)
(151, 7.29143e-08)
(152, 8.8989e-08)
(153, 6.07009e-08)
(154, 3.06564e-08)
(155, 1.80432e-08)
(156, 1.30006e-08)
(157, 4.55156e-09)
(158, 3.97642e-09)
(159, 4.00521e-09)
(160, 8.14253e-09)
(161, 1.11224e-08)
(162, 7.81709e-09)
(163, 8.85252e-09)
(164, 2.05518e-08)
(165, 1.88247e-08)
(166, 2.63815e-08)
(167, 3.21077e-08)
(168, 4.04666e-08)
(169, 3.9967e-08)
(170, 5.55315e-08)
(171, 2.46269e-08)
(172, 1.57213e-08)
(173, 1.0879e-08)
(174, 1.38512e-08)
(175, 7.081e-09)
(176, 3.04468e-09)
(177, 2.74477e-09)
(178, 3.0487e-09)
(179, 2.87635e-09)
(180, 2.50542e-09)
(181, 1.52239e-09)
(182, 6.45497e-10)
(183, 3.03917e-10)
(184, 3.96314e-10)
(185, 4.6787e-10)
(186, 1.30715e-10)
(187, 1.05647e-10)
(188, 7.34702e-11)
(189, 4.2517e-11)
(190, 4.71584e-11)
(191, 5.12196e-11)
(192, 4.36294e-11)
(193, 1.57038e-11)
(194, 1.26351e-11)
(195, 9.72029e-12)
(196, 7.64189e-12)
(197, 6.55373e-12)
(198, 2.55419e-12)
(199, 2.25637e-12)
(200, 2.47786e-12)
(201, 3.06532e-12)
(202, 2.00213e-12)
(203, 1.07964e-12)
(204, 7.66691e-13)
(205, 1.1925e-12)
(206, 7.13983e-13)
(207, 7.80667e-13)
(208, 6.91461e-13)
(209, 4.58374e-13)
(210, 1.69824e-13)
(211, 2.17882e-13)
(212, 2.21203e-13)
(213, 1.9374e-13)
(214, 1.45961e-13)
(215, 1.09442e-13)
(216, 1.19085e-13)
(217, 1.98105e-13)
(218, 8.22874e-14)
(219, 4.00415e-14)
(220, 3.65371e-14)
(221, 5.07126e-14)
(222, 5.35688e-14)
(223, 5.21062e-14)
(224, 5.92427e-14)
(225, 8.40919e-14)
(226, 4.73295e-14)
(227, 1.66295e-14)
(228, 1.92869e-14)
(229, 1.75338e-14)
(230, 1.67112e-14)
(231, 1.62899e-14)
(232, 1.09787e-14)
(233, 6.81884e-15)
(234, 1.58185e-14)
(235, 2.10594e-14)
(236, 4.77055e-15)
(237, 1.07888e-14)
(238, 1.75704e-14)
(239, 4.2461e-14)
(240, 3.69317e-14)
(241, 1.14503e-14)
(242, 9.71405e-15)
(243, 1.14596e-14)
(244, 1.0741e-14)
(245, 9.3457e-15)
(246, 1.22718e-14)
(247, 1.27312e-14)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=x, color=red,   mark size=3pt, line width=1.5pt] coordinates { 
 (131, 1.01367e-05) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=x, color=black,   mark size=3pt, line width=1.5pt] coordinates { 
 (133, 1.87506e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks,  mark=o, color=blue,  mark size=3pt, line width=1.0pt] coordinates { 
 (182, 1.52239e-09) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/okCond_3_trueRes.tex <==
\addplot[color=myyellow, line width=1.0pt] coordinates { 
(0, 1)
(1, 0.657097)
(2, 0.626965)
(3, 0.612147)
(4, 0.887326)
(5, 0.744882)
(6, 0.751643)
(7, 0.651591)
(8, 0.705007)
(9, 0.607611)
(10, 0.682987)
(11, 0.451794)
(12, 0.577344)
(13, 0.673018)
(14, 0.687341)
(15, 0.796501)
(16, 0.52864)
(17, 0.71715)
(18, 0.813362)
(19, 0.751568)
(20, 0.646775)
(21, 0.497938)
(22, 0.348251)
(23, 0.436799)
(24, 0.412782)
(25, 0.301714)
(26, 0.264768)
(27, 0.279855)
(28, 0.30366)
(29, 0.364867)
(30, 0.351715)
(31, 0.492873)
(32, 0.52018)
(33, 0.44369)
(34, 0.29178)
(35, 0.322314)
(36, 0.293845)
(37, 0.346179)
(38, 0.325833)
(39, 0.245966)
(40, 0.206203)
(41, 0.27924)
(42, 0.149116)
(43, 0.166875)
(44, 0.191896)
(45, 0.165155)
(46, 0.163154)
(47, 0.15222)
(48, 0.277802)
(49, 0.316657)
(50, 0.283461)
(51, 0.24363)
(52, 0.234253)
(53, 0.375595)
(54, 0.37043)
(55, 0.243425)
(56, 0.239563)
(57, 0.352944)
(58, 0.247774)
(59, 0.168471)
(60, 0.123437)
(61, 0.146105)
(62, 0.218556)
(63, 0.242172)
(64, 0.191306)
(65, 0.185013)
(66, 0.186682)
(67, 0.199486)
(68, 0.0916318)
(69, 0.143667)
(70, 0.15015)
(71, 0.0733129)
(72, 0.0587494)
(73, 0.0723524)
(74, 0.0803343)
(75, 0.0508311)
(76, 0.0385857)
(77, 0.0375881)
(78, 0.0805716)
(79, 0.0625984)
(80, 0.0280928)
(81, 0.0442261)
(82, 0.101735)
(83, 0.141375)
(84, 0.183947)
(85, 0.109199)
(86, 0.125388)
(87, 0.287517)
(88, 0.121051)
(89, 0.155141)
(90, 0.13267)
(91, 0.0791222)
(92, 0.185556)
(93, 0.0738948)
(94, 0.115187)
(95, 0.0644363)
(96, 0.0517909)
(97, 0.0254997)
(98, 0.0296805)
(99, 0.0624145)
(100, 0.0490592)
(101, 0.0567303)
(102, 0.0578281)
(103, 0.12262)
(104, 0.0835629)
(105, 0.0298219)
(106, 0.0245132)
(107, 0.0512089)
(108, 0.0232443)
(109, 0.0186591)
(110, 0.0181014)
(111, 0.00681872)
(112, 0.000518876)
(113, 0.00512431)
(114, 0.00263268)
(115, 0.000460935)
(116, 0.000321684)
(117, 0.000726678)
(118, 0.00138042)
(119, 0.000406283)
(120, 0.00016828)
(121, 0.000581363)
(122, 0.000669597)
(123, 0.000328319)
(124, 7.00672e-05)
(125, 3.9676e-05)
(126, 3.30864e-05)
(127, 0.000103518)
(128, 9.56321e-05)
(129, 2.18721e-05)
(130, 6.83033e-06)
(131, 1.77798e-06)
(132, 7.31555e-07)
(133, 1.16603e-07)
(134, 1.48807e-07)
(135, 7.32755e-08)
(136, 2.34471e-07)
(137, 1.74986e-07)
(138, 2.83145e-07)
(139, 5.06056e-07)
(140, 7.6323e-07)
(141, 1.14375e-06)
(142, 5.74382e-07)
(143, 2.02297e-07)
(144, 1.28236e-07)
(145, 6.83471e-08)
(146, 6.40223e-08)
(147, 2.27104e-08)
(148, 1.88314e-08)
(149, 2.21392e-08)
(150, 4.11452e-08)
(151, 6.29169e-08)
(152, 7.40709e-08)
(153, 5.68269e-08)
(154, 3.67616e-08)
(155, 3.44727e-08)
(156, 1.77146e-08)
(157, 8.85564e-09)
(158, 7.86054e-09)
(159, 6.78322e-09)
(160, 4.23092e-09)
(161, 3.59732e-09)
(162, 8.76386e-09)
(163, 6.62565e-09)
(164, 1.29547e-08)
(165, 9.80455e-09)
(166, 2.51149e-08)
(167, 3.15071e-08)
(168, 3.40151e-08)
(169, 3.06253e-08)
(170, 3.57897e-08)
(171, 4.96371e-08)
(172, 1.23641e-08)
(173, 2.46365e-09)
(174, 2.18558e-09)
(175, 1.39899e-09)
(176, 1.73854e-09)
(177, 1.2976e-09)
(178, 1.26946e-09)
(179, 7.488e-10)
(180, 4.03286e-10)
(181, 4.89394e-10)
(182, 3.34196e-10)
(183, 1.24636e-10)
(184, 1.09107e-10)
(185, 7.88993e-11)
(186, 7.82106e-11)
(187, 3.83034e-11)
(188, 2.2124e-11)
(189, 3.25652e-11)
(190, 2.23142e-11)
(191, 7.59111e-12)
(192, 1.01327e-11)
(193, 1.16295e-11)
(194, 1.18974e-11)
(195, 3.44211e-12)
(196, 3.12697e-12)
(197, 1.87531e-12)
(198, 1.73792e-12)
(199, 3.43301e-12)
(200, 1.31405e-12)
(201, 1.30819e-12)
(202, 4.50529e-13)
(203, 3.36478e-13)
(204, 2.75789e-13)
(205, 2.89658e-13)
(206, 2.25954e-13)
(207, 2.84196e-13)
(208, 2.47784e-13)
(209, 2.07961e-13)
(210, 2.10029e-13)
(211, 2.09711e-13)
(212, 2.08523e-13)
(213, 2.09931e-13)
(214, 2.11301e-13)
(215, 2.10691e-13)
(216, 2.10916e-13)
(217, 2.10046e-13)
(218, 2.10283e-13)
(219, 2.09931e-13)
}; \label{plot:fp64} 
\addplot[ color=mygreen, line width=1.0pt, dotted] coordinates { 
(0, 1)
(1, 0.657097)
(2, 0.626969)
(3, 0.61218)
(4, 0.887379)
(5, 0.745014)
(6, 0.751659)
(7, 0.651488)
(8, 0.702497)
(9, 0.608023)
(10, 0.683546)
(11, 0.451404)
(12, 0.576561)
(13, 0.675273)
(14, 0.686542)
(15, 0.797353)
(16, 0.528316)
(17, 0.717824)
(18, 0.814784)
(19, 0.749718)
(20, 0.645813)
(21, 0.501879)
(22, 0.360253)
(23, 0.475967)
(24, 0.441865)
(25, 0.358917)
(26, 0.272075)
(27, 0.26025)
(28, 0.345323)
(29, 0.349715)
(30, 0.413883)
(31, 0.338758)
(32, 0.525408)
(33, 0.490206)
(34, 0.459016)
(35, 0.306141)
(36, 0.33388)
(37, 0.377177)
(38, 0.327658)
(39, 0.344489)
(40, 0.287659)
(41, 0.246799)
(42, 0.223234)
(43, 0.262885)
(44, 0.151199)
(45, 0.16697)
(46, 0.227659)
(47, 0.186428)
(48, 0.149042)
(49, 0.153463)
(50, 0.235352)
(51, 0.395348)
(52, 0.354909)
(53, 0.318032)
(54, 0.293851)
(55, 0.285128)
(56, 0.27573)
(57, 0.398938)
(58, 0.364097)
(59, 0.265041)
(60, 0.23663)
(61, 0.407671)
(62, 0.346657)
(63, 0.191204)
(64, 0.131047)
(65, 0.151038)
(66, 0.18035)
(67, 0.204915)
(68, 0.254313)
(69, 0.276857)
(70, 0.230446)
(71, 0.156691)
(72, 0.241321)
(73, 0.197491)
(74, 0.161452)
(75, 0.112267)
(76, 0.110158)
(77, 0.163728)
(78, 0.128158)
(79, 0.0582655)
(80, 0.0719907)
(81, 0.0798942)
(82, 0.0733285)
(83, 0.0660826)
(84, 0.0491526)
(85, 0.0415009)
(86, 0.0437196)
(87, 0.0727482)
(88, 0.0694106)
(89, 0.0606406)
(90, 0.0463726)
(91, 0.04118)
(92, 0.05611)
(93, 0.0734821)
(94, 0.121503)
(95, 0.165021)
(96, 0.154955)
(97, 0.248766)
(98, 0.186978)
(99, 0.168763)
(100, 0.14713)
(101, 0.158156)
(102, 0.240663)
(103, 0.231845)
(104, 0.0911499)
(105, 0.0891435)
(106, 0.125788)
(107, 0.134883)
(108, 0.0995881)
(109, 0.0762989)
(110, 0.10029)
(111, 0.0695702)
(112, 0.0597155)
(113, 0.0277987)
(114, 0.0342365)
(115, 0.0414481)
(116, 0.0526087)
(117, 0.055459)
(118, 0.0586795)
(119, 0.0763456)
(120, 0.086003)
(121, 0.0952145)
(122, 0.0838606)
(123, 0.0627222)
(124, 0.0449958)
(125, 0.03479)
(126, 0.0468655)
(127, 0.0248035)
(128, 0.0194014)
(129, 0.022732)
(130, 0.0311905)
(131, 0.0253338)
(132, 0.0120972)
(133, 0.00996289)
(134, 0.00729308)
(135, 0.0081289)
(136, 0.00432915)
(137, 0.00291245)
(138, 0.0031448)
(139, 0.00205045)
(140, 0.00166908)
(141, 0.00183198)
(142, 0.00139866)
(143, 0.00145038)
(144, 0.00155495)
(145, 0.002431)
(146, 0.00414268)
(147, 0.00437671)
(148, 0.00278427)
(149, 0.00175121)
(150, 0.00142702)
(151, 0.00107574)
(152, 0.000823156)
(153, 0.00102347)
(154, 0.000825843)
(155, 0.00136171)
(156, 0.00164836)
(157, 0.00106561)
(158, 0.000783001)
(159, 0.00110235)
(160, 0.00156627)
(161, 0.00174186)
(162, 0.0012144)
(163, 0.000680383)
(164, 0.000658718)
(165, 0.000577024)
(166, 0.000527569)
(167, 0.000562807)
(168, 0.000432107)
(169, 0.000270122)
(170, 0.000285096)
(171, 0.000219786)
(172, 0.000269713)
(173, 0.000285803)
(174, 0.000177004)
(175, 0.00016318)
(176, 0.000259984)
(177, 0.000291178)
(178, 0.000275319)
(179, 0.000133054)
(180, 0.00013372)
(181, 0.00016597)
(182, 0.000154126)
(183, 0.000171118)
(184, 0.00018344)
(185, 0.000184857)
(186, 0.000186448)
(187, 0.00026275)
(188, 0.00021361)
(189, 0.000118083)
(190, 9.47075e-05)
(191, 0.00015621)
(192, 0.00015466)
(193, 0.000149827)
(194, 0.000155008)
(195, 0.000180638)
(196, 0.000178174)
(197, 0.000111621)
(198, 0.00012683)
(199, 0.000159786)
(200, 0.000342895)
(201, 0.000377378)
(202, 0.000246136)
(203, 0.000281835)
(204, 0.000370639)
(205, 0.00048835)
(206, 0.00022412)
(207, 0.00017977)
(208, 0.000115431)
(209, 8.76503e-05)
(210, 0.00010416)
(211, 8.19819e-05)
(212, 8.14726e-05)
(213, 6.91338e-05)
(214, 6.26496e-05)
(215, 6.73172e-05)
(216, 7.07225e-05)
(217, 4.6813e-05)
(218, 4.53506e-05)
(219, 4.37181e-05)
(220, 3.34886e-05)
(221, 3.32309e-05)
(222, 3.64862e-05)
(223, 2.77668e-05)
(224, 4.03581e-05)
(225, 7.29366e-05)
(226, 0.000119618)
(227, 0.000100149)
(228, 9.5503e-05)
(229, 0.000125064)
(230, 0.000223553)
(231, 0.00022621)
(232, 0.000165505)
(233, 0.000193941)
(234, 0.000165927)
(235, 0.000158285)
(236, 0.000114016)
(237, 9.41096e-05)
(238, 5.53697e-05)
(239, 7.52328e-05)
(240, 9.88481e-05)
(241, 8.22906e-05)
(242, 5.85942e-05)
(243, 3.30033e-05)
(244, 3.19633e-05)
(245, 3.09533e-05)
(246, 2.06743e-05)
(247, 1.65598e-05)
}; \label{plot:fp16} 
\addplot[color=mydeepblue, line width=1.0pt, dashed] coordinates { 
(0, 1)
(1, 0.657097)
(2, 0.626965)
(3, 0.612147)
(4, 0.887326)
(5, 0.744882)
(6, 0.751643)
(7, 0.651591)
(8, 0.705007)
(9, 0.607611)
(10, 0.682987)
(11, 0.451794)
(12, 0.577344)
(13, 0.673018)
(14, 0.687341)
(15, 0.796501)
(16, 0.52864)
(17, 0.71715)
(18, 0.813362)
(19, 0.751568)
(20, 0.646775)
(21, 0.497938)
(22, 0.348251)
(23, 0.436799)
(24, 0.412782)
(25, 0.301714)
(26, 0.264768)
(27, 0.279855)
(28, 0.30366)
(29, 0.364867)
(30, 0.351715)
(31, 0.492873)
(32, 0.52018)
(33, 0.44369)
(34, 0.29178)
(35, 0.322314)
(36, 0.293845)
(37, 0.346179)
(38, 0.325833)
(39, 0.245966)
(40, 0.206203)
(41, 0.27924)
(42, 0.149116)
(43, 0.166875)
(44, 0.191896)
(45, 0.165157)
(46, 0.163155)
(47, 0.152217)
(48, 0.277801)
(49, 0.316657)
(50, 0.28346)
(51, 0.243625)
(52, 0.234157)
(53, 0.373968)
(54, 0.339603)
(55, 0.252306)
(56, 0.241582)
(57, 0.353012)
(58, 0.247743)
(59, 0.16842)
(60, 0.123326)
(61, 0.14221)
(62, 0.228992)
(63, 0.248467)
(64, 0.191381)
(65, 0.185029)
(66, 0.186684)
(67, 0.199492)
(68, 0.0917623)
(69, 0.143239)
(70, 0.150069)
(71, 0.0733334)
(72, 0.0589253)
(73, 0.0833711)
(74, 0.0705768)
(75, 0.0507061)
(76, 0.0393728)
(77, 0.0383904)
(78, 0.0686544)
(79, 0.0418337)
(80, 0.0303812)
(81, 0.0513325)
(82, 0.100524)
(83, 0.131614)
(84, 0.226641)
(85, 0.111584)
(86, 0.148111)
(87, 0.178572)
(88, 0.120635)
(89, 0.157127)
(90, 0.214589)
(91, 0.0700793)
(92, 0.155447)
(93, 0.0782487)
(94, 0.118014)
(95, 0.0790907)
(96, 0.046681)
(97, 0.0222818)
(98, 0.0385128)
(99, 0.0629179)
(100, 0.0459744)
(101, 0.0504867)
(102, 0.0808305)
(103, 0.123965)
(104, 0.0830965)
(105, 0.0260945)
(106, 0.0274134)
(107, 0.032265)
(108, 0.0190329)
(109, 0.0160611)
(110, 0.0381793)
(111, 0.010062)
(112, 0.00051849)
(113, 0.00733314)
(114, 0.00343915)
(115, 0.00116387)
(116, 0.000310481)
(117, 0.000444095)
(118, 0.00121948)
(119, 0.000453085)
(120, 0.000238609)
(121, 0.000215127)
(122, 0.000860479)
(123, 0.000346307)
(124, 4.86395e-05)
(125, 4.35674e-05)
(126, 4.02351e-05)
(127, 5.99801e-05)
(128, 0.000184685)
(129, 7.46821e-05)
(130, 1.01367e-05)
(131, 3.50417e-06)
(132, 1.87506e-06)
(133, 5.07827e-07)
(134, 4.80525e-07)
(135, 6.28776e-08)
(136, 1.25971e-07)
(137, 1.5747e-07)
(138, 3.70535e-07)
(139, 5.86938e-07)
(140, 8.88571e-07)
(141, 1.10419e-06)
(142, 2.59454e-07)
(143, 1.64997e-07)
(144, 7.82534e-08)
(145, 6.21855e-08)
(146, 4.47873e-08)
(147, 1.66631e-08)
(148, 2.13804e-08)
(149, 3.04461e-08)
(150, 7.54495e-08)
(151, 7.29143e-08)
(152, 8.8989e-08)
(153, 6.07009e-08)
(154, 3.06565e-08)
(155, 1.80432e-08)
(156, 1.30006e-08)
(157, 4.55156e-09)
(158, 3.97641e-09)
(159, 4.00522e-09)
(160, 8.14252e-09)
(161, 1.11224e-08)
(162, 7.81708e-09)
(163, 8.85253e-09)
(164, 2.05518e-08)
(165, 1.88247e-08)
(166, 2.63815e-08)
(167, 3.21077e-08)
(168, 4.04666e-08)
(169, 3.9967e-08)
(170, 5.55315e-08)
(171, 2.46269e-08)
(172, 1.57213e-08)
(173, 1.0879e-08)
(174, 1.38512e-08)
(175, 7.08099e-09)
(176, 3.04468e-09)
(177, 2.74476e-09)
(178, 3.04871e-09)
(179, 2.87634e-09)
(180, 2.50543e-09)
(181, 1.52239e-09)
(182, 6.45484e-10)
(183, 3.0394e-10)
(184, 3.96288e-10)
(185, 4.6787e-10)
(186, 1.30701e-10)
(187, 1.0567e-10)
(188, 7.34721e-11)
(189, 4.25064e-11)
(190, 4.71678e-11)
(191, 5.12154e-11)
(192, 4.36496e-11)
(193, 1.57034e-11)
(194, 1.26263e-11)
(195, 9.72671e-12)
(196, 7.64041e-12)
(197, 6.55871e-12)
(198, 2.55824e-12)
(199, 2.25727e-12)
(200, 2.47772e-12)
(201, 3.06731e-12)
(202, 2.00831e-12)
(203, 1.08501e-12)
(204, 7.74244e-13)
(205, 1.204e-12)
(206, 7.0484e-13)
(207, 8.09662e-13)
(208, 6.95949e-13)
(209, 4.49565e-13)
(210, 2.08406e-13)
(211, 2.49883e-13)
(212, 2.56572e-13)
(213, 2.06497e-13)
(214, 2.07427e-13)
(215, 1.60786e-13)
(216, 1.77328e-13)
(217, 2.37989e-13)
(218, 1.4913e-13)
(219, 1.2796e-13)
(220, 1.35276e-13)
(221, 1.26717e-13)
(222, 1.38267e-13)
(223, 1.44275e-13)
(224, 1.46345e-13)
(225, 1.7024e-13)
(226, 1.46092e-13)
(227, 1.38404e-13)
(228, 1.48488e-13)
(229, 1.60627e-13)
(230, 1.73697e-13)
(231, 1.73768e-13)
(232, 1.71396e-13)
(233, 1.76109e-13)
(234, 1.81875e-13)
(235, 1.79032e-13)
(236, 1.8779e-13)
(237, 2.03009e-13)
(238, 1.99796e-13)
(239, 2.06512e-13)
(240, 2.11419e-13)
(241, 2.09362e-13)
(242, 2.13439e-13)
(243, 2.09406e-13)
(244, 2.03757e-13)
(245, 1.92009e-13)
(246, 1.87158e-13)
(247, 1.90559e-13)
}; \label{plot:fp64mixed} 
 \addplot[only marks, mark=x, color=red,   mark size=3pt, line width=1.5pt] coordinates { 
 (131, 1.01367e-05) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks, mark=x, color=black,   mark size=3pt, line width=1.5pt] coordinates { 
 (133, 1.87506e-06) 
}; \label{plot:fp64tofp32} 
 \addplot[only marks,  mark=o, color=blue,  mark size=3pt, line width=1.0pt] coordinates { 
 (182, 1.52239e-09) 
}; \label{plot:residualfp64tofp32} 


==> 5.Numerical/data/smallCond_1eig.tex <==
\addplot[only marks, mark=o, mark size=1pt, color=black, line width=0.5pt] coordinates {
(1, 0.1)
(2, 0.109091)
(3, 0.118182)
(4, 0.127273)
(5, 0.136364)
(6, 0.145455)
(7, 0.154545)
(8, 0.163636)
(9, 0.172727)
(10, 0.181818)
(11, 0.190909)
(12, 0.2)
(13, 0.209091)
(14, 0.218182)
(15, 0.227273)
(16, 0.236364)
(17, 0.245455)
(18, 0.254545)
(19, 0.263636)
(20, 0.272727)
(21, 0.281818)
(22, 0.290909)
(23, 0.3)
(24, 0.309091)
(25, 0.318182)
(26, 0.327273)
(27, 0.336364)
(28, 0.345455)
(29, 0.354545)
(30, 0.363636)
(31, 0.372727)
(32, 0.381818)
(33, 0.390909)
(34, 0.4)
(35, 0.409091)
(36, 0.418182)
(37, 0.427273)
(38, 0.436364)
(39, 0.445455)
(40, 0.454545)
(41, 0.463636)
(42, 0.472727)
(43, 0.481818)
(44, 0.490909)
(45, 0.5)
(46, 0.509091)
(47, 0.518182)
(48, 0.527273)
(49, 0.536364)
(50, 0.545455)
(51, 0.554545)
(52, 0.563636)
(53, 0.572727)
(54, 0.581818)
(55, 0.590909)
(56, 0.6)
(57, 0.609091)
(58, 0.618182)
(59, 0.627273)
(60, 0.636364)
(61, 0.645455)
(62, 0.654545)
(63, 0.663636)
(64, 0.672727)
(65, 0.681818)
(66, 0.690909)
(67, 0.7)
(68, 0.709091)
(69, 0.718182)
(70, 0.727273)
(71, 0.736364)
(72, 0.745455)
(73, 0.754545)
(74, 0.763636)
(75, 0.772727)
(76, 0.781818)
(77, 0.790909)
(78, 0.8)
(79, 0.809091)
(80, 0.818182)
(81, 0.827273)
(82, 0.836364)
(83, 0.845455)
(84, 0.854545)
(85, 0.863636)
(86, 0.872727)
(87, 0.881818)
(88, 0.890909)
(89, 0.9)
(90, 0.909091)
(91, 0.918182)
(92, 0.927273)
(93, 0.936364)
(94, 0.945455)
(95, 0.954545)
(96, 0.963636)
(97, 0.972727)
(98, 0.981818)
(99, 0.990909)
(100, 1)
}; \label{plot:eig}

==> 5.Numerical/data/smallCond_2eig.tex <==
\addplot[only marks, mark=o, mark size=1pt, color=black, line width=0.5pt] coordinates {
(1, 0.0126325) 
(2, 0.0131618) 
(3, 0.013786) 
(4, 0.0186857) 
(5, 0.0199942) 
(6, 0.0235834) 
(7, 0.0292466) 
(8, 0.033128) 
(9, 0.0379067) 
(10, 0.0426078) 
(11, 0.0470415) 
(12, 0.054006) 
(13, 0.0602899) 
(14, 0.0670692) 
(15, 0.0745456) 
(16, 0.0838024) 
(17, 0.0919002) 
(18, 0.10089) 
(19, 0.110759) 
(20, 0.120011) 
(21, 0.130786) 
(22, 0.141827) 
(23, 0.152735) 
(24, 0.164815) 
(25, 0.176528) 
(26, 0.188807) 
(27, 0.201491) 
(28, 0.214819) 
(29, 0.227984) 
(30, 0.241282) 
(31, 0.256019) 
(32, 0.269524) 
(33, 0.2835) 
(34, 0.298123) 
(35, 0.312934) 
(36, 0.328116) 
(37, 0.343202) 
(38, 0.358437) 
(39, 0.374021) 
(40, 0.390811) 
(41, 0.406226) 
(42, 0.423994) 
(43, 0.440526) 
(44, 0.457816) 
(45, 0.474166) 
(46, 0.490369) 
(47, 0.505065) 
(48, 0.52155) 
(49, 0.537672) 
(50, 0.554444) 
(51, 0.565327) 
(52, 0.572749) 
(53, 0.588136) 
(54, 0.600991) 
(55, 0.615549) 
(56, 0.629938) 
(57, 0.64611) 
(58, 0.661849) 
(59, 0.678514) 
(60, 0.693074) 
(61, 0.70709) 
(62, 0.722918) 
(63, 0.740558) 
(64, 0.755086) 
(65, 0.770978) 
(66, 0.78207) 
(67, 0.7964) 
(68, 0.811436) 
(69, 0.823376) 
(70, 0.836898) 
(71, 0.848131) 
(72, 0.862981) 
(73, 0.873269) 
(74, 0.885074) 
(75, 0.891972) 
(76, 0.902885) 
(77, 0.914623) 
(78, 0.924847) 
(79, 0.93099) 
(80, 0.941137) 
(81, 0.947876) 
(82, 0.958347) 
(83, 0.963258) 
(84, 0.968255) 
(85, 0.976753) 
(86, 0.98167) 
(87, 0.988143) 
(88, 0.989117) 
(89, 0.995017) 
(90, 0.99672) 
(91, 0.999277) 
(92, 1.00258) 
(93, 1.00962) 
(94, 1.0119) 
}; 
% \label{plot:eig}

==> 5.Numerical/data/varyConditionNum1e1.tex <==
\addplot[color=vtorange, line width=1.5pt] coordinates {
(0, 1)
(1, 0.450237)
(2, 0.241371)
(3, 0.124143)
(4, 0.0711549)
(5, 0.0392425)
(6, 0.0225448)
(7, 0.0123136)
(8, 0.00671121)
(9, 0.00303886)
(10, 0.00144141)
(11, 0.000708016)
(12, 0.000299382)
(13, 0.000150875)
(14, 7.22692e-05)
(15, 3.72076e-05)
(16, 1.8776e-05)
(17, 9.46672e-06)
(18, 5.13553e-06)
(19, 2.81192e-06)
(20, 1.33554e-06)
(21, 6.41582e-07)
(22, 3.58113e-07)
(23, 1.76425e-07)
(24, 9.16291e-08)
(25, 4.69805e-08)
(26, 2.14895e-08)
(27, 1.21123e-08)
(28, 5.2812e-09)
(29, 2.49971e-09)
(30, 1.09875e-09)
(31, 5.9054e-10)
(32, 2.96888e-10)
(33, 1.37048e-10)
(34, 7.37411e-11)
(35, 3.89497e-11)
(36, 1.85133e-11)
(37, 8.51672e-12)
(38, 3.54989e-12)
(39, 1.77796e-12)
(40, 7.74556e-13)
(41, 3.78912e-13)
(42, 1.52283e-13)
(43, 7.51034e-14)
}; \label{plot:fp64}
\addplot[ color=mydeepblue, line width=2.5pt, dashed] coordinates {
(0, 1)
(1, 0.450237)
(2, 0.241371)
(3, 0.124143)
(4, 0.0711549)
(5, 0.0392425)
(6, 0.0225448)
(7, 0.0123136)
(8, 0.00671121)
(9, 0.00303886)
(10, 0.00144141)
(11, 0.000708016)
(12, 0.000299382)
(13, 0.000150875)
(14, 7.22692e-05)
(15, 3.72076e-05)
(16, 1.8776e-05)
(17, 9.46671e-06)
(18, 5.13553e-06)
(19, 2.81192e-06)
(20, 1.33554e-06)
(21, 6.41581e-07)
(22, 3.58112e-07)
(23, 1.76425e-07)
(24, 9.1629e-08)
(25, 4.69804e-08)
(26, 2.14895e-08)
(27, 1.21123e-08)
(28, 5.2812e-09)
(29, 2.4997e-09)
(30, 1.09879e-09)
(31, 5.90502e-10)
(32, 2.96877e-10)
(33, 1.37078e-10)
(34, 7.37635e-11)
(35, 3.89603e-11)
(36, 1.85227e-11)
(37, 8.51975e-12)
(38, 3.55131e-12)
(39, 1.77889e-12)
(40, 7.74904e-13)
(41, 3.79099e-13)
(42, 1.52426e-13)
(43, 7.51851e-14)
}; \label{plot:fp64mixed}
\addplot[ color=mygreen, line width=1.5pt, dotted] coordinates {
(0, 1)
(1, 0.450237)
(2, 0.24139)
(3, 0.124169)
(4, 0.0711653)
(5, 0.0392435)
(6, 0.0225403)
(7, 0.0123117)
(8, 0.00671191)
(9, 0.00303879)
(10, 0.00144147)
(11, 0.000708132)
(12, 0.000299417)
(13, 0.000150898)
(14, 7.22164e-05)
(15, 3.72025e-05)
(16, 1.87818e-05)
(17, 9.45716e-06)
(18, 5.13615e-06)
(19, 2.80966e-06)
(20, 1.33482e-06)
(21, 6.41293e-07)
(22, 3.57855e-07)
(23, 1.763e-07)
(24, 9.15889e-08)
(25, 4.69881e-08)
(26, 2.14892e-08)
(27, 1.21207e-08)
(28, 5.28156e-09)
(29, 2.50241e-09)
(30, 1.10124e-09)
(31, 5.92002e-10)
(32, 2.97542e-10)
(33, 1.37452e-10)
(34, 7.40806e-11)
(35, 3.91732e-11)
(36, 1.86369e-11)
(37, 8.60628e-12)
(38, 3.62368e-12)
(39, 1.85431e-12)
(40, 8.46124e-13)
(41, 4.47872e-13)
(42, 2.11443e-13)
(43, 1.31219e-13)
(44, 7.39395e-14)
}; \label{plot:fp16}
\addplot[only marks, mark=*, color=black, mark options={ fill=black}, line width=1.5pt] coordinates {
(15, 3.72076e-05)
}; \label{plot:fp64tofp32}
\addplot[only marks, mark=*, color=mygreen, mark options={ fill=mygreen}, line width=1.5pt] coordinates {
(29, 2.4997e-09)
};\label{plot:fp32tofp16}


 

==> 5.Numerical/data/varyConditionNum1e2.tex <==
\addplot[color=vtorange, line width=1.5pt] coordinates {
(0, 1)
(1, 0.544211)
(2, 0.43881)
(3, 0.369319)
(4, 0.316247)
(5, 0.260111)
(6, 0.235175)
(7, 0.203779)
(8, 0.172092)
(9, 0.133484)
(10, 0.102394)
(11, 0.088253)
(12, 0.0702704)
(13, 0.0605887)
(14, 0.0539195)
(15, 0.0477762)
(16, 0.0427875)
(17, 0.0363957)
(18, 0.0300501)
(19, 0.028704)
(20, 0.0238064)
(21, 0.0151937)
(22, 0.0102092)
(23, 0.00820208)
(24, 0.00494406)
(25, 0.00294587)
(26, 0.00203383)
(27, 0.00169409)
(28, 0.00116747)
(29, 0.000726109)
(30, 0.000484971)
(31, 0.000290553)
(32, 0.000197199)
(33, 0.000125515)
(34, 9.86511e-05)
(35, 6.96263e-05)
(36, 6.05552e-05)
(37, 4.77178e-05)
(38, 3.65238e-05)
(39, 2.36541e-05)
(40, 1.49396e-05)
(41, 8.13123e-06)
(42, 5.23441e-06)
(43, 2.76801e-06)
(44, 1.70529e-06)
(45, 9.97635e-07)
(46, 6.31462e-07)
(47, 4.17748e-07)
(48, 2.68759e-07)
(49, 1.4641e-07)
(50, 8.96047e-08)
(51, 6.58471e-08)
(52, 3.60386e-08)
(53, 1.83715e-08)
(54, 9.16081e-09)
(55, 5.19643e-09)
(56, 2.53474e-09)
(57, 9.99026e-10)
(58, 5.29206e-10)
(59, 3.14666e-10)
(60, 1.6527e-10)
(61, 6.77145e-11)
(62, 3.11337e-11)
(63, 1.47604e-11)
(64, 6.50173e-12)
(65, 2.92525e-12)
(66, 1.28293e-12)
(67, 5.19709e-13)
(68, 2.43188e-13)
(69, 1.04728e-13)
(70, 4.32502e-14)
}; \label{plot:fp64}
\addplot[ color=mydeepblue, line width=2.5pt, dashed] coordinates {
(0, 1)
(1, 0.544211)
(2, 0.43881)
(3, 0.369319)
(4, 0.316247)
(5, 0.260111)
(6, 0.235175)
(7, 0.203779)
(8, 0.172092)
(9, 0.133484)
(10, 0.102394)
(11, 0.088253)
(12, 0.0702704)
(13, 0.0605887)
(14, 0.0539195)
(15, 0.0477762)
(16, 0.0427875)
(17, 0.0363957)
(18, 0.0300501)
(19, 0.028704)
(20, 0.0238064)
(21, 0.0151937)
(22, 0.0102092)
(23, 0.00820208)
(24, 0.00494406)
(25, 0.00294587)
(26, 0.00203383)
(27, 0.00169409)
(28, 0.00116747)
(29, 0.000726109)
(30, 0.000484971)
(31, 0.000290553)
(32, 0.000197199)
(33, 0.000125515)
(34, 9.86511e-05)
(35, 6.96263e-05)
(36, 6.05552e-05)
(37, 4.77178e-05)
(38, 3.65238e-05)
(39, 2.36541e-05)
(40, 1.49396e-05)
(41, 8.13123e-06)
(42, 5.23441e-06)
(43, 2.76801e-06)
(44, 1.70529e-06)
(45, 9.97634e-07)
(46, 6.31462e-07)
(47, 4.17748e-07)
(48, 2.68759e-07)
(49, 1.4641e-07)
(50, 8.96047e-08)
(51, 6.58471e-08)
(52, 3.60385e-08)
(53, 1.83715e-08)
(54, 9.1608e-09)
(55, 5.19643e-09)
(56, 2.53474e-09)
(57, 9.98888e-10)
(58, 5.29124e-10)
(59, 3.14565e-10)
(60, 1.65223e-10)
(61, 6.77231e-11)
(62, 3.12177e-11)
(63, 1.4924e-11)
(64, 6.88378e-12)
(65, 3.62111e-12)
(66, 1.6972e-12)
(67, 6.67461e-13)
(68, 3.31308e-13)
(69, 1.67469e-13)
(70, 9.14334e-14)
}; \label{plot:fp64mixed}
\addplot[ color=mygreen, line width=1.5pt, dotted] coordinates {
(0, 1)
(1, 0.544211)
(2, 0.438838)
(3, 0.369323)
(4, 0.316184)
(5, 0.260064)
(6, 0.235192)
(7, 0.20376)
(8, 0.17206)
(9, 0.133436)
(10, 0.102378)
(11, 0.0882489)
(12, 0.070251)
(13, 0.0606022)
(14, 0.0539072)
(15, 0.0477522)
(16, 0.0427651)
(17, 0.0363788)
(18, 0.0300431)
(19, 0.0286853)
(20, 0.0237904)
(21, 0.0151927)
(22, 0.0102064)
(23, 0.00819317)
(24, 0.00493662)
(25, 0.00294336)
(26, 0.00203194)
(27, 0.00169244)
(28, 0.00116734)
(29, 0.000725639)
(30, 0.000484906)
(31, 0.000290726)
(32, 0.000197361)
(33, 0.000125743)
(34, 9.89401e-05)
(35, 6.99311e-05)
(36, 6.09404e-05)
(37, 4.81945e-05)
(38, 3.70084e-05)
(39, 2.43365e-05)
(40, 1.58661e-05)
(41, 9.00494e-06)
(42, 5.885e-06)
(43, 3.54038e-06)
(44, 2.61443e-06)
(45, 2.06881e-06)
(46, 2.10781e-06)
(47, 2.33597e-06)
(48, 2.25679e-06)
(49, 1.91326e-06)
(50, 1.70384e-06)
(51, 1.27602e-06)
(52, 7.25523e-07)
(53, 4.69342e-07)
(54, 3.58804e-07)
(55, 2.49243e-07)
(56, 1.4383e-07)
(57, 8.96481e-08)
(58, 7.72755e-08)
(59, 6.25663e-08)
(60, 6.28196e-08)
(61, 6.71828e-08)
(62, 4.17198e-08)
(63, 2.29825e-08)
(64, 1.28389e-08)
(65, 7.09185e-09)
(66, 3.89451e-09)
(67, 2.0331e-09)
(68, 1.13173e-09)
(69, 7.70403e-10)
(70, 6.25045e-10)
(71, 5.25486e-10)
(72, 4.27767e-10)
(73, 2.72555e-10)
(74, 1.33156e-10)
(75, 7.40693e-11)
(76, 4.3838e-11)
(77, 3.39546e-11)
(78, 3.4405e-11)
(79, 3.01627e-11)
(80, 2.041e-11)
(81, 1.1589e-11)
(82, 8.5744e-12)
(83, 8.93941e-12)
(84, 9.96058e-12)
(85, 1.00768e-11)
(86, 7.73741e-12)
(87, 5.1773e-12)
(88, 5.36834e-12)
(89, 5.28377e-12)
(90, 3.12419e-12)
(91, 1.55911e-12)
(92, 9.50887e-13)
(93, 5.88127e-13)
(94, 4.82883e-13)
(95, 3.35899e-13)
(96, 1.73954e-13)
(97, 8.66199e-14)
}; \label{plot:fp16}
\addplot[only marks, mark=*, color=black, mark options={ fill=black}, line width=1.5pt] coordinates {
(36, 6.05552e-05)
}; \label{plot:fp64tofp32}
\addplot[only marks, mark=*, color=mygreen, mark options={ fill=mygreen}, line width=1.5pt] coordinates {
 (56, 2.53474e-09)
};\label{plot:fp32tofp16}




==> 5.Numerical/data/varyConditionNum1e5.tex <==
\addplot[color=vtorange, line width=1.5pt] coordinates {
(0, 1)
(1, 0.536966)
(2, 0.365827)
(3, 0.315541)
(4, 0.35696)
(5, 0.387851)
(6, 0.432596)
(7, 0.489748)
(8, 0.435371)
(9, 0.461652)
(10, 0.435264)
(11, 0.362387)
(12, 0.485582)
(13, 0.618906)
(14, 0.62305)
(15, 0.749495)
(16, 0.814717)
(17, 1.02179)
(18, 1.30697)
(19, 2.00241)
(20, 2.81786)
(21, 3.50408)
(22, 4.57256)
(23, 5.16128)
(24, 5.89897)
(25, 6.24143)
(26, 5.82055)
(27, 5.35186)
(28, 5.06394)
(29, 4.36046)
(30, 3.73226)
(31, 2.74161)
(32, 2.34332)
(33, 1.87396)
(34, 1.33398)
(35, 1.12841)
(36, 0.852151)
(37, 0.625073)
(38, 0.410935)
(39, 0.251617)
(40, 0.163524)
(41, 0.115414)
(42, 0.0605193)
(43, 0.0337933)
(44, 0.0221717)
(45, 0.0146575)
(46, 0.00980318)
(47, 0.00548242)
(48, 0.0034616)
(49, 0.00217464)
(50, 0.00134698)
(51, 0.000998087)
(52, 0.000759683)
(53, 0.000425507)
(54, 0.000227499)
(55, 0.000129941)
(56, 7.88687e-05)
(57, 3.89824e-05)
(58, 2.1661e-05)
(59, 1.04554e-05)
(60, 4.74982e-06)
(61, 2.29385e-06)
(62, 1.09154e-06)
(63, 5.60901e-07)
(64, 2.99316e-07)
(65, 1.37361e-07)
(66, 6.04714e-08)
(67, 2.60526e-08)
(68, 8.52771e-09)
(69, 3.69976e-09)
(70, 1.36104e-09)
(71, 4.06494e-10)
(72, 1.53605e-10)
(73, 6.3671e-11)
(74, 2.42019e-11)
(75, 1.01002e-11)
(76, 5.1964e-12)
(77, 2.67826e-12)
(78, 1.33813e-12)
(79, 5.72073e-13)
(80, 2.32081e-13)
(81, 7.91527e-14)
}; \label{plot:fp64}
\addplot[ color=mydeepblue, line width=2.5pt, dashed] coordinates {
(0, 1)
(1, 0.536966)
(2, 0.365827)
(3, 0.315541)
(4, 0.35696)
(5, 0.387851)
(6, 0.432596)
(7, 0.489748)
(8, 0.435371)
(9, 0.461652)
(10, 0.435264)
(11, 0.362387)
(12, 0.485582)
(13, 0.618906)
(14, 0.62305)
(15, 0.749495)
(16, 0.814717)
(17, 1.02179)
(18, 1.30697)
(19, 2.00241)
(20, 2.81786)
(21, 3.50408)
(22, 4.57256)
(23, 5.16128)
(24, 5.89897)
(25, 6.24143)
(26, 5.82055)
(27, 5.35186)
(28, 5.06394)
(29, 4.36046)
(30, 3.73226)
(31, 2.74161)
(32, 2.34332)
(33, 1.87396)
(34, 1.33398)
(35, 1.12841)
(36, 0.852151)
(37, 0.625073)
(38, 0.410935)
(39, 0.251617)
(40, 0.163524)
(41, 0.115414)
(42, 0.0605193)
(43, 0.0337933)
(44, 0.0221717)
(45, 0.0146575)
(46, 0.00980318)
(47, 0.00548242)
(48, 0.0034616)
(49, 0.00217464)
(50, 0.00134698)
(51, 0.000998087)
(52, 0.000759683)
(53, 0.000425507)
(54, 0.000227499)
(55, 0.000129941)
(56, 7.88687e-05)
(57, 3.89824e-05)
(58, 2.1661e-05)
(59, 1.04554e-05)
(60, 4.74982e-06)
(61, 2.29385e-06)
(62, 1.09154e-06)
(63, 5.60901e-07)
(64, 2.99316e-07)
(65, 1.37361e-07)
(66, 6.04714e-08)
(67, 2.60526e-08)
(68, 8.52771e-09)
(69, 3.69976e-09)
(70, 1.3609e-09)
(71, 4.06387e-10)
(72, 1.53565e-10)
(73, 6.36545e-11)
(74, 2.4188e-11)
(75, 1.0089e-11)
(76, 5.17464e-12)
(77, 2.65658e-12)
(78, 1.33442e-12)
(79, 5.83923e-13)
(80, 2.59428e-13)
(81, 1.41635e-13)
(82, 1.87732e-13)
(83, 3.84802e-13)
(84, 6.8042e-13)
(85, 5.46453e-13)
(86, 4.96971e-13)
(87, 7.06131e-13)
(88, 1.36996e-12)
(89, 1.76082e-12)
(90, 1.59828e-12)
(91, 1.91129e-12)
(92, 3.09714e-12)
(93, 5.26211e-12)
(94, 7.74227e-12)
(95, 4.65643e-12)
(96, 5.18936e-12)
(97, 4.85136e-12)
(98, 2.73917e-12)
(99, 2.045e-12)
(100, 2.263e-12)
}; \label{plot:fp64mixed}
\addplot[ color=mygreen, line width=1.5pt, dotted] coordinates {
(0, 1)
(1, 0.536966)
(2, 0.365832)
(3, 0.315532)
(4, 0.356988)
(5, 0.387891)
(6, 0.432591)
(7, 0.489678)
(8, 0.435259)
(9, 0.461721)
(10, 0.435381)
(11, 0.362335)
(12, 0.485511)
(13, 0.618336)
(14, 0.622687)
(15, 0.749677)
(16, 0.814619)
(17, 1.02212)
(18, 1.30473)
(19, 2.00031)
(20, 2.82572)
(21, 3.50595)
(22, 4.56518)
(23, 5.17881)
(24, 5.85933)
(25, 6.19761)
(26, 5.78026)
(27, 5.33642)
(28, 5.03573)
(29, 4.39374)
(30, 3.66503)
(31, 2.75382)
(32, 2.34897)
(33, 1.87839)
(34, 1.36391)
(35, 1.16381)
(36, 0.900976)
(37, 0.683872)
(38, 0.455958)
(39, 0.265943)
(40, 0.170896)
(41, 0.126675)
(42, 0.0727145)
(43, 0.0396763)
(44, 0.0247929)
(45, 0.0170944)
(46, 0.0123146)
(47, 0.00787631)
(48, 0.0054414)
(49, 0.00478474)
(50, 0.00450623)
(51, 0.00560251)
(52, 0.00627863)
(53, 0.00589584)
(54, 0.00522488)
(55, 0.00577956)
(56, 0.00551352)
(57, 0.00472636)
(58, 0.00451177)
(59, 0.00518889)
(60, 0.00623378)
(61, 0.00941563)
(62, 0.0136337)
(63, 0.0198308)
(64, 0.0294329)
(65, 0.0344817)
(66, 0.0317944)
(67, 0.0306309)
(68, 0.0396157)
(69, 0.0666628)
(70, 0.0973035)
(71, 0.0978306)
(72, 0.0807815)
(73, 0.0587973)
(74, 0.0500207)
(75, 0.0385716)
(76, 0.0357448)
(77, 0.027953)
(78, 0.017804)
(79, 0.00964345)
(80, 0.00410407)
(81, 0.00266651)
(82, 0.00283345)
(83, 0.00288956)
(84, 0.00186098)
(85, 0.000823239)
(86, 0.000418619)
(87, 0.00025226)
(88, 0.000205391)
(89, 0.00014446)
(90, 7.78386e-05)
(91, 4.89994e-05)
(92, 3.56925e-05)
(93, 3.52772e-05)
(94, 4.68263e-05)
(95, 5.77636e-05)
(96, 5.98056e-05)
(97, 6.69759e-05)
(98, 5.28594e-05)
(99, 4.70539e-05)
(100, 5.2513e-05)
}; \label{plot:fp16}
\addplot[only marks, mark=*, color=black, mark options={ fill=black}, line width=1.5pt] coordinates {
(57, 3.89824e-05)
}; \label{plot:fp64tofp32}
\addplot[only marks, mark=*, color=mygreen, mark options={ fill=mygreen}, line width=1.5pt] coordinates {
 (69, 3.69976e-09)
};\label{plot:fp32tofp16}


